Theoretical Insights Into Multiclass Classification: A High-dimensional Asymptotic View

Contemporary machine learning applications often involve classification tasks with many classes. Despite their extensive use, a precise understanding of the statistical properties and behavior of classification algorithms is still missing, especially in modern regimes where the number of classes is rather large. In this paper, we take a step in this direction by providing the first asymptotically precise analysis of linear multiclass classification. Our theoretical analysis allows us to precisely characterize how the test error varies over different training algorithms, data distributions, problem dimensions as well as number of classes, inter/intra class correlations and class priors. Specifically, our analysis reveals that the classification accuracy is highly distribution-dependent with different algorithms achieving optimal performance for different data distributions and/or training/features sizes. Unlike linear regression/binary classification, the test error in multiclass classification relies on intricate functions of the trained model (e.g., correlation between some of the trained weights) whose asymptotic behavior is difficult to characterize. This challenge is already present in simple classifiers, such as those minimizing a square loss. Our novel theoretical techniques allow us to overcome some of these challenges. The insights gained may pave the way for a precise understanding of other classification algorithms beyond those studied in this paper.

==> Bayes_proof_bc.tex <==
\section{Proof of Proposition \ref{propo:Bayes}}
By \eqref{eq:Bayes_def} the Bayes estimator is the ML estimator:
\begin{align}
\yh_{n+1} &= \arg\max_{\eb_j,~j\in[k]} P\left( \y=\eb_j~|~\X,\Y,\x_{n+1}\right) \nn\\
&= \arg\max_{\eb_j,~j\in[k]} \E_{\M|\X,\Y} \left[P\left( \y=\eb_j~|~\x_{n+1},\M\right) \right] \nn\\
&= \arg\max_{\eb_j,~j\in[k]} \int P\left( \y=\eb_j~|~\x_{n+1},\M\right) \,\mathrm{d}P\left(\M~|~\X,\Y\right)\nn\\
&= \arg\max_{\eb_j,~j\in[k]} \int \frac{P\left( \x_{n+1}\,|\,\y=\eb_j,\M\right)}{P\left(\x_{n+1}|\M\right)} \,\mathrm{d}P\left(\M~|~\X,\Y\right)\label{eq:Bayesr}\\
&= \arg\max_{j\in[k]} \int \exp\left(-\twonorm{\x_{n+1} - \mub_j}^2\big/2\right) \,\mathrm{d}P\left(\M~|~\X,\Y\right).\label{eq:ML}
\end{align}
{\color{blue}missing $p(\x_{n+1}|M)$}
where in \eqref{eq:Bayesr} we used the Bayes rule and in the last  line we recall that $\z_{n+1}\sim\Nn(0,\Id_d)$.
To continue, we compute the posterior probability of the mean matrix given the training data as follows:
\bea
P\left(\M~|~\X,\Y\right) &\propto P\left(\X~|~\M,\Y\right)\cdot P\left(\M\right) \propto \exp\left(-\frac{\twonorm{\X-\M\Y}^2}{2}\right)\cdot \exp\left(-\frac{\twonorm{\M}^2}{2(r^2/d)}\right) \nn\\
&\propto\prod_{c=1}^k  \left\{\exp\left(-\frac{\twonorm{\mub_c}^2}{2(r^2/d)}\right) \cdot\prod_{i\in\Cc_c} \exp\left(-\frac{\twonorm{\x_i-\mub_c}^2}{2}\right)\right\},
\end{align}
where we denote by $\Cc_c$ the collection of training samples that belong to class $c\in[k]$, i.e. $\Cc_c=\{i\in[n]~|~\y_i=\eb_c\}.$ With this the objective function of the ML rule in \eqref{eq:ML} becomes:
\begin{align}
\yh_{n+1} = \arg \max_{j\in[k]}~\Ic(\ell,\Cc_{j}\cap{n+1})\cdot\prod_{\substack{c=1 \\ c\neq j}}^k\Ic(c,\Cc_c)\label{eq:Bayes1}
%\left\{\int \mathrm{d}{\mub_j}\,\exp\left(-\frac{\twonorm{\mub_j}^2}{2(r^2/d)}\right) \cdot\prod_{i\in\Cc_c\cup\{n+1\}} \exp\left(-\frac{\twonorm{\x_i-\mub_j}^2}{2}\right)\right\} \prod_{c\neq j}\left\{ \int \mathrm{d}{\mub_c}\, \exp\left(-\frac{\twonorm{\mub_c}^2}{2(r^2/d)}\right) \cdot\prod_{i\in\Cc_c} \exp\left(-\frac{\twonorm{\x_i-\mub_c}^2}{2}\right)  \right\}
\end{align}
where for $\ell\in[k]$ and a subset $\Ac\subset[n+1]$ we denote
$$
\Ic(\ell,\Ac) := \int \mathrm{d}{\mub_c}\,\exp\left(-\frac{\twonorm{\mub_c}^2}{2(r^2/d)}\right) \cdot \exp\left(-\sum_{i\in\Ac}\frac{\twonorm{\x_i-\mub_c}^2}{2}\right)\,.
$$
A simple argument of completing the squares and invoking a gaussian integral yields
\bea
\Ic(\ell,\Ac) &:= \sqrt{\frac{(d/r^2+|\Ac|)}{(2{\varpi})^d}}\exp\left(-\frac{\left(1-\frac{1}{d/r^2+|\Ac|}\right)}{2}\sum_{i\in\Ac}\twonorm{\x_i}^2 + \frac{1}{2\left(d/r^2+|\Ac|\right)}\sum_{i\in\Ac}\inp{\x_i}{\sum_{\substack{j\in\Ac\\j\neq i}}\x_j} \right) \nn \\
&:= \sqrt{\frac{(d/r^2+|\Ac|)}{(2{\varpi})^d}}\exp\left(-\frac{1}{2\left(\frac{d}{r^2}+{|\Ac|}\right)}\left( \left(\frac{d}{r^2}+|\Ac| - 1\right) \sum_{i\in\Ac}\twonorm{\x_i}^2 - \sum_{i\in\Ac}\inp{\x_i}{\sum_{\substack{j\in\Ac\\j\neq i}}\x_j} \right) \right) \nn\\
&:= \sqrt{\frac{(d/r^2+|\Ac|)}{(2{\varpi})^d}}\exp\left(-\frac{1}{2\left(\frac{d/n}{r^2}+{|\Ac|/n}\right)}\left( \left(\frac{d/n}{r^2}+\frac{|\Ac|}{n} - \frac{1}{n}\right) \sum_{i\in\Ac}\twonorm{\x_i}^2 - \frac{1}{n}\sum_{i\in\Ac}\inp{\x_i}{\sum_{\substack{j\in\Ac\\j\neq i}}\x_j} \right) \right) \nn
\end{align}
Using this in \eqref{eq:Bayes1} we have that
\bea
\yh_{n+1} = \arg\max_{j\in[k]} ~\Ic(j) \cdot \exp\left(-\frac{1}{2\left(\frac{d/n}{r^2}+\frac{n_j+1}{n}\right)}\left( \left(\frac{d/n}{r^2}+\frac{n_j}{n}\right) \twonorm{\x_{n+1}}^2 - \frac{2}{n}\inp{\x_{n+1}}{\sum_{\substack{\ell\in\Cc_j}}\x_\ell} \right) \right) \label{eq:Bayes2}
\end{align}
where $\xi(n_c) := \frac{d/n}{r^2}+\frac{n_c}{n},~c\in[k]$ and 
\bea
\Ic(j):= \prod_{\substack{c=1\\ c\neq j}}^{k}e^{-\frac{1}{2\xi(n_c)}\left( \left(\xi(n_c) - \frac{1}{n}\right) \sum_{i\in\Cc}\twonorm{\x_i}^2 - \frac{1}{n}\sum_{i\in\Cc}\inp{\x_i}{\sum_{\substack{\ell\in\Cc\\\ell\neq i}}\x_\ell} \right) }\cdot e^{-\frac{1}{2\left(\xi(n_{j})+\frac{1}{n}\right)}\left( \xi(n_{j}) \sum_{i\in\Cc_j}\twonorm{\x_i}^2 - \frac{1}{n}\sum_{i\in\Cc_j}\inp{\x_i}{\sum_{\substack{\ell\in\Cc_j\\\ell\neq i}}\x_\ell} \right)} \,. \nn
\end{align}
Since the term $\Ic$ is independent of $j$ in the maximization in \eqref{eq:Bayes2}, we conclude that
\bea
\yh_{n+1} &= \arg\max_{j\in[k]} ~\log\left(\Ic(j)\right)-\frac{1}{2\left(\frac{d/n}{r^2}+\frac{n_j+1}{n}\right)}\left\{\left(\frac{d/n}{r^2}+\frac{n_j}{n}\right) \twonorm{\x_{n+1}}^2 - \frac{2}{n}\inp{\x_{n+1}}{\sum_{\substack{\ell\in\Cc_j}}\x_\ell} \right\}\nn \\
&= \arg\max_{j\in[k]} ~\log\left(\Ic(j)\right) +  \frac{1}{2\left(\frac{d/n}{r^2}+\frac{n_j+1}{n}\right)}\left\{  \frac{2}{n}\inp{\x_{n+1}}{\sum_{\substack{\ell\in\Cc_j}}\x_\ell} \right\}
 \label{eq:Bayes3}
\end{align}
Next, we evaluate the objective in \eqref{eq:Bayes3} in the asymptotic limit $n,d\rightarrow\infty, n/d=\gamma$. First, since $n_c/n\rP \pi$, note that $\Ic(j)-\Ic(\ell)\rP 0$ for all $i,j\in[k]$. Moreover, note that
\bea
\frac{1}{n}\inp{\x_{n+1}}{\sum_{\ell\in \Cc_j}\x_\ell} &= \frac{1}{n}\inp{\M\y_{n+1} + \z_{n+1}}{ n_j\,\mub_j + \sum_{\ell\in \Cc_j}\z_\ell}\nn\\
&= \frac{n_j}{n}\inp{\M\y_{n+1}}{\mub_j}  + \frac{n_j}{n}\inp{\z_{n+1}}{\mub_j}  + \frac{1}{n}\sum_{\ell\in\Cc_j}\inp{\M\y_{n+1}}{\z_\ell} +  \frac{1}{n}\sum_{\ell\in\Cc_j}\inp{\z_{n+1}}{\z_\ell} \label{eq:fourTerms}
\end{align}
For each one of the four terms in \eqref{eq:fourTerms}, we have the following by the CLT:
\bea
&\frac{n_j}{n}\inp{\M\y_{n+1}}{\mub_\ell} \rP \pi r^2 \inp{\y_{n+1}}{\eb_j} \nn\\
& \frac{n_j}{n}\inp{\z_{n+1}}{\mub_j} \rD \Nn(0,\pi^2 r^2)\nn\\
&\frac{1}{n}\sum_{\ell\in\Cc_j}\inp{\M\y_{n+1}}{\z_\ell} \rP 0 \nn\\
&\frac{1}{n}\sum_{\ell\in\Cc_j}\inp{\z_{n+1}}{\z_\ell} \rD \Nn(0,\pi \gamma), \nn
\end{align}
where in the last line we used the fact that $\frac{1}{\sqrt{n_j}}\sum_{\ell\in\Cc_j}\frac{\inp{\z_{n+1}}{\z_\ell}}{\sqrt{n}}\rD \Nn(0,\gamma)$. 

Therefore, in the asymptotic limit, the Bayes estimator is the solution to:
\bea
\yh_{n+1} &= \arg\max_{\eb_j, j\in[k]} \pi r^2 \inp{\y_{n+1}}{\eb_j} + \sqrt{\pi\left(\pi r^2 + \gamma\right)}\, G_j,\quad G_1,\ldots,G_k\simiid\Nn(0,1).
\end{align}
As such, the probability of error is
\bea
\P_e &= \P\left(\yh_{n+1}\neq\y_{n+1}\right) = \P\left(  \pi r^2 + \sqrt{\pi\left(\pi r^2 + \gamma\right)}\, G_0 \leq \max_{\ell\in[k-1]} \sqrt{\pi\left(\pi r^2 + \gamma\right)}\, G_\ell  \right)\nn\\
&= \P\left( G_0 + \max_{\ell\in[k-1]}  G_\ell \geq r^2\sqrt{\frac{\pi}{\pi r^2 + \gamma}}  \right),
\end{align}


==> Organization.tex <==
%\section{Organization and Notation}


%\subsection{Organization of the supplementary}

%\subsection{Notation}

==> Proof_LS.tex <==
\section{Proofs for LS}

\begin{align*}
\underset{\mtx{W}\in\R^{k\times d},\text{ }\vct{b}\in\R^k}{\min}\quad \frac{1}{2n}\fronorm{\mtx{W}\mtx{X}+\vct{b}\vct{1}_n^T-\mtx{Y}}^2=&\sum_{\ell=1}^k \min_{\vct{w}_\ell, \vct{b}_\ell}\text{ }\frac{1}{2n}\twonorm{\mtx{X}^T\vct{w}_\ell+b_\ell\vct{1}_n-\mtx{Y}_\ell}^2\\
=&\sum_{\ell=1}^k \min_{\vct{w}_\ell, \vct{b}_\ell}\text{ }\frac{1}{2n}\twonorm{\mtx{Y}^T\mtx{M}^T\vct{w}_\ell+\sigma\mtx{Z}^T\vct{w}_\ell+b_\ell\vct{1}_n-\mtx{Y}_\ell}^2
\end{align*}

Define 
\begin{align*}
\mathcal{L}_{PO}\left(\vct{w}_\ell,b_\ell\right):=\frac{1}{2n}\twonorm{\mtx{Y}^T\mtx{M}^T\vct{w}_\ell+\sigma\mtx{Z}^T\vct{w}_\ell+b_\ell\vct{1}_n-\mtx{Y}_\ell}^2
\end{align*}
To continue further note that by duality we have
\begin{align*}
\min_{\vct{w}_\ell, \vct{b}_\ell}\text{ }\mathcal{L}_{PO}\left(\vct{w}_\ell,b_\ell\right) =\min_{\vct{w}_\ell, \vct{b}_\ell}\text{ }\max_{\vct{s}}\text{ }\frac{1}{n}\left(\vct{s}^T\mtx{Y}^T\mtx{M}^T\vct{w}_\ell+\sigma\vct{s}^T\mtx{Z}^T\vct{w}_\ell+b_\ell\vct{s}^T\vct{1}_n-\vct{s}^T\mtx{Y}_\ell-\frac{\twonorm{\vct{s}}^2}{2}\right)
\end{align*}
Note that the above is jointly convex in $(\vct{w}_\ell, b_\ell)$ and concave in $\vct{s}$. We consider the Auxiliary Optimization (AO) problem
\begin{align*}
\min_{\vct{w}_\ell, \vct{b}_\ell}\text{ }\max_{\vct{s}}\text{ }\frac{1}{n}\left(\vct{s}^T\mtx{Y}^T\mtx{M}^T\vct{w}_\ell+\sigma\twonorm{\vct{w}_\ell}\vct{g}^T\vct{s}+\sigma\twonorm{\vct{s}}\vct{h}^T\vct{w}_\ell+b_\ell\vct{s}^T\vct{1}_n-\vct{s}^T\mtx{Y}_\ell-\frac{\twonorm{\vct{s}}^2}{2}\right)
\end{align*}
Maximizing over the direction of $\vct{s}$ and its norm $\beta=\twonorm{\vct{s}}$ we arrive at
\begin{align*}
\min_{\vct{w}_\ell, \vct{b}_\ell}\text{ }\max_{\beta\ge 0}\text{ } &\frac{1}{n}\left(\beta\twonorm{\sigma\twonorm{\vct{w}_\ell}\vct{g}+\mtx{Y}^T\mtx{M}^T\vct{w}_\ell+b_\ell\vct{1}_n-\mtx{Y}_\ell}+\sigma\beta\vct{h}^T\vct{w}_\ell-\frac{\beta^2}{2}\right)\\
&\quad\quad\quad\quad\quad\quad=\min_{\vct{w}_\ell, \vct{b}_\ell}\text{ }\frac{1}{2n}\left(\twonorm{\sigma\twonorm{\vct{w}_\ell}\vct{g}+\mtx{Y}^T\mtx{M}^T\vct{w}_\ell+b_\ell\vct{1}_n-\mtx{Y}_\ell}+\sigma\vct{h}^T\vct{w}_\ell\right)_{+}^2\\
&\quad\quad\quad\quad\quad\quad=\frac{1}{2}\left(\min_{\vct{w}_\ell, \vct{b}_\ell}\text{ } \frac{1}{\sqrt{n}}\twonorm{\sigma\twonorm{\vct{w}_\ell}\vct{g}+\mtx{Y}^T\mtx{M}^T\vct{w}_\ell+b_\ell\vct{1}_n-\mtx{Y}_\ell}+\frac{1}{\sqrt{n}}\sigma\vct{h}^T\vct{w}_\ell\right)_{+}^2
\end{align*}
To continue we decompose the optimization over $\vct{w}_\ell$ into its norm $\alpha=\twonorm{\vct{w}_\ell}$ and its direction to arrive at the following optimization problem inside the paranthesis
\begin{align*}
\min_{\vct{b}_\ell}\text{ }\min_{\alpha\ge 0}\text{ }\min_{\vct{w}_\ell:\text{ }\twonorm{\vct{w}_\ell}=1}\text{ }\frac{1}{\sqrt{n}}\twonorm{\alpha\sigma\vct{g}+\alpha\mtx{Y}^T\mtx{M}^T\vct{w}_\ell+b_\ell\vct{1}_n-\mtx{Y}_\ell}+\frac{1}{\sqrt{n}}\alpha\sigma\vct{h}^T\vct{w}_\ell
\end{align*}
To continue consider the eigenvalue decomposition
\begin{align*}
\mtx{M}\mtx{Y}=\mtx{U}\mtx{\Sigma}\mtx{V}^T,
\end{align*}
with $\mtx{U}\in\R^{d\times r}$, $\mtx{\Sigma}\in\R^{r\times r}$, and $\mtx{V}\in\R^{n\times r}$ where $r=$rank$(\mtx{M}\mtx{Y})\le k$. Using this decomposition we have
\begin{align*}
&\frac{1}{\sqrt{n}}\twonorm{\alpha\sigma\vct{g}+\alpha\mtx{Y}^T\mtx{M}^T\vct{w}_\ell+b_\ell\vct{1}_n-\mtx{Y}_\ell}+\frac{1}{\sqrt{n}}\alpha\sigma\vct{h}^T\vct{w}_\ell\\
&\quad=\frac{1}{\sqrt{n}}\sqrt{\twonorm{\mtx{V}\mtx{V}^T\left(\alpha\sigma\vct{g}+\alpha\mtx{Y}^T\mtx{M}^T\vct{w}_\ell+b_\ell\vct{1}_n-\mtx{Y}_\ell\right)}^2+\twonorm{\left(\mtx{I}-\mtx{V}\mtx{V}^T\right)\left(\alpha\sigma\vct{g}+\alpha\mtx{Y}^T\mtx{M}^T\vct{w}_\ell+b_\ell\vct{1}_n-\mtx{Y}_\ell\right)}^2}\\
&\quad\quad+\frac{1}{\sqrt{n}}\alpha\sigma\vct{h}^T\vct{w}_\ell\\
&\quad=\frac{1}{\sqrt{n}}\sqrt{\twonorm{\alpha\sigma\mtx{V}\mtx{V}^T\vct{g}+\alpha\mtx{Y}^T\mtx{M}^T\vct{w}_\ell+b_\ell\vct{1}_n-\mtx{Y}_\ell}^2+\alpha^2\sigma^2\twonorm{\left(\mtx{I}-\mtx{V}\mtx{V}^T\right)\vct{g}}^2}\\
&\quad\quad+\frac{1}{\sqrt{n}}\alpha\sigma\vct{h}^T\vct{w}_\ell\\
&\quad=\frac{1}{\sqrt{n}}\sqrt{2\alpha^2\sigma^2\langle \mtx{V}^T\vct{g},\mtx{V}^T\mtx{Y}^T\mtx{M}^T\vct{w}_\ell\rangle +\twonorm{\alpha\mtx{Y}^T\mtx{M}^T\vct{w}_\ell+b_\ell\vct{1}_n-\mtx{Y}_\ell}^2+\alpha^2\sigma^2\twonorm{\mtx{V}\mtx{V}^T\vct{g}}^2+\alpha^2\sigma^2\twonorm{\left(\mtx{I}-\mtx{V}\mtx{V}^T\right)\vct{g}}^2}\\
&\quad\quad+\frac{1}{\sqrt{n}}\alpha\sigma\vct{h}^T\vct{w}_\ell\\
&\quad=\sqrt{2\alpha^2\sigma^2\frac{\langle \mtx{V}^T\vct{g},\mtx{V}^T\mtx{Y}^T\mtx{M}^T\vct{w}_\ell\rangle}{n} +\frac{1}{n}\twonorm{\alpha\mtx{Y}^T\mtx{M}^T\vct{w}_\ell+b_\ell\vct{1}_n-\mtx{Y}_\ell}^2+\alpha^2\sigma^2\frac{\twonorm{\vct{g}}^2}{n}}\\
&\quad\quad+\frac{1}{\sqrt{n}}\alpha\sigma\langle \mtx{U}^T\vct{h}, \mtx{U}^T\vct{w}_\ell\rangle +\frac{1}{\sqrt{n}}\alpha\sigma\vct{h}^T\left(\mtx{I}-\mtx{U}\mtx{U}^T\right)\vct{w}_\ell
\end{align*}
where in the last line we used the fact that $\vct{1}_n, \mtx{Y}_\ell\in\text{span}\left(\mtx{V}\right)$. Note that since $r\le k$ and $k$ is fixed we have $\lim_{n\rightarrow+\infty} \frac{\langle \mtx{V}^T\vct{g},\mtx{V}^T\mtx{Y}^T\mtx{M}^T\vct{w}_\ell\rangle}{n}=0$, $\lim_{n\rightarrow+\infty} \frac{1}{\sqrt{n}}\alpha\sigma\langle \mtx{U}^T\vct{h}, \mtx{U}^T\vct{w}_\ell\rangle=0$, and $\lim_{n\rightarrow+\infty}\frac{\twonorm{\vct{g}}^2}{n}=1$. Thus using the fact that $\vct{1}_n, \mtx{Y}_\ell\in\text{span}\left(\mtx{V}\right)$ the minimization over $\vct{w}_\ell$ takes the form
\begin{align*}
\min_{\vct{w}_\ell:\text{ }\twonorm{\vct{w}_\ell}=1}\text{ }\sqrt{\frac{1}{n}\twonorm{\alpha\mtx{\Sigma}\mtx{U}^T\vct{w}_\ell+\mtx{V}^T\left(b_\ell\vct{1}_n-\mtx{Y}_\ell\right)}^2+\alpha^2\sigma^2}+\frac{1}{\sqrt{n}}\alpha\sigma\vct{h}^T\left(\mtx{I}-\mtx{U}\mtx{U}^T\right)\vct{w}_\ell
\end{align*}
To continue further define $\mtx{U}_\perp\in\R^{d\times (d-r)}$ so that $\mtx{U}_\perp\mtx{U}_\perp^T= \mtx{I}-\mtx{U}\mtx{U}^T$. Furthermore, define
\begin{align*}
\vct{w}_\ell=\mtx{U}\vct{w}+\mtx{U}_\perp\vct{w}_\perp\quad\text{with}\quad\vct{w}\in\R^r\quad\text{and}\quad\vct{w}_\perp\in\R^{d-r}. 
\end{align*}
After this change of variable, the optimize problem over $\vct{w}_\ell$ reduce to 
\begin{align*}
&\min_{0\le\gamma\le 1}\text{ }\min_{\vct{w}:\text{ }\twonorm{\vct{w}}=\gamma}\text{ }\min_{\vct{w}_\perp:\text{ }\twonorm{\vct{w}_\perp}=\sqrt{1-\gamma^2}}\text{ }\sqrt{\frac{1}{n}\twonorm{\alpha\mtx{\Sigma}\vct{w}+\mtx{V}^T\left(b_\ell\vct{1}_n-\mtx{Y}_\ell\right)}^2+\alpha^2\sigma^2}+\frac{1}{\sqrt{n}}\alpha\sigma\langle \mtx{U}_\perp^T\vct{h},\vct{w}_\perp\rangle\\
&\quad\quad\quad\quad\quad\quad=\min_{0\le\gamma\le 1}\text{ }\min_{\vct{w}:\text{ }\twonorm{\vct{w}}=\gamma}\text{ }\sqrt{\frac{1}{n}\twonorm{\alpha\mtx{\Sigma}\vct{w}+\mtx{V}^T\left(b_\ell\vct{1}_n-\mtx{Y}_\ell\right)}^2+\alpha^2\sigma^2}-\frac{1}{\sqrt{n}}\sqrt{1-\gamma^2}\alpha\sigma\twonorm{\mtx{U}_\perp^T\vct{h}}\\
&\quad\quad\quad\quad\quad\quad=\min_{0\le\gamma\le 1}\text{ }\min_{\vct{w}:\text{ }\twonorm{\vct{w}}=1}\text{ }\sqrt{\frac{1}{n}\twonorm{\alpha\gamma\mtx{\Sigma}\vct{w}+\mtx{V}^T\left(b_\ell\vct{1}_n-\mtx{Y}_\ell\right)}^2+\alpha^2\sigma^2}-\frac{1}{\sqrt{n}}\sqrt{1-\gamma^2}\alpha\sigma\twonorm{\mtx{U}_\perp^T\vct{h}}
\end{align*}
Now using the fact that $\lim_{n\rightarrow+\infty}\frac{\twonorm{\mtx{U}_\perp^T\vct{h}}}{\sqrt{n}}=\lim_{n\rightarrow+\infty} \sqrt{1-\frac{r}{n}}=1$ the above reduces to
\begin{align*}
\min_{0\le\gamma\le 1}\text{ }\min_{\vct{w}:\text{ }\twonorm{\vct{w}}=1}\text{ }\sqrt{\frac{1}{n}\twonorm{\alpha\gamma\mtx{\Sigma}\vct{w}+\mtx{V}^T\left(b_\ell\vct{1}_n-\mtx{Y}_\ell\right)}^2+\alpha^2\sigma^2}-\sqrt{1-\gamma^2}\alpha\sigma%\\
%&\quad\quad\quad\quad\quad\quad=\min_{0\le\gamma\le 1}\text{ }\sqrt{\frac{1}{n}\min_{\vct{w}:\text{ }\twonorm{\vct{w}}=1}\text{ }\twonorm{\alpha\gamma\mtx{\Sigma}\vct{w}+\mtx{V}^T\left(b_\ell\vct{1}_n-\vct{v}_\ell\right)}^2+\alpha^2\sigma^2}-\sqrt{1-\gamma^2}\alpha\sigma
\end{align*}
Thus we have
\begin{align*}
&\min_{\vct{b}_\ell}\text{ }\min_{\alpha\ge 0}\text{ }\min_{\vct{w}_\ell:\text{ }\twonorm{\vct{w}_\ell}=1}\text{ }\frac{1}{\sqrt{n}}\twonorm{\alpha\sigma\vct{g}+\alpha\mtx{Y}^T\mtx{M}^T\vct{w}_\ell+b_\ell\vct{1}_n-\mtx{Y}_\ell}+\frac{1}{\sqrt{n}}\alpha\sigma\vct{h}^T\vct{w}_\ell\\
&\quad\quad\quad\quad\quad\quad
=\min_{\alpha\ge 0}\text{ }\min_{0\le\gamma\le 1}\text{ }\min_{\vct{w}:\text{ }\twonorm{\vct{w}}=1}\text{ }\sqrt{\frac{1}{n}\twonorm{\alpha\gamma\mtx{\Sigma}\vct{w}+\mtx{V}^T\left(b_\ell\vct{1}_n-\mtx{Y}_\ell\right)}^2+\alpha^2\sigma^2}-\sqrt{1-\gamma^2}\alpha\sigma
\end{align*}
Rewriting the above in terms of the original variable $\vct{w}_\ell$ the above reduces to
\begin{align*}
&\min_{\vct{w}_\ell}\text{ }\sqrt{\frac{1}{n}\twonorm{\mtx{\Sigma}\mtx{U}^T\vct{w}_\ell+\mtx{V}^T\left(b_\ell\vct{1}_n-\mtx{Y}_\ell\right)}^2+\sigma^2\twonorm{\vct{w}_\ell}^2}-\twonorm{\mtx{U}_\perp^T\vct{w}_\ell}\sigma\\
&\quad\quad\quad\quad\quad\quad\quad\quad=\min_{\vct{w}_\ell}\text{ }\sqrt{\frac{1}{n}\twonorm{\mtx{\Sigma}\mtx{U}^T\vct{w}_\ell+\mtx{V}^T\left(b_\ell\vct{1}_n-\mtx{Y}_\ell\right)}^2+\sigma^2\twonorm{\mtx{U}^T\vct{w}_\ell}^2+\sigma^2\twonorm{\mtx{U}_\perp^T\vct{w}_\ell}^2}-\twonorm{\mtx{U}_\perp^T\vct{w}_\ell}\sigma
\end{align*}
To continue note that $\min_x\text{ }\sqrt{a^2+x^2}-\abs{x}=\abs{a}$. Thus the above reduces to
\begin{align*}
\min_{\vct{w}_\ell}\text{ }\sqrt{\frac{1}{n}\twonorm{\mtx{\Sigma}\mtx{U}^T\vct{w}_\ell+\mtx{V}^T\left(b_\ell\vct{1}_n-\mtx{Y}_\ell\right)}^2+\sigma^2\twonorm{\mtx{U}^T\vct{w}_\ell}^2}=\sqrt{\min_{\vct{w}_\ell}\text{ }\frac{1}{n}\twonorm{\mtx{\Sigma}\mtx{U}^T\vct{w}_\ell+\mtx{V}^T\left(b_\ell\vct{1}_n-\mtx{Y}_\ell\right)}^2+\sigma^2\twonorm{\mtx{U}^T\vct{w}_\ell}^2}
\end{align*}
Thus asymptotically
\begin{align*}
&\frac{1}{2}\left(\min_{\vct{w}_\ell, \vct{b}_\ell}\text{ } \frac{1}{\sqrt{n}}\twonorm{\sigma\twonorm{\vct{w}_\ell}\vct{g}+\mtx{Y}^T\mtx{M}^T\vct{w}_\ell+b_\ell\vct{1}_n-\mtx{Y}_\ell}+\frac{1}{\sqrt{n}}\sigma\vct{h}^T\vct{w}_\ell\right)_{+}^2\\
&\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad=\min_{\vct{w}_\ell, b_\ell}\text{ }\frac{1}{2n}\twonorm{\mtx{\Sigma}\mtx{U}^T\vct{w}_\ell+\mtx{V}^T\left(b_\ell\vct{1}_n-\mtx{Y}_\ell\right)}^2+\frac{1}{2}\sigma^2\twonorm{\mtx{U}^T\vct{w}_\ell}^2\\
&\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad=\min_{\vct{w}_\ell, b_\ell}\text{ }\frac{1}{2n}\twonorm{\begin{bmatrix} \mtx{\Sigma} & \mtx{V}^T\vct{1}_n\end{bmatrix}\begin{bmatrix}\mtx{U}^T\vct{w}_\ell \\ b_\ell\end{bmatrix}-\mtx{V}^T\mtx{Y}_\ell}^2+\frac{1}{2}\twonorm{\begin{bmatrix} \sigma\mtx{I} & \vct{0}\end{bmatrix}\begin{bmatrix} \mtx{U}^T\vct{w}_\ell \\ b_\ell\end{bmatrix}}^2
\end{align*}
Setting the gradient with respect to $\mtx{U}^T\vct{w}_\ell$ and $b_\ell$ to zero we arrive at
\begin{align*}
\frac{1}{n}\begin{bmatrix} \mtx{\Sigma} & \mtx{V}^T\vct{1}_n\end{bmatrix}^T\left(\begin{bmatrix} \mtx{\Sigma} & \mtx{V}^T\vct{1}_n\end{bmatrix}\begin{bmatrix}\mtx{U}^T\vct{w}_\ell \\ b_\ell\end{bmatrix}-\mtx{V}^T\mtx{Y}_\ell\right)+\begin{bmatrix} \sigma\mtx{I} & \vct{0}\end{bmatrix}^T\begin{bmatrix} \sigma\mtx{I} & \vct{0}\end{bmatrix}\begin{bmatrix} \mtx{U}^T\vct{w}_\ell \\ b_\ell\end{bmatrix}=0
\end{align*}
Thus we have
\begin{align*}
\begin{bmatrix}
\mtx{\Sigma}^2+n\sigma^2\mtx{I} & \mtx{\Sigma}\mtx{V}^T\vct{1}_n\\
\left(\mtx{\Sigma}\mtx{V}^T\vct{1}_n\right)^T& n
\end{bmatrix}
\begin{bmatrix} \mtx{U}^T\vct{w}_\ell \\ b_\ell\end{bmatrix}
=
\begin{bmatrix}
\mtx{\Sigma}\mtx{V}^T\mtx{Y}_\ell \\
n_\ell
\end{bmatrix}
\end{align*}
Furthermore, using the fact that $\vct{1}_n\in \text{span}(\mtx{V})$ we have $\vct{1}_n^T\mtx{V}\mtx{V}^T\vct{1}_n=\twonorm{\vct{1}_n}^2=n$. Also by definition of $\mtx{Y}$ and $\mtx{V}$ we have $\mtx{Y}=\text{diag}(\sqrt{n_1}, \sqrt{n_2}, \ldots, \sqrt{n_k})\mtx{R}\mtx{V}^T$ for some rotation matrix $\mtx{R}\in\R^{k\times k}$ (i..e.~obeying $\mtx{R}^T\mtx{R}=\mtx{I}$). Thus 
\begin{align*}
\mtx{V}^T\vct{1}_n=&\mtx{R}^T\mtx{R}\mtx{V}^T\vct{1}_n\\
=&\mtx{R}^T\text{diag}\left(\frac{1}{\sqrt{n_1}}, \frac{1}{\sqrt{n_2}}, \ldots, \frac{1}{\sqrt{n_k}}\right)\mtx{Y}\vct{1}_n\\
=&\mtx{R}^T\text{diag}\left(\frac{1}{\sqrt{n_1}}, \frac{1}{\sqrt{n_2}}, \ldots, \frac{1}{\sqrt{n_k}}\right)\begin{bmatrix}
n_1\\
n_2\\
\vdots\\
n_k
\end{bmatrix}\\
=&\mtx{R}^T\begin{bmatrix}
\sqrt{n_1}\\
\sqrt{n_2}\\
\vdots\\
\sqrt{n_k}
\end{bmatrix}\\
=&\sqrt{n}\mtx{R}^T\sqrt{\vct{\pi}}.
\end{align*}
where $\pi_\ell:=\frac{n_\ell}{n}$ and for a vector $\vct{\pi}$, $\sqrt{\vct{\pi}}$ should be interpreted entry-wise. Similarly, we have
\begin{align*}
\mtx{V}^T\mtx{Y}_\ell=&\mtx{R}^T\text{diag}\left(\frac{1}{\sqrt{n_1}}, \frac{1}{\sqrt{n_2}}, \ldots, \frac{1}{\sqrt{n_k}}\right)\mtx{Y}\mtx{Y}_\ell\\
=&n_\ell\mtx{R}^T\text{diag}\left(\frac{1}{\sqrt{n_1}}, \frac{1}{\sqrt{n_2}}, \ldots, \frac{1}{\sqrt{n_k}}\right) \vct{e}_\ell\\
=&\sqrt{n_\el}\mtx{R}^T \vct{e}_\ell.
\end{align*}
We also have
\begin{align*}
\langle \mtx{V}^T\vct{1}_n, \mtx{V}^T\mtx{Y}_\ell\rangle = \sqrt{n_\ell n}\sqrt{\vct{\pi}}^T\mtx{R}\mtx{R}^T \vct{e}_\ell=\sqrt{n_\ell n}\sqrt{\vct{\pi}}^T \vct{e}_\ell=\sqrt{\pi_\ell} \sqrt{n_\ell n}=n_\ell
\end{align*}
Using the above identities we arrive at
\begin{align*}
\begin{bmatrix}
\mtx{\Sigma}^2+n\sigma^2\mtx{I} & \sqrt{n}\mtx{\Sigma}\mtx{R}^T\sqrt{\vct{\pi}}\\
\sqrt{n}\left(\mtx{\Sigma}\mtx{R}^T\sqrt{\vct{\pi}}\right)^T& n
\end{bmatrix}
\begin{bmatrix} \mtx{U}^T\vct{w}_\ell \\ b_\ell\end{bmatrix}
=
\begin{bmatrix}
\mtx{\Sigma}\sqrt{n_\el}\mtx{R}^T \vct{e}_\ell\\
n_\ell
\end{bmatrix}
\end{align*}
which can be rewritten as
\begin{align*}
\begin{bmatrix}
\frac{1}{n}\mtx{\Sigma}^2+\sigma^2\mtx{I} & \frac{1}{\sqrt{n}}\mtx{\Sigma}\mtx{R}^T\sqrt{\vct{\pi}}\\
\left(\frac{1}{\sqrt{n}}\mtx{\Sigma}\mtx{R}^T\sqrt{\vct{\pi}}\right)^T& 1
\end{bmatrix}
\begin{bmatrix} \mtx{U}^T\vct{w}_\ell \\ b_\ell\end{bmatrix}
=
\begin{bmatrix}
\frac{1}{\sqrt{n}}\mtx{\Sigma}\sqrt{\pi_\el}\mtx{R}^T \vct{e}_\ell\\
\pi_\ell
\end{bmatrix}
\end{align*}
This can then be simplifies to
\begin{align*}
\begin{bmatrix}
\widetilde{\mtx{\Sigma}}^2+\sigma^2\mtx{I} & \widetilde{\mtx{\Sigma}}\mtx{R}^T\sqrt{\vct{\pi}}\\
\left(\widetilde{\mtx{\Sigma}}\mtx{R}^T\sqrt{\vct{\pi}}\right)^T& 1
\end{bmatrix}
\begin{bmatrix} \mtx{U}^T\vct{w}_\ell \\ b_\ell\end{bmatrix}
=
\begin{bmatrix}
\widetilde{\mtx{\Sigma}}\sqrt{\pi_\el}\mtx{R}^T \vct{e}_\ell\\
\pi_\ell
\end{bmatrix}
\end{align*}
where $\widetilde{\mtx{\Sigma}}=\frac{1}{\sqrt{n}}\mtx{\Sigma}$. Thus
\begin{align*}
\begin{bmatrix} \mtx{U}^T\widehat{\vct{w}}_\ell \\ \widehat{b}_\ell\end{bmatrix}
=\sqrt{\pi_\ell}\left(\begin{bmatrix}
\widetilde{\mtx{\Sigma}}^2+\sigma^2\mtx{I} & \widetilde{\mtx{\Sigma}}\mtx{R}^T\sqrt{\vct{\pi}}\\
\left(\widetilde{\mtx{\Sigma}}\mtx{R}^T\sqrt{\vct{\pi}}\right)^T& 1
\end{bmatrix}\right)^{-1}
\begin{bmatrix}
\widetilde{\mtx{\Sigma}}\mtx{R}^T \vct{e}_\ell\\
\sqrt{\pi_\ell}
\end{bmatrix}
\end{align*}
This in turn implies that
\begin{align*}
\widehat{\vct{w}}_\ell=&\mtx{U}\mtx{U}^T\widehat{\vct{w}}_\ell=\sqrt{\pi_\ell}\mtx{U}\left(\widetilde{\mtx{\Sigma}}^2+\sigma^2\mtx{I} -\widetilde{\mtx{\Sigma}}\mtx{R}^T\sqrt{\vct{\pi}}\sqrt{\vct{\pi}}^T\mtx{R}\widetilde{\mtx{\Sigma}}\right)^{-1}\left(\widetilde{\mtx{\Sigma}}\mtx{R}^T\vct{e}_\ell-\sqrt{\pi_\ell}\widetilde{\mtx{\Sigma}}\mtx{R}^T\sqrt{\vct{\pi}}\right)\\
=&\sqrt{\pi_\ell}\mtx{U}\mtx{R}\widetilde{\mtx{\Sigma}}^{-1}\left(\mtx{I}+\sigma^2\widetilde{\mtx{\Sigma}}^{-2} -\sqrt{\vct{\pi}}\sqrt{\vct{\pi}}^T\right)^{-1}\mtx{R}\widetilde{\mtx{\Sigma}}^2\mtx{R}^T\left(\vct{e}_\ell-\sqrt{\pi_\ell}\sqrt{\vct{\pi}}\right)
\end{align*}
and
\begin{align*}
\widehat{b}_\ell=&\sqrt{\pi_\ell}\left(1-\sqrt{\vct{\pi}}^T\left(\mtx{I}+\sigma^2\widetilde{\mtx{\Sigma}}^{-2}\right)^{-1}\sqrt{\vct{\pi}}\right)^{-1}\left(1-\sqrt{\vct{\pi}}^T\left(\mtx{I}+\sigma^2\widetilde{\mtx{\Sigma}}^{-2}\right)^{-1}\vct{e}_\ell\right)%\\
%=&\pi_\ell\left(1-\vct{\pi}^T\left(\frac{1}{n}\mtx{I}+\sigma^2\mtx{\Sigma}^{-2}\right)^{-1}\vct{\pi}\right)^{-1}\left(1-\frac{\pi_\ell}{\frac{1}{n}+\frac{\sigma^2}{\sigma_\ell^2}}\right)
\end{align*}
FYI, Instead of using singular value decomposition of $\mtx{M}\mtx{Y}$ one can define things based on the matrix $\mtx{M}\text{diag}(\sqrt{\vct{\pi}})$ in which case the eigenvalue decomposition takes the form
\begin{align*}
\mtx{M}\text{diag}(\sqrt{\vct{\pi}})=\mtx{U}\widetilde{\mtx{\Sigma}}\mtx{R}^T
\end{align*}
%\section{temp}
%\begin{lemma}
%Let $\mtx{\Sigma}\succeq \mtx{0}$ be a diagonal PSD matrix. We have
%\begin{align*}
%\min_{\vct{x}:\text{ }\twonorm{\vct{x}}=1}\frac{1}{2}\twonorm{\mtx{\Sigma}\vct{x}-\vct{y}}^2=0
%\end{align*}
%which is equivalent to
%\begin{align*}
%\min_{\vct{x}:\text{ }\twonorm{\vct{x}}=1}\frac{1}{2}\twonorm{\mtx{\Sigma}\vct{x}-\vct{y}}^2=0
%\end{align*}
%\end{lemma}
%\begin{proof}
%Taking derivative with respect to $\vct{x}$ we arrive at
%\begin{align*}
%\mtx{\Sigma}\left(\mtx{\Sigma}\vct{x}-\vct{y}\right)+\lambda \vct{x}=0\quad\rightarrow\quad\widehat{\vct{x}}=\left(\mtx{\Sigma}^2+\lambda\mtx{I}\right)^{-1}\mtx{\Sigma}\vct{y}
%\end{align*}
%Thus we have to pick $\lambda$ so that
%\begin{align*}
%\sum_i \frac{\sigma_i^2 y_i^2}{\left(\sigma_i^2+\lambda\right)^2}=1
%\end{align*}
%\end{proof}


==> Proof_sketch.tex <==
\section{Proof outline for (weighted) least-squares:\\ key ideas and challenges}
%\subsection{Key ideas and challenges}
In this section, we provide a proof sketch for the analysis of the multiclass least-squares (LS) classifier. 

Specifically, we discuss our approach towards specifying the high-dimensional limits of the key quantities needed to evaluate the classification error:
$
\bb, \Sigmab_{\w,\mub},
$ and $ \Sigmab_{\w,\w}$.  We note that our proofs for the Weighted Least-Squares (WLS) classifiers follow the same general strategy, but in some parts require significantly more involved and intricate analysis and derivations. 

Our proofs follow the following general steps. See proof of each theorem for complete details and derivations.

\vp
\noindent\textbf{Step I: Decomposing the loss across classes.} Recall from Section \ref{classalg} that the multiclass LS classifier produces a linear classifier $\vct{x}\mapsto \mtx{W}\vct{x}+\vct{b}$ via a least-squares fit to the training data:
%\begin{align}
\begin{align}
(\Wh,\bh):=\frac{1}{2n}\fronorm{\mtx{W}\mtx{X}+\vct{b}\vct{1}_n^T-\mtx{Y}}^2.  \label{eq:LS_def_app}
\end{align}
Notice that the objective function above is separable. That is, 
\begin{align*}
\frac{1}{2n}\fronorm{\mtx{W}\mtx{X}+\vct{b}\vct{1}_n^T-\mtx{Y}}^2=\frac{1}{2n}\sum_{\ell=1}^k\twonorm{\mtx{X}^T\vct{w}_\ell+b_\ell\vct{1}_n-\mtx{Y}_\ell}^2.
\end{align*}
 Hence, for each $\ell\in[k]$, 
\bea
(\wh_\ell,\bh_\ell) = \arg\min_{\vct{w}_\ell, \vct{b}_\ell}\text{ }\frac{1}{2n}\twonorm{\mtx{X}^T\vct{w}_\ell+\bb_\ell\vct{1}_n-\mtx{Y}_\ell}^2. \label{eq:LS_sep}
\end{align}
This decomposition is convenient for analysis as it is easier to compute the statistical properties of the simple single-output LS in \eqref{eq:LS_sep} compared to the multi-output objective in \eqref{eq:LS_def_app}. Indeed, as we show, this simplification will eventually allow us to compute the high-dimensional behavior of the intercepts $\bh_\ell,~\ell\in[k]$, the mean-correlations $\inp{\wh_\ell}{\mub_c},~\ell,c\in[k]$, the norms $\twonorm{\wh_\ell},~\ell\in[k]$ and the LS training loss $ \twonorm{\mtx{X}^T\wh_\ell+\bh_\ell\vct{1}_n-\mtx{Y}_\ell}$. 

\vp\noindent\textbf{Step II: Reduction to an Auxiliary Optimization (AO) problem via CGMT.} To calculate the high-dimensional behavior \eqref{eq:LS_sep} we use the Convex Gaussian min-max Theorem (CGMT) \cite{StoLasso,COLT} framework. We provide a brief introduction of the CGMT machinery in Section \ref{sec:back_CGMT}. Roughly stated, this framework allows us to replace a \emph{Primary Optimization} (PO) problem of the form \eqref{eq:LS_sep} with an \emph{Auxiliary Optimization} (AO) problem that is simpler to analyze, but is predictive of the behavior of the latter. For instance, for the PO in \eqref{eq:LS_sep} in the GMM after some algebraic manipulations the AO problem takes the form
\begin{align}
\label{PFAO}
\frac{1}{2}\left(\min_{\vct{w}_\ell, \vct{b}_\ell}\text{ } \frac{1}{\sqrt{n}}\twonorm{ \sigma\twonorm{\vct{w}_\ell}\vct{g}+\mtx{Y}^T\mtx{M}^T\vct{w}_\ell+b_\ell\vct{1}_n-\mtx{Y}_\ell}+\frac{1}{\sqrt{n}}\sigma \vct{h}^T\vct{w}_\ell\right)_{+}^2,
\end{align}
where $(x)_{+}:=\max(0,x)$ and $\vct{g}\in\R^n$ and $\vct{h}\in\R^d$ are two independent Gaussian random vectors distributed as $\mathcal{N}(\vct{0},\mtx{I}_n)$ and $\mathcal{N}(\vct{0},\mtx{I}_d)$.

\vp\noindent\textbf{Step III: Simplification of the AO and computing $\mtx{\Sigma}_{\w,\mub}$ and $\vct{b}$.}
In this step we carry out a series of intricate calculations to further simplify \eqref{PFAO} and characterize its various asymptotic properties. In particular, in this step we compute the high-dimensional behavior of the intercepts $\bh_\ell,~\ell\in[k]$, the mean-correlations $\inp{\wh_\ell}{\mub_c},~\ell,c\in[k]$, the norms $\twonorm{\wh_\ell},~\ell\in[k]$ and the LS training loss $ \twonorm{\mtx{X}^T\wh_\ell+\bh_\ell\vct{1}_n-\mtx{Y}_\ell}$. For instance, for GMM these calculations allow us to conclude that
%\begin{subequations}
%\begin{align}\label{eq:LS_GM}
%\bh &\rP\diag{\pib}\left(\one_k+\left(\pib\one_k^T-\Iden_k\right)\Vb\Sigmab\Deltab^{-1}\Sigmab\Vb^T\pib \right)\\
%\Sigmab_{\w,\mub}& \rP -\Vb\Sigmab\Deltab^{-1}\Sigmab\Vb^T\left(\pib\one_k^T-\Iden_k\right) \\
%\Sigmab_{\w,\w} &\rP\frac{\gamma}{1-\gamma} \left(\diag{\pib}-\pib\pib^T\right) \nonumber\\
%&\quad\quad+ \diag{\pib}\left(\pib\one_k^T - \Iden_k\right)^T\Vb\Sigmab \Deltab^{-1} \left(\Deltab^{-1} + \frac{\gamma}{1-\gamma}\Iden_r\right) \Sigmab\Vb^T \left(\pib\one_k^T - \Iden_k\right) \diag{\pib}
%\end{align}
%\end{subequations}
%\MS{I think it should be
\begin{align*}
\bh &\rP\pib-\Pb\Vb\Sigmab\Deltab^{-1}\Sigmab\Vb^T\pib\,\quad\text{and}\quad
%\diag{\pib}\left(\one_k+\left(\pib\one_k^T-\Iden_k\right)\Vb\Sigmab\Deltab^{-1}\Sigmab\Vb^T\pib \right)\\
\Sigmab_{\w,\mub} \rP \Pb\Vb\Sigmab\Deltab^{-1}\Sigmab\Vb^T \,,
\end{align*}
where $
\Pb := \diag{\pib}-\pib\pib^T\succeq \zero_{k\times k}$ and $\Deltab:=\sigma^2\Iden_r + \Sigmab\Vb^T\Pb\Vb\Sigmab \succ \zero_{r\times r}.$

\vp\noindent\textbf{Step IV: Computing $\mtx{\Sigma}_{\w,\w}$ and capturing cross-correlations.}
The final and most involved part of our analysis is characterizing the asymptotic behavior of $\mtx{\Sigma}_{w,w}$. To see why this is particularly challenging note that the reduction from \eqref{eq:LS_def_app} to \eqref{eq:LS_sep} ``breaks" the dependence of all 
$\wh_1,\wh_2,\ldots,\wh_k$ on the \emph{same} feature matrix $\X$. Capturing this dependence is crucial in determining  the ``cross-correlations" $\inp{\wh_\ell}{\wh_c},~\ell\neq c$. As noted in Section \ref{sec:test} the matrix $\mtx{\Sigma}_{\w,\w}$ is needed to calculate the class-wise and total miss-classification errors. Unfortunately, the CGMT is \emph{not} directly applicable to the multi-output LS optimization in \eqref{eq:LS_def_app}. Our idea to circumvent this challenge builds on the following simple observation: the vector $\wh_{\ell,c} = \wh_\ell + \wh_c$ is itself the solution to another simple single-output LS problem.
\begin{lemma}\label{lem:joint_LS_sketch}
For $\ell\neq c\in[k]$, let $\wh_\ell$, $\wh_c$ be the $\ell$ and $c$-th row of $\widehat{\mtx{W}}$ which is the solution to the multi-output least-squares minimization \eqref{eq:LS_def_app}. Denote $\wh_{\ell,c}:=\wh_\ell+\wh_c$. Then, $\wh_{\ell,c}$ is a minimizer in the following single-output least-squares problem:
\begin{align}%\label{eq:joint_LS}
\wh_{\ell,c} = \arg\min_{\w, b} \frac{1}{2n}\twonorm{\Y_{\ell} + \Y_{c} - \X^T \w - b\one_n }^2\,.\nn
\end{align}
\end{lemma}
Thanks to Lemma \ref{lem:joint_LS_sketch}, we can use the CGMT to characterize the limiting behavior of $\twonorm{\wh_\ell+\wh_c}$. These calculations are similar to (but, in certain cases, such as for weighted least-squares, more involved than) those in Steps II and III above. Now note that an asymptotic characterization of $\twonorm{\wh_\ell+\wh_c}$ immediately yields the asymptotic characterization of $\inp{\wh_\ell}{\wh_c}$ as
\begin{align}\label{eq:inp_from_norms}
\inp{\wh_\ell}{\wh_c} = \frac{\twonorm{\wh_\ell+\wh_c}^2-\twonorm{\wh_\ell}^2-\twonorm{\wh_c}^2}{2},
\end{align} 
and $\twonorm{\wh_\ell}, \twonorm{\wh_c}$ are already computed in Step IV. For instance, for GMM the analysis in this step allow us to calculate the asymptotic behavior of $\mtx{\Sigma}_{w,w}$ as follows
\begin{align*}
\Sigmab_{\w,\w} &\rP\frac{\gamma}{(1-\gamma)\sigma^2} \Pb+ \Pb\Vb\Sigmab \Deltab^{-1} \Big(\Deltab^{-1} - \frac{\gamma}{(1-\gamma)\sigma^2}\Iden_r\Big) \Sigmab\Vb^T \Pb.
\end{align*}
%While other approaches, such as the use of  Random Matrix Theory (RMT) are possible here, we have found the CGMT approach rather convenient. Besides, while RMT is only directly applicable to closed-form estimators (such as LS), we believe that the CGMT approach can be extended to other instances such as the multi-class cross-entropy and SVM classifiers.

%After a brief introduction of the CGMT machinery in Section \ref{sec:back_CGMT}, we outline how to properly apply it to analyze the high-dimensional behavior of \eqref{eq:LS_sep}. As we will see the first crucial step is to properly choose an Auxiliary Optimization (AO) problem that is simpler to analyze than the Primary Optimization (PO) of interest in \eqref{eq:LS_sep}, but is predictive of the behavior of the latter. This is rather straightforward for the LS objective in \eqref{eq:LS_sep} \cite{StoLasso,OTH13,NIPS} and we outline the idea in Section \ref{sec:find_AO}. After properly identifying the AO, one needs to analyze its properties. The papers \cite{COLT,Master} have introduced a principled machinery for this purpose, but the details of the analysis are mostly problem-dependent. Specifically, the analysis of the AO for the multiclass setting is more involved compared to the corresponding analysis in the binary case. All the details are deferred to later sections in the Appendix; see Section \ref{sec:} for how they are organized. 

%The decomposition of the multiclass LS classifier into $k$ separable optimization problems as in \eqref{eq:LS_sep} conveniently allows the use of the CGMT as prescribed above.  However, a ``naive" application of the CGMT on the original optimization of the classifier does \emph{not} allow us to compute all the necessary correleations $\inp{\w_i}{\w_j},~i\neq j$ between the classfier's weights to precisely capture the total/class-wise errors. Instead, our key idea is to formulate an artificial optimization problem, which captures the missing correlations and at the same time conveniently allows us to leverage the CGMT. We explain how we tackle this challenge in Section \ref{sec:KKT_idea}.



\subsection{Background on CGMT}\label{sec:back_CGMT}

The CGMT is an extension of Gordon's Gaussian min-max inequality (GMT) \cite{Gor88}. In the context of high-dimensional inference problems, Gordon's inequality was first successfully used in the study oh sharp phase-transitions in noiseless Compressed Sensing \cite{Sto,Cha,TroppEdge,Sto}. More recently, \cite{StoLasso} (see also \cite[Sec.~10.3]{TroppEdge}) discovered that Gordon's inequality is essentially tight for certain convex problems. A concrete and general formulation of this idea was given by \cite{COLT} and was called the CGMT. 

%Next, we summarize the essential ideas of the CGMT \cite[Thm.~3]{COLT} (see also \cite[Section~6]{Master} for further details and the relation to Gordon's original inequality).

In order to summarize the essential ideas, consider the following two Gaussian processes:
\begin{subequations}\label{eq:POAO}
\begin{align}
X_{\w,\ub} &:= \ub^T \G \w + \psi(\w,\ub),\label{eq:PO_obj}\\
Y_{\w,\ub} &:= \twonorm{\w} \g^T \ub + \twonorm{\ub} \h^T \w + \psi(\w,\ub),\label{eq:AO_obj}
\end{align}
\end{subequations}
where: $\G\in\mathbb{R}^{n\times d}$, $\g \in \mathbb{R}^n$, $\h\in\mathbb{R}^d$, they all have entries iid Gaussian; the sets $\mathcal{S}_{\w}\subset\R^d$ and $\mathcal{S}_{\ub}\subset\R^n$ are compact; and, $\psi: \mathbb{R}^d\times \mathbb{R}^n \to \mathbb{R}$. For these two processes, define the following (random) min-max optimization programs, which are refered to as the \emph{primary optimization} (PO) problem and the \emph{auxiliary optimization} AO:
%
\begin{subequations}
\begin{align}\label{eq:PO_loc}
\Phi(\G)&=\min\limits_{\w \in \mathcal{S}_{\w}} \max\limits_{\ub\in\mathcal{S}_{\ub}} X_{\w,\ub},\\
%\end{equation}
%and
%\begin{equation}
\label{eq:AO_loc}
\phi(\g,\h)&=\min\limits_{\w \in \mathcal{S}_{\w}} \max\limits_{\ub\in\mathcal{S}_{\ub}} Y_{\w,\ub}.
\end{align}
\end{subequations}

%
%According to the CGMT
%\footnote{In fact, this is only a slight reformulation of Gordon's original comparison inequality \cite{Gor88}; see \cite{COLT}}, for any $c\in\R$, it holds:
%%
%\begin{equation}\label{eq:gmt}
%\mathbb{P}\left( \Phi(\G) < c\right) \leq 2 \mathbb{P}\left(  \phi(\g,\h) < c \right).
%\end{equation}
%%
%In other words, a high-probability lower bound on the AO is a high-probability lower bound on the PO. The premise is that it is often much simpler to lower bound the AO rather than the PO. 
%
%However, the real power of the CGMT comes in its second statement, which asserts that if the PO is \emph{convex} then the AO in  can be used to tightly infer properties of the original PO, including the optimal cost and the optimal solution.
%%We think of the two problems in \eqref{eq:PO_loc} and \eqref{eq:AO_loc} as random optimization problems, in which $\G$, $\g$ and $\h$ all have i.i.d standard normal entries. 
%More precisely, 
If the sets $\mathcal{S}_{\w}$ and $\mathcal{S}_{\ub}$ are convex and \emph{bounded}, and $\psi$ is continuous \emph{convex-concave} on $\mathcal{S}_{\w}\times \mathcal{S}_{\ub}$, then, for any $\nu \in \mathbb{R}$ and $t>0$, it holds
%
\begin{equation}\label{eq:cgmt}
\mathbb{P}\left( \abs{\Phi(\G)-\nu} > t\right) \leq 2\,\mathbb{P}\left(  \abs{\phi(\g,\h)-\nu} > t \right).
\end{equation}
%
In words, concentration of the optimal cost of the AO problem around $q^\ast$ implies concentration of the optimal cost of the corresponding PO problem around the same value $q^\ast$.  Asymptotically, if we can show that $\phi(\g,\h)\rP q^\ast$, then we can conclude that $\Phi(\G)\rP q^\ast$. Moreover, starting from \eqref{eq:cgmt} and under appropriate strict convexity conditions, the CGMT shows that concentration of the optimal solution of the AO problem implies concentration of the optimal solution of the PO around the same value. For example, if minimizers of \eqref{eq:AO_loc} satisfy $\twonorm{\w_\phi(\g,\h)} \rP \alpha^\ast$ for some $\alpha^\ast>0$, then, the same holds true for the minimizers of \eqref{eq:PO_loc}: $\twonorm{\w_\Phi(\G)} \rP \alpha^\ast$. Thus, one can analyze the AO to infer corresponding properties of the PO, the premise being of course that the former is simpler to handle than the latter. 

In \cite{Master}, the authors introduce a principled machinery that allows to (a) express a quite general family of convex inference optimization problems  in the form of the PO and (b) simplify the AO from a (random) optimization over vector variables to an easier optimization over only few scalar variables, termed the ``\emph{scalarized AO}".






%\subsection{Computing $\Sigma_{w,\mu}$ and $b$: CGMT on the separable optimization problem}
%Notice that the objective function of the LS classifier is separable: $\frac{1}{2n}\fronorm{\mtx{W}\mtx{X}+\vct{b}\vct{1}_n^T-\mtx{Y}}^2=\frac{1}{2n}\twonorm{\mtx{X}^T\vct{w}_\ell+b_\ell\vct{1}_n-\mtx{Y}_\ell}^2 $. Hence, for each $\ell\in[k]$, 
%\bea
%(\wh_\ell,\bh_\ell) = \arg\min_{\vct{w}_\ell, \vct{b}_\ell}\text{ }\frac{1}{2n}\twonorm{\mtx{X}^T\vct{w}_\ell+\bb_\ell\vct{1}_n-\mtx{Y}_\ell}^2. \label{eq:LS_sep}
%\end{align}
%This decomposition is convenient for analysis as it is easier to compute the statistical properties of the simple single-output LS in \eqref{eq:LS_sep} compared to the multi-output objective in \eqref{eq:LS_def}. Indeed, this reduction suffices to compute the limiting behavior of the intercepts $\bh_\ell,~\ell\in[k]$, the mean-correlations $\inp{\wh_\ell}{\mub_c},~\ell,c\in[k]$, the norms $\twonorm{\wh_\ell},~\ell\in[k]$ and the LS training loss $ \twonorm{\mtx{X}^T\wh_\ell+\bh_\ell\vct{1}_n-\mtx{Y}_\ell}$. For this analysis, we use the Convex Gaussian min-max Theorem (CGMT) \cite{StoLasso,COLT}. While other approaches, such as the use of  Random Matrix Theory (RMT) are possible, we have found the CGMT approach rather convenient. Besides, while RMT is only directly applicable to closed-form estimators (such as LS), we believe that the CGMT approach can be extended to other instances such as the multi-class cross-entropy and SVM classifiers.






==> Proof_sketchold.tex <==
\section{Proof strategy for least-squares: key ideas and challenges}
%\subsection{Key ideas and challenges}
In this section, we provide a proof sketch for the analysis of the multiclass least-squares (LS) classifier. 

Specifically, we discuss our approach towards specifying the high-dimensional limits of the key quantities needed to evaluate the classification error:
$
\bb, \Sigmab_{\w,\mub},
$ and $ \Sigmab_{\w,\w}$. 
 Recall from Section \ref{classalg} that the the multiclass LS classifier produces a linear classifier $\vct{x}\mapsto \mtx{W}\vct{x}+\vct{b}$ via a least-squares fit to the training data:
%\begin{align}
\begin{align}
(\Wh,\bh):=\frac{1}{2n}\fronorm{\mtx{W}\mtx{X}+\vct{b}\vct{1}_n^T-\mtx{Y}}^2.  \label{eq:LS_def_app}
\end{align}
Notice that the objective function above is separable: $\frac{1}{2n}\fronorm{\mtx{W}\mtx{X}+\vct{b}\vct{1}_n^T-\mtx{Y}}^2=\frac{1}{2n}\twonorm{\mtx{X}^T\vct{w}_\ell+b_\ell\vct{1}_n-\mtx{Y}_\ell}^2 $. Hence, for each $\ell\in[k]$, 
\bea
(\wh_\ell,\bh_\ell) = \arg\min_{\vct{w}_\ell, \vct{b}_\ell}\text{ }\frac{1}{2n}\twonorm{\mtx{X}^T\vct{w}_\ell+\bb_\ell\vct{1}_n-\mtx{Y}_\ell}^2. \label{eq:LS_sep}
\end{align}
This decomposition is convenient for analysis as it is easier to compute the statistical properties of the simple single-output LS in \eqref{eq:LS_sep} compared to the multi-output objective in \eqref{eq:LS_def_app}. Indeed, as we show, this simplification allows to compute the high-dimensional behavior of the intercepts $\bh_\ell,~\ell\in[k]$, the mean-correlations $\inp{\wh_\ell}{\mub_c},~\ell,c\in[k]$, the norms $\twonorm{\wh_\ell},~\ell\in[k]$ and the LS training loss $ \twonorm{\mtx{X}^T\wh_\ell+\bh_\ell\vct{1}_n-\mtx{Y}_\ell}$. For this analysis, we use the Convex Gaussian min-max Theorem (CGMT) \cite{StoLasso,COLT} framework. We provide a brief introduction of the CGMT machinery in Section \ref{sec:back_CGMT}.



%While other approaches, such as the use of  Random Matrix Theory (RMT) are possible here, we have found the CGMT approach rather convenient. Besides, while RMT is only directly applicable to closed-form estimators (such as LS), we believe that the CGMT approach can be extended to other instances such as the multi-class cross-entropy and SVM classifiers.

After a brief introduction of the CGMT machinery in Section \ref{sec:back_CGMT}, we outline how to properly apply it to analyze the high-dimensional behavior of \eqref{eq:LS_sep}. As we will see the first crucial step is to properly choose an Auxiliary Optimization (AO) problem that is simpler to analyze than the Primary Optimization (PO) of interest in \eqref{eq:LS_sep}, but is predictive of the behavior of the latter. This is rather straightforward for the LS objective in \eqref{eq:LS_sep} \cite{StoLasso,OTH13,NIPS} and we outline the idea in Section \ref{sec:find_AO}. After properly identifying the AO, one needs to analyze its properties. The papers \cite{COLT,Master} have introduced a principled machinery for this purpose, but the details of the analysis are mostly problem-dependent. Specifically, the analysis of the AO for the multiclass setting is more involved compared to the corresponding analysis in the binary case. All the details are deferred to later sections in the Appendix; see Section \ref{sec:} for how they are organized. 

The decomposition of the multiclass LS classifier into $k$ separable optimization problems as in \eqref{eq:LS_sep} conveniently allows the use of the CGMT as prescribed above.  However, a ``naive" application of the CGMT on the original optimization of the classifier does \emph{not} allow us to compute all the necessary correleations $\inp{\w_i}{\w_j},~i\neq j$ between the classfier's weights to precisely capture the total/class-wise errors. Instead, our key idea is to formulate an artificial optimization problem, which captures the missing correlations and at the same time conveniently allows us to leverage the CGMT. We explain how we tackle this challenge in Section \ref{sec:KKT_idea}.

\subsection{Background: The CGMT}\label{sec:back_CGMT}

The CGMT is an extension of Gordon's Gaussian min-max inequality (GMT) \cite{Gor88}. In the context of high-dimensional inference problems, Gordon's inequality was first successfully used in the study oh sharp phase-transitions in noiseless Compressed Sensing \cite{Sto,Cha,TroppEdge,Sto,TroppUniversal}. More recently, \cite{StoLasso} (see also \cite[Sec.~10.3]{TroppEdge}) discovered that Gordon's inequality is essentially tight for certain convex problems. A concrete and general formulation of this idea was given by \cite{COLT} and was called the CGMT. 

%Next, we summarize the essential ideas of the CGMT \cite[Thm.~3]{COLT} (see also \cite[Section~6]{Master} for further details and the relation to Gordon's original inequality).

In order to summarize the essential ideas, consider the following two Gaussian processes:
\begin{subequations}\label{eq:POAO}
\begin{align}
X_{\w,\ub} &:= \ub^T \G \w + \psi(\w,\ub),\\
Y_{\w,\ub} &:= \twonorm{\w} \g^T \ub + \twonorm{\ub} \h^T \w + \psi(\w,\ub),\label{eq:AO_obj}
\end{align}
\end{subequations}
where: $\G\in\mathbb{R}^{n\times d}$, $\g \in \mathbb{R}^n$, $\h\in\mathbb{R}^d$, they all have entries iid Gaussian; the sets $\mathcal{S}_{\w}\subset\R^d$ and $\mathcal{S}_{\ub}\subset\R^n$ are compact; and, $\psi: \mathbb{R}^d\times \mathbb{R}^n \to \mathbb{R}$. For these two processes, define the following (random) min-max optimization programs, which are refered to as the \emph{primary optimization} (PO) problem and the \emph{auxiliary optimization} AO:
%
\begin{subequations}
\begin{align}\label{eq:PO_loc}
\Phi(\G)&=\min\limits_{\w \in \mathcal{S}_{\w}} \max\limits_{\ub\in\mathcal{S}_{\ub}} X_{\w,\ub},\\
%\end{equation}
%and
%\begin{equation}
\label{eq:AO_loc}
\phi(\g,\h)&=\min\limits_{\w \in \mathcal{S}_{\w}} \max\limits_{\ub\in\mathcal{S}_{\ub}} Y_{\w,\ub}.
\end{align}
\end{subequations}

%
%According to the CGMT
%\footnote{In fact, this is only a slight reformulation of Gordon's original comparison inequality \cite{Gor88}; see \cite{COLT}}, for any $c\in\R$, it holds:
%%
%\begin{equation}\label{eq:gmt}
%\mathbb{P}\left( \Phi(\G) < c\right) \leq 2 \mathbb{P}\left(  \phi(\g,\h) < c \right).
%\end{equation}
%%
%In other words, a high-probability lower bound on the AO is a high-probability lower bound on the PO. The premise is that it is often much simpler to lower bound the AO rather than the PO. 
%
%However, the real power of the CGMT comes in its second statement, which asserts that if the PO is \emph{convex} then the AO in  can be used to tightly infer properties of the original PO, including the optimal cost and the optimal solution.
%%We think of the two problems in \eqref{eq:PO_loc} and \eqref{eq:AO_loc} as random optimization problems, in which $\G$, $\g$ and $\h$ all have i.i.d standard normal entries. 
%More precisely, 
if the sets $\mathcal{S}_{\w}$ and $\mathcal{S}_{\ub}$ are convex and \emph{bounded}, and $\psi$ is continuous \emph{convex-concave} on $\mathcal{S}_{\w}\times \mathcal{S}_{\ub}$, then, for any $\nu \in \mathbb{R}$ and $t>0$, it holds
%
\begin{equation}\label{eq:cgmt}
\mathbb{P}\left( \abs{\Phi(\G)-\nu} > t\right) \leq 2 \mathbb{P}\left(  \abs{\phi(\g,\h)-\nu} > t \right).
\end{equation}
%
In words, concentration of the optimal cost of the AO problem around $q^\ast$ implies concentration of the optimal cost of the corresponding PO problem around the same value $q^\ast$.  Asymptotically, if we can show that $\phi(\g,\h)\rP q^\ast$, then we can conclude that $\Phi(\G)\rP q^\ast$. Moreover, starting from \eqref{eq:cgmt} and under appropriate strict convexity conditions, the CGMT shows that concentration of the optimal solution of the AO problem implies concentration of the optimal solution of the PO around the same value. For example, if minimizers of \eqref{eq:AO_loc} satisfy $\twonorm{\w_\phi(\g,\h)} \rP \alpha^\ast$ for some $\alpha^\ast>0$, then, the same holds true for the minimizers of \eqref{eq:PO_loc}: $\twonorm{\w_\Phi(\G)} \rP \alpha^\ast$. Thus, one can analyze the AO to infer corresponding properties of the PO, the premise being of course that the former is simpler to handle than the latter. In \cite{Master}, the authors introduce a principled machinery that allows to (a) express a quite general family of convex inference optimization problems  in the form of the PO and (b) simplify the AO from a (random) optimization over vector variables to an easier optimization over only few scalar variables, termed the ``scalarized AO".






\subsection{Computing $\Sigma_{w,\mu}$ and $b$: CGMT on the separable optimization problem}
%Notice that the objective function of the LS classifier is separable: $\frac{1}{2n}\fronorm{\mtx{W}\mtx{X}+\vct{b}\vct{1}_n^T-\mtx{Y}}^2=\frac{1}{2n}\twonorm{\mtx{X}^T\vct{w}_\ell+b_\ell\vct{1}_n-\mtx{Y}_\ell}^2 $. Hence, for each $\ell\in[k]$, 
%\bea
%(\wh_\ell,\bh_\ell) = \arg\min_{\vct{w}_\ell, \vct{b}_\ell}\text{ }\frac{1}{2n}\twonorm{\mtx{X}^T\vct{w}_\ell+\bb_\ell\vct{1}_n-\mtx{Y}_\ell}^2. \label{eq:LS_sep}
%\end{align}
%This decomposition is convenient for analysis as it is easier to compute the statistical properties of the simple single-output LS in \eqref{eq:LS_sep} compared to the multi-output objective in \eqref{eq:LS_def}. Indeed, this reduction suffices to compute the limiting behavior of the intercepts $\bh_\ell,~\ell\in[k]$, the mean-correlations $\inp{\wh_\ell}{\mub_c},~\ell,c\in[k]$, the norms $\twonorm{\wh_\ell},~\ell\in[k]$ and the LS training loss $ \twonorm{\mtx{X}^T\wh_\ell+\bh_\ell\vct{1}_n-\mtx{Y}_\ell}$. For this analysis, we use the Convex Gaussian min-max Theorem (CGMT) \cite{StoLasso,COLT}. While other approaches, such as the use of  Random Matrix Theory (RMT) are possible, we have found the CGMT approach rather convenient. Besides, while RMT is only directly applicable to closed-form estimators (such as LS), we believe that the CGMT approach can be extended to other instances such as the multi-class cross-entropy and SVM classifiers.


\subsection{Computing $\Sigma_{w,w}$: Capturing cross-correlations via KKT}\label{sec:KKT_idea}

However, note that the reduction from \eqref{eq:LS_def} to \eqref{eq:LS_sep} ``breaks" the dependence of all 
$\wh_1,\wh_2,\ldots,\wh_k$ on the \emph{same} feature matrix $\X$. Capturing this dependence is crucial in determining  the ``cross-correlations" $\inp{\wh_\ell}{\wh_c},~\ell\neq c$. As noted in Section \ref{sec:test} the matrix $\Sigma_{\w,\w}$ enters the calculations of our end objective: the classification error of \eqref{eq:LS_def}. Unfortunately, the CGMT is \emph{not} directly applicable to the multi-output LS optimization in \eqref{eq:LS_def}. Our idea to circumvent this challenge builds on the following simple observation: the vector $\wh_{\ell,c} = \wh_\ell + \wh_c$ is itself the solution to another simple single-output LS problem.
\begin{lemma}\label{lem:joint_LS}
For $\ell\neq c\in[k]$ let $\wh_\ell$, $\wh_j$ be solutions to the multi-output least-squares minimization \eqref{eq:LS_def}. Denote $\wh_{\ell,c}:=\wh_\ell+\wh_c$. Then, $\wh_{\ell,c}$ is a minimizer in the following single-output least-squares problem:
\begin{align}\label{eq:joint_LS}
\wh_{\ell,j} = \arg\min_{\w, b} \frac{1}{2n}\twonorm{\Y_{\ell} + \Y_{j} - \X^T \w - b\one_n }^2
\end{align}
\end{lemma}
Thanks to Lemma \ref{lem:joint_LS}, we can use the CGMT to characterize the limiting behavior of $\twonorm{\wh_\ell+\wh_c}$. Observe that this immediately gives the limit of $\inp{\wh_\ell}{\wh_c}$ since 
\begin{align}\label{eq:inp_from_norms}
\inp{\wh_\ell}{\wh_c} = \frac{\twonorm{\wh_\ell+\wh_c}^2-\twonorm{\wh_\ell}^2-\twonorm{\wh_c}^2}{2},
\end{align} 
and $\twonorm{\wh_\ell}, \twonorm{\wh_c}$ are already computed from \eqref{eq:LS_sep}.





==> WLS_GM.tex <==
\subsection{Weighted least-squares classifier}
\label{GMWLS}
We now focus on characterizing the intercepts/correlation matrices for the WLS classifier.
% and again assume the Grammian matrix has eigenvalue decomposition $\Sigmab_{\mub,\mub}=\Vb\Sigmab^2\Vb^T$.


%{\color{blue}Need to change notation for rank of $\M^T\M$ to something else other than $r$, which is reserved for signal energies}
%\subsubsection{Underparameterized regime}
\begin{theorem}\label{thm:WLS_GM}
Consider data generated according to GMM and $\gamma<1$. Consider a weighted LS classifier with weights $\mtx{D}=\diag{\omega_1,\ldots,\omega_k}$ and let $\eta$ be the unique solution to $\sum_{\ell=1}^k \frac{\pi_\ell \omega_\ell^2}{\omega_\ell^2+\eta}=\gamma$.
Also define
$
\Pb := \diag{\widetilde{\pib}}-\widetilde{\pib}\widetilde{\pib}^T\succeq \zero_{k\times k}$ and $\Deltab:=\sigma^2\Iden_r + \Sigmab\Vb^T\Pb\Vb\Sigmab \succ \zero_{r\times r}$ with the entries of $\widetilde{\pib}$ given by $\widetilde{\pi}_\ell=\frac{1}{\gamma}\frac{\pi_\ell \omega_\ell^2}{\omega_\ell^2+\eta}$. Then, for the WLS linear classifier $\left(\Wh,\bh\right)$ the following asymptotic limits hold
%\begin{subequations}
%\begin{align}\label{eq:LS_GM}
%\bh &\rP\diag{\pib}\left(\one_k+\left(\pib\one_k^T-\Iden_k\right)\Vb\Sigmab\Deltab^{-1}\Sigmab\Vb^T\pib \right)\\
%\Sigmab_{\w,\mub}& \rP -\Vb\Sigmab\Deltab^{-1}\Sigmab\Vb^T\left(\pib\one_k^T-\Iden_k\right) \\
%\Sigmab_{\w,\w} &\rP\frac{\gamma}{1-\gamma} \left(\diag{\pib}-\pib\pib^T\right) \nonumber\\
%&\quad\quad+ \diag{\pib}\left(\pib\one_k^T - \Iden_k\right)^T\Vb\Sigmab \Deltab^{-1} \left(\Deltab^{-1} + \frac{\gamma}{1-\gamma}\Iden_r\right) \Sigmab\Vb^T \left(\pib\one_k^T - \Iden_k\right) \diag{\pib}
%\end{align}
%\end{subequations}
%\MS{I think it should be
\begin{subequations}
\begin{align}\label{eq:WLS_GM}
\bh &\rP\widetilde{\pib}-\Pb\Vb\Sigmab\Deltab^{-1}\Sigmab\Vb^T\widetilde{\pib}\,,\quad
%\diag{\pib}\left(\one_k+\left(\pib\one_k^T-\Iden_k\right)\Vb\Sigmab\Deltab^{-1}\Sigmab\Vb^T\pib \right)\\
\Sigmab_{\w,\mub} \rP \Pb\Vb\Sigmab\Deltab^{-1}\Sigmab\Vb^T \,,\\
\Sigmab_{\w,\w} &\rP\frac{\zeta}{\sigma^2} \Pb+ \Pb\Vb\Sigmab \Deltab^{-1} \Big(\Deltab^{-1} - \frac{\zeta}{\sigma^2}\Iden_r\Big) \Sigmab\Vb^T \Pb+\frac{\eta\zeta}{\sigma^2}\mtx{Q}\,.
\end{align}
\end{subequations}
Here, $\zeta:={\gamma}\big/{\left(\eta \,\sum_{\ell=1}^k\frac{\pi_\ell\omega_\ell^2}{(\omega_\ell^2+\eta)^2}\right)}$ and $\mtx{Q}\in\R^{k\times k}$ is a known matrix depending on various problem parameters. Its precise value is given in \eqref{eq:Qmat_app}.%depends on problem parameters and is precisely specified in the supplementary.
%}
%  $\Wh^T=\begin{bmatrix}\vct{w}_1 &\vct{w}_2 &\cdots &\vct{w}_k \end{bmatrix}
%\in\R^{d\times k}$ and $\bb=\begin{bmatrix} b_1 & b_2 & \ldots & b_k \end{bmatrix}^T$ 
% in the high-asymptotic regime $n,d\rightarrow\infty, d/n\rightarrow\gamma.$
%\begin{align}
%$\bh\rP \betab,$  $\Sigmab_{\w,\mub} \rP \Sb_{\w,\mub}$ and $\Sigmab_{\w,\w} \rP \Sb_{\w\w}.$ In particular, the limiting value of the classification error can be computed by substituting these in \eqref{eq:Pe_GMM_gen}.
%\end{align}

%Moreover, for a fresh data sample $(\x\in\R^d,y\in[k])$ the test error probability $\P_e=\P\left(\arg\max_{c\in[k]}\inp{\w}{\x}\neq y\right)$ converges to the following limit
%\begin{align}
%\P_e \rP \P\left( \arg\max_{c\in[k]}\left\{G_c+\betab_c + \eb_c^T\Sigma_{\w,\mub}\eb_Y\right\} \neq Y \right),
%\end{align}
%where $\Pr(Y=i)=\pi_i,~i\in[k]$ and $\begin{bmatrix}G_1,\ldots,G_k\end{bmatrix}\sim\Nn\left(\zero,\Sigma_{\w,\w}\right)$.
\end{theorem} 
%The above result allows us to precisely characterize the class-wise/total test accuracy for WLS. 
Surprisingly, the effect of the weights is essentially equivalent to adjusting the class priors from $\vct{\pi}$ to $\widetilde{\vct{\pi}}$ defined in the theorem (modulo the extra additive term in the cross correlation matrix $\Sigmab_{\w,\w} $). This shows that weighted LS has similar performance to an un-weighted LS applied to a model with different class priors $\widetilde{\vct{\pi}}$. This characterization allows us to precisely understand how different weighting schemes can alter test accuracy for rare/minority classes.

%\begin{remark}If the Gram matrix $\M^T\M$ is invertible and letting $F:=\left(\M^T\M\right)^{-1}+\diag{\pi}$ the expressions in \eqref{eq:LS_GM} simplify as follows:
%....
%\end{remark}
%  From those simpler formulae, it can be checked that 

%It can be readily checked from Proposition \ref{thm:ave_GM} that when means are orthogonal, the solutions $\wh_i, i\in[k]$ of the class averaging classifier are also (asymptotically) orthogonal. However, Corollary \ref{cor:LS_ortho} shows that this is not the case for the LS classifier. We show next that these spurious correlations hurt the classification error. Specifically, directly comparing \eqref{eq:uls} to \eqref{eq:G0_ave}, it can be seen that $$u_{LS} = u_{ave}\sqrt{1-\gamma}\,<\,u_{ave}\Longrightarrow \P_{e,\rm ave} < \P_{e,\rm LS}\,,$$ for all values of $k, 0<\gamma< 1$ and $\mu^2$. Thus, for orthogononal means of equal energy and balanced classes, \emph{the averaging estimator strictly outperforms LS for all $0<\gamma< 1$ and $k\geq 2$.}


%\begin{figure}[t]
%\begin{center}
%\includegraphics[width=.9\textwidth]{Example.eps}
%\end{center}
%\caption{Test error of LS vs averaging method for equal-prior, equal-energy and orthogonal means. Here $k=4$, $r^2=5$, $d=125$ and averaging over 25 realizations.}
%\end{figure}


%\noindent\textbf{Equal energy \& equal priors.}~~Further assume that $r_i=r, \forall i\in[k]$ and $\pi_i=\pi=1/k,\forall i\in[k]$.  In this case,
%$
%\P\left( \text{error} \,|\, \y = \e_c \right) = 1 - \P\left( \Sb_c^{{1}/{2}}\, \z > \tb \right),
%$
%with 
%$$\Sb_c=\frac{\pi}{1+\pi r^2}\left(\frac{\pi r^2}{1+\pi r^2}+\frac{\gamma}{1-\gamma}\right)(\Id + \one\one^T)
%\qquad\text{and}\qquad
%\tb = -\frac{\pi r^2}{1+\pi r^2}\one.
%$$ 
%Thus, setting 
%\bea\label{eq:uls}
%u_{\rm LS}:=r^2\sqrt{ \frac{\pi}{ \pi r^2 + \left(\frac{\gamma}{1-\gamma}\right) \left({1+\pi r^2}\right)}}=r^2\sqrt{ \frac{1-\gamma}{r^2+\gamma/\pi}},
%\end{align}
% the probability of error is given by:
%$$
%\P_e = \P\left(  G_0 + \max_{j\in[k-1]} G_j \geq u_{\rm LS} \right),\quad G_0,G_1,\ldots,G_{k-1}\simiid\Nn(0,1)\,.
%$$
%%The union bound \eqref{eq:UB} gives:
%%\bea
%%\P_e = \P_c \leq (k-1) \cdot Q\left( \frac{u_{\rm LS}}{\sqrt{2}} \right) %= (k-1) \cdot Q\left( \frac{r}{\sqrt{2\left(1+\frac{\gamma k}{ r^2}\right)}} \right)
%%\end{align}
%Directly comparing \eqref{eq:uls} to \eqref{eq:uave}, it can be seen that $$u_{LS} = u_{ave}\sqrt{1-\gamma}\,<\,u_{ave}\Longrightarrow \P_{c,\rm ave} < \P_{c,\rm LS}\,,$$ for all values of $k, \gamma<1$ and $r^2$. Thus, for orthogononal means of equal energy and balanced classes, \emph{the averaging estimator strictly outperforms LS for all $\gamma<1$ and $k\geq 2$.}





==> WLS_GMMBackup.tex <==
\section{Fixed Weighted}

\begin{align*}
\underset{\mtx{W}\in\R^{k\times d},\text{ }\vct{b}\in\R^k}{\min}\quad \frac{1}{2n}\fronorm{\left(\mtx{W}\mtx{X}+\vct{b}\vct{1}_n^T-\mtx{Y}\right)\mtx{D}}^2=&\sum_{\ell=1}^k \min_{\vct{w}_\ell, \vct{b}_\ell}\text{ }\frac{1}{2n}\twonorm{\mtx{D}\left(\mtx{X}^T\vct{w}_\ell+b_\ell\vct{1}_n-\mtx{Y}_\ell\right)}^2\\
=&\sum_{\ell=1}^k \min_{\vct{w}_\ell, \vct{b}_\ell}\text{ }\frac{1}{2n}\twonorm{\mtx{D}\left(\mtx{Y}^T\mtx{M}^T\vct{w}_\ell+ \mtx{Z}^T\vct{w}_\ell+b_\ell\vct{1}_n-\mtx{Y}_\ell\right)}^2
\end{align*}

Define 
\begin{align}
\mathcal{L}_{PO}\left(\vct{w}_\ell,b_\ell\right):=\frac{1}{2n}\twonorm{\mtx{D}\left(\mtx{Y}^T\mtx{M}^T\vct{w}_\ell+ \mtx{Z}^T\vct{w}_\ell+b_\ell\vct{1}_n-\mtx{Y}_\ell\right)}^2\label{eq:LS_PO}
\end{align}


\noindent\textbf{Identifying the AO.}~~To continue further note that by duality we have
\begin{align*}
\min_{\vct{w}_\ell, \vct{b}_\ell}\text{ }\mathcal{L}_{PO}\left(\vct{w}_\ell,b_\ell\right) =&\min_{\vct{u}, \vct{w}_\ell, \vct{b}_\ell}\text{ }\max_{\vct{s}}\text{ }\frac{1}{n}\left(\vct{s}^T\mtx{D}\mtx{Y}^T\mtx{M}^T\vct{w}_\ell+ \vct{s}^T\mtx{D}\mtx{Z}^T\vct{w}_\ell+b_\ell\vct{s}^T\mtx{D}\vct{1}_n-\vct{s}^T\mtx{D}\mtx{Y}_\ell-\vct{s}^T\vct{u}+\frac{\twonorm{\vct{u}}^2}{2}\right)%\\
%=&\min_{\vct{w}_\ell, \vct{b}_\ell}\text{ }\max_{\vct{s}}\text{ }\frac{1}{n}\left(\vct{s}^T\mtx{Y}^T\mtx{M}^T\vct{w}_\ell+ \vct{s}^T\mtx{Z}^T\vct{w}_\ell+b_\ell\vct{s}^T\vct{1}_n-\vct{s}^T\mtx{Y}_\ell-\frac{\twonorm{\mtx{D}^{-1}\vct{s}}^2}{2}\right)
\end{align*}
Note that the above is jointly convex in $(\vct{u}, \vct{w}_\ell, b_\ell)$ and concave in $\vct{s}$. We consider the Auxiliary Optimization (AO) problem
\begin{align*}
\min_{\vct{u},\vct{w}_\ell, \vct{b}_\ell}\text{ }\max_{\vct{s}}\text{ }\frac{1}{n}\left(\vct{s}^T\mtx{D}\mtx{Y}^T\mtx{M}^T\vct{w}_\ell+ \sigma\twonorm{\vct{w}_\ell}\vct{g}^T\mtx{D}\vct{s}+ \sigma\twonorm{\mtx{D}\vct{s}}\vct{h}^T\vct{w}_\ell+b_\ell\vct{s}^T\mtx{D}\vct{1}_n-\vct{s}^T\mtx{D}\mtx{Y}_\ell-\vct{s}^T\vct{u}+\frac{\twonorm{\vct{u}}^2}{2}\right),
\end{align*}
where $\vct{g}\in\R^n$ and $\vct{h}\in\R^d$ are independent Gaussian random vectors with i.i.d.~$\mathcal{N}(0,1)$ entries. To continue further we carry out a change of variable $\vct{s}\rightarrow \mtx{D}\vct{s}$ to arrive at
\begin{align*}
\min_{\vct{u},\vct{w}_\ell, \vct{b}_\ell}\text{ }\max_{\vct{s}}\text{ }\frac{1}{n}\left(\vct{s}^T\mtx{Y}^T\mtx{M}^T\vct{w}_\ell+ \sigma\twonorm{\vct{w}_\ell}\vct{g}^T\vct{s}+ \sigma\twonorm{\vct{s}}\vct{h}^T\vct{w}_\ell+b_\ell\vct{s}^T\vct{1}_n-\vct{s}^T\mtx{Y}_\ell-\vct{s}^T\mtx{D}^{-1}\vct{u}+\frac{\twonorm{\vct{u}}^2}{2}\right),
\end{align*}
Maximizing over the direction of $\vct{s}$ and its norm $\beta=\twonorm{\vct{s}}$ we arrive at
\begin{align*}
&\min_{\vct{u},\vct{w}_\ell, \vct{b}_\ell}\text{ }\max_{\beta\ge 0}\text{ }\max_{\vct{s}: \twonorm{\vct{s}}=1}\text{ }\frac{1}{n}\left(\beta\vct{s}^T\mtx{Y}^T\mtx{M}^T\vct{w}_\ell+ \sigma\beta\twonorm{\vct{w}_\ell}\vct{g}^T\vct{s}+ \sigma\beta\vct{h}^T\vct{w}_\ell+b_\ell\beta\vct{s}^T\vct{1}_n-\beta\vct{s}^T\mtx{Y}_\ell-\beta\vct{s}^T\mtx{D}^{-1}\vct{u}+\frac{\twonorm{\vct{u}}^2}{2}\right)\\
&\quad\quad=\min_{\vct{u},\vct{w}_\ell, \vct{b}_\ell}\text{ }\max_{\beta\ge 0}\text{ }\frac{1}{n}\left(\beta\twonorm{\mtx{Y}^T\mtx{M}^T\vct{w}_\ell+ \sigma\twonorm{\vct{w}_\ell}\vct{g}+b_\ell\vct{1}_n-\mtx{Y}_\ell-\mtx{D}^{-1}\vct{u}}+ \sigma\beta\vct{h}^T\vct{w}_\ell+\frac{\twonorm{\vct{u}}^2}{2}\right)\\
&\quad\quad=\min_{\vct{u}, \vct{b}_\ell}\text{ }\max_{\beta\ge 0}\text{ }\min_{\vct{w}_\ell}\text{ }\frac{1}{n}\left(\beta\twonorm{\mtx{Y}^T\mtx{M}^T\vct{w}_\ell+ \sigma\twonorm{\vct{w}_\ell}\vct{g}+b_\ell\vct{1}_n-\mtx{Y}_\ell-\mtx{D}^{-1}\vct{u}}+ \sigma\beta\vct{h}^T\vct{w}_\ell+\frac{\twonorm{\vct{u}}^2}{2}\right)
\end{align*}
To continue, consider the singular value decomposition  
\begin{align}\label{eq:M_SVD}
\mtx{M}=\mtx{U}\mtx{\Sigma}\mtx{V}^T = 
\begin{bmatrix}\ub_1 & \ub_2 & \ldots & \ub_r \end{bmatrix} \diag{\sigma_1,\sigma_2,\ldots,\sigma_r} \begin{bmatrix}\vb^T_1 \\ \vb_2^T \\ \ldots \\ \vb_r^T \end{bmatrix} ,
\end{align}
with $r:=rank(\mtx{M})\le k$ and define the variable $\vct{\alpha}=\mtx{U}^T\vct{w}_\ell$ and $\vct{\alpha}_{\perp}=\mtx{U}_{\perp}^T\vct{w}_\ell$ where $\mtx{U}_{\perp}$ is the orthogonal complement of the columns of $\mtx{U}$. With these definitions the above optimization problem reduces to
\begin{align*}
\min_{\vct{u}, \vct{b}_\ell}\text{ }\max_{\beta\ge 0}\text{ }\min_{\vct{\alpha}}\text{ }\min_{\vct{\alpha}_\perp}\text{ }\frac{1}{n}\left(\beta\twonorm{\mtx{Y}^T\mtx{V}\mtx{\Sigma}\vct{\alpha}+ \sigma\sqrt{\twonorm{\vct{\alpha}}^2+\twonorm{\vct{\alpha}_\perp}^2}\vct{g}+b_\ell\vct{1}_n-\mtx{Y}_\ell-\mtx{D}^{-1}\vct{u}}+ \sigma\beta\vct{h}^T\mtx{U}\vct{\alpha}+ \sigma\beta\vct{h}^T\mtx{U}_{\perp}\vct{\alpha}_{\perp}+\frac{\twonorm{\vct{u}}^2}{2}\right)
\end{align*}
Decomposing the optimization over $\vct{\alpha}_\perp$ in terms of its direction and norm $\alpha_0=\twonorm{\vct{\alpha}_\perp}$ we arrive at
\begin{align*}
\min_{\vct{u}, \vct{b}_\ell}\text{ }\max_{\beta\ge 0}\text{ }\min_{\vct{\alpha}}\text{ }\min_{\alpha_0\ge 0}\text{ }\frac{1}{n}\left(\beta\twonorm{\mtx{Y}^T\mtx{V}\mtx{\Sigma}\vct{\alpha}+ \sigma\sqrt{\twonorm{\vct{\alpha}}^2+\alpha_0^2}\vct{g}+b_\ell\vct{1}_n-\mtx{Y}_\ell-\mtx{D}^{-1}\vct{u}}+ \sigma\beta\vct{h}^T\mtx{U}\vct{\alpha}- \sigma\alpha_0\beta\twonorm{\mtx{U}_{\perp}^T\vct{h}}+\frac{\twonorm{\vct{u}}^2}{2}\right)
\end{align*}
Since $\mtx{U}^T\vct{h}$ is $r\le k$ dimensional in our asymptotic regime the $\vct{h}^T\mtx{U}\vct{\alpha}$ term can be ignored. Also replacing $\beta$ with $\beta/\sqrt{n}$ we thus arrive at
\begin{align*}
&\min_{\vct{u}, \vct{b}_\ell}\text{ }\max_{\beta\ge 0}\text{ }\min_{\vct{\alpha}}\text{ }\min_{\alpha_0\ge 0}\text{ }\frac{\beta}{\sqrt{n}}\twonorm{\mtx{Y}^T\mtx{V}\mtx{\Sigma}\vct{\alpha}+ \sigma\sqrt{\twonorm{\vct{\alpha}}^2+\alpha_0^2}\vct{g}+b_\ell\vct{1}_n-\mtx{Y}_\ell-\mtx{D}^{-1}\vct{u}}- \frac{1}{\sqrt{n}}\sigma\alpha_0\beta\twonorm{\mtx{U}_{\perp}^T\vct{h}}+\frac{\twonorm{\vct{u}}^2}{2n}\\
&=\min_{\vct{u}, \vct{b}_\ell}\text{ }\max_{\beta\ge 0}\text{ }\min_{\vct{\alpha}}\text{ }\min_{\alpha_0\ge 0}\text{ }\min_{\tau\ge 0}\text{ }\frac{\beta}{2n\tau}\twonorm{\mtx{Y}^T\mtx{V}\mtx{\Sigma}\vct{\alpha}+ \sigma\sqrt{\twonorm{\vct{\alpha}}^2+\alpha_0^2}\vct{g}+b_\ell\vct{1}_n-\mtx{Y}_\ell-\mtx{D}^{-1}\vct{u}}^2+\frac{\beta\tau}{2}\\
&\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad-\frac{1}{\sqrt{n}}\sigma\alpha_0\beta\twonorm{\mtx{U}_{\perp}^T\vct{h}}+\frac{\twonorm{\vct{u}}^2}{2n}\\
&=\min_{ \vct{b}_\ell}\text{ }\max_{\beta\ge 0}\text{ }\min_{\vct{\alpha}}\text{ }\min_{\alpha_0\ge 0}\text{ }\min_{\tau\ge 0}\text{ }\min_{\vct{u}}\text{ }\frac{\beta}{2n\tau}\twonorm{\mtx{Y}^T\mtx{V}\mtx{\Sigma}\vct{\alpha}+ \sigma\sqrt{\twonorm{\vct{\alpha}}^2+\alpha_0^2}\vct{g}+b_\ell\vct{1}_n-\mtx{Y}_\ell-\mtx{D}^{-1}\vct{u}}^2+\frac{\beta\tau}{2}\\
&\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad-\frac{1}{\sqrt{n}}\sigma\alpha_0\beta\twonorm{\mtx{U}_{\perp}^T\vct{h}}+\frac{\twonorm{\vct{u}}^2}{2n}
\end{align*}
Setting the derivative with respect to $\vct{u}$ to zero we arrive at
\begin{align*}
\vct{u}=\frac{\beta}{\tau}\mtx{D}^{-1}\left(\mtx{I}+\frac{\beta}{\tau}\mtx{D}^{-2}\right)^{-1}\left(\mtx{Y}^T\mtx{V}\mtx{\Sigma}\vct{\alpha}+ \sigma\sqrt{\twonorm{\vct{\alpha}}^2+\alpha_0^2}\vct{g}+b_\ell\vct{1}_n-\mtx{Y}_\ell\right)
\end{align*}
Plugging the latter into the above the AO simplifies to
\begin{align*}
&\min_{ \vct{b}_\ell}\text{ }\max_{\beta\ge 0}\text{ }\min_{\vct{\alpha}}\text{ }\min_{\alpha_0\ge 0}\text{ }\min_{\tau\ge 0}\text{ }\text{ }\frac{\beta}{2\tau n}\text{trace}\left(\vct{t}^T\left(\mtx{I}+\frac{\beta}{\tau}\mtx{D}^{-2}\right)^{-1}\vct{t}\right)-\frac{1}{\sqrt{n}}\sigma\alpha_0\beta\twonorm{\mtx{U}_{\perp}^T\vct{h}}+\frac{\beta\tau}{2}
%+\frac{\twonorm{\vct{u}}^2}{2n}
\end{align*}
where
\begin{align*}
\vct{t}:=\mtx{Y}^T\mtx{V}\mtx{\Sigma}\vct{\alpha}+ \sigma\sqrt{\twonorm{\vct{\alpha}}^2+\alpha_0^2}\vct{g}+b_\ell\vct{1}_n-\mtx{Y}_\ell=\mtx{Y}^T\left(\mtx{V}\mtx{\Sigma}\vct{\alpha}-\vct{e}_\ell\right)+ \sigma\sqrt{\twonorm{\vct{\alpha}}^2+\alpha_0^2}\vct{g}+b_\ell\vct{1}_n
\end{align*}
To continue note that in our asymptotic regime we have
\begin{align*}
\frac{1}{\sqrt{n}}\twonorm{\mtx{U}_{\perp}^T\vct{h}}\text{ }\rP\text{ }\sqrt{\gamma}
\end{align*}
and the cross terms can be ignored so that in an asymptotic sense
\begin{align*}
\frac{1}{n}\text{trace}\left(\vct{t}^T\left(\mtx{I}+\frac{\beta}{\tau}\mtx{D}^{-2}\right)^{-1}\vct{t}\right)=&\frac{1}{n}\sigma^2\left(\twonorm{\vct{\alpha}}^2+\alpha_0^2\right)\text{trace}\left(\left(\mtx{I}+\frac{\beta}{\tau}\mtx{D}^{-2}\right)^{-1}\right)\\
&+\frac{1}{n}\text{trace}\left(\left(\mtx{Y}^T\left(\mtx{V}\mtx{\Sigma}\vct{\alpha}-\vct{e}_\ell\right)+b_\ell\vct{1}_n\right)^T\left(\mtx{I}+\frac{\beta}{\tau}\mtx{D}^{-2}\right)^{-1}\left(\mtx{Y}^T\left(\mtx{V}\mtx{\Sigma}\vct{\alpha}-\vct{e}_\ell\right)+b_\ell\vct{1}_n\right)\right)
\end{align*}
Therefore we arrive at
\begin{align*}
&\min_{ \vct{b}_\ell}\text{ }\max_{\beta\ge 0}\text{ }\min_{\vct{\alpha}}\text{ }\min_{\tau\ge 0}\text{ }\min_{\alpha_0\ge 0}\text{ }\text{ }\frac{\beta}{2\tau n}\sigma^2\left(\twonorm{\vct{\alpha}}^2+\alpha_0^2\right)\text{trace}\left(\left(\mtx{I}+\frac{\beta}{\tau}\mtx{D}^{-2}\right)^{-1}\right)-\sigma\alpha_0\beta\sqrt{\gamma}+\frac{\beta\tau}{2}\\
&\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad +\frac{\beta}{2\tau n}\text{trace}\left(\left(\mtx{Y}^T\left(\mtx{V}\mtx{\Sigma}\vct{\alpha}-\vct{e}_\ell\right)+b_\ell\vct{1}_n\right)^T\left(\mtx{I}+\frac{\beta}{\tau}\mtx{D}^{-2}\right)^{-1}\left(\mtx{Y}^T\left(\mtx{V}\mtx{\Sigma}\vct{\alpha}-\vct{e}_\ell\right)+b_\ell\vct{1}_n\right)\right)
%+\frac{\twonorm{\vct{u}}^2}{2n}
\end{align*}
which can be rewritten in the form
\begin{align*}
&\min_{ \vct{b}_\ell}\text{ }\max_{\beta\ge 0}\text{ }\min_{\vct{\alpha}}\text{ }\min_{\tau\ge 0}\text{ }\text{ }\text{ }\frac{\beta}{2\tau n}\sigma^2\twonorm{\vct{\alpha}}^2\text{trace}\left(\left(\mtx{I}+\frac{\beta}{\tau}\mtx{D}^{-2}\right)^{-1}\right)+\frac{\beta\tau}{2}\\
&\quad\quad\quad\quad\quad\quad\quad\quad\quad +\frac{\beta}{2\tau n}\text{trace}\left(\left(\mtx{Y}^T\left(\mtx{V}\mtx{\Sigma}\vct{\alpha}-\vct{e}_\ell\right)+b_\ell\vct{1}_n\right)^T\left(\mtx{I}+\frac{\beta}{\tau}\mtx{D}^{-2}\right)^{-1}\left(\mtx{Y}^T\left(\mtx{V}\mtx{\Sigma}\vct{\alpha}-\vct{e}_\ell\right)+b_\ell\vct{1}_n\right)\right)\\
&\quad\quad\quad\quad\quad\quad\quad\quad\quad+\frac{\beta}{2\tau n}\sigma^2\alpha_0^2\text{trace}\left(\left(\mtx{I}+\frac{\beta}{\tau}\mtx{D}^{-2}\right)^{-1}\right)-\alpha_0\sigma\beta\sqrt{\gamma}
%+\frac{\twonorm{\vct{u}}^2}{2n}
\end{align*}
To continue further we shall assume $\mtx{D}=\text{diag}\left(\mtx{Y}^T\vct{\omega}\right)$. Note that in this case
\begin{align*}
\frac{1}{n} \text{trace}\left(\left(\mtx{I}+\frac{\beta}{\tau}\mtx{D}^{-2}\right)^{-1}\right)=\frac{1}{n}\sum_{i=1}^n \frac{(\vct{y}_i^T\vct{\omega})^2}{(\vct{y}_i^T\vct{\omega})^2+\frac{\beta}{\tau}}=\sum_{\ell=1}^k \frac{n_\ell}{n}\frac{\omega_\ell^2}{\omega_\ell^2+\frac{\beta}{\tau}}\text{ }\rP\text{ }\sum_{\ell=1}^k\frac{\pi_\ell\omega_\ell^2}{\omega_\ell^2+\frac{\beta}{\tau}}
\end{align*}
Also
\begin{align*}
&\frac{1}{n}\text{trace}\left(\left(\mtx{Y}^T\left(\mtx{V}\mtx{\Sigma}\vct{\alpha}-\vct{e}_\ell\right)+b_\ell\vct{1}_n\right)^T\left(\mtx{I}+\frac{\beta}{\tau}\mtx{D}^{-2}\right)^{-1}\left(\mtx{Y}^T\left(\mtx{V}\mtx{\Sigma}\vct{\alpha}-\vct{e}_\ell\right)+b_\ell\vct{1}_n\right)\right)\\
&=\frac{1}{n}\text{trace}\left(\left(\mtx{V}\mtx{\Sigma}\vct{\alpha}-\vct{e}_\ell\right)^T\mtx{Y}\left(\mtx{I}+\frac{\beta}{\tau}\mtx{D}^{-2}\right)^{-1}\mtx{Y}^T\left(\mtx{V}\mtx{\Sigma}\vct{\alpha}-\vct{e}_\ell\right)\right)\\
&\quad+\frac{2}{n}b_\ell\vct{1}_n^T\left(\mtx{I}+\frac{\beta}{\tau}\mtx{D}^{-2}\right)^{-1}\mtx{Y}^T\left(\mtx{V}\mtx{\Sigma}\vct{\alpha}-\vct{e}_\ell\right)+\frac{b_\ell^2}{n} \text{trace}\left(\left(\mtx{I}+\frac{\beta}{\tau}\mtx{D}^{-2}\right)^{-1}\right)\\
&\rP\text{ }\text{trace}\left(\left(\mtx{V}\mtx{\Sigma}\vct{\alpha}-\vct{e}_\ell\right)^T\text{diag}\left(\frac{\pi_1\omega_1^2}{\omega_1^2+\frac{\beta}{\tau}},\frac{\pi_2\omega_2^2}{\omega_2^2+\frac{\beta}{\tau}},\ldots,\frac{\pi_k\omega_k^2}{\omega_k^2+\frac{\beta}{\tau}}\right)\left(\mtx{V}\mtx{\Sigma}\vct{\alpha}-\vct{e}_\ell\right)\right)\\
&\quad+2b_\ell\begin{bmatrix}\frac{\pi_1\omega_1^2}{\omega_1^2+\frac{\beta}{\tau}}&\frac{\pi_2\omega_2^2}{\omega_2^2+\frac{\beta}{\tau}}&\ldots &\frac{\pi_k\omega_k^2}{\omega_k^2+\frac{\beta}{\tau}}\end{bmatrix}\left(\mtx{V}\mtx{\Sigma}\vct{\alpha}-\vct{e}_\ell\right)+b_\ell^2\left(\sum_{\ell=1}^k\frac{\pi_\ell\omega_\ell^2}{\omega_\ell^2+\frac{\beta}{\tau}}\right)\\
\end{align*}
Next define 
\begin{align}\label{eq:Amatnew2}
\mtx{A}(\eta):=&\begin{bmatrix} \sigma^2\left(\vct{\pi}^T\vct{\nu}(\eta)\right)\mtx{I}+\Sigmab\Vb^T\text{diag}\left(\vct{\pi}\right)\text{diag}\left(\vct{\nu}(\eta)\right)\Vb\Sigmab & \Sigmab\Vb^T\text{diag}\left(\vct{\nu}(\eta)\right)\vct{\pi} \\ 
\vct{\pi}^T\text{diag}\left(\vct{\nu}(\eta)\right)\Vb\Sigmab & \vct{\pi}^T\vct{\nu}(\eta) \end{bmatrix}\nonumber\\
\cb_\ell :=& \begin{bmatrix} \Sigmab\Vb^T\eb_\ell \\ 1 \end{bmatrix}
\end{align}
where
\begin{align*}
\vct{\nu}(\eta)=\frac{1}{\gamma}\begin{bmatrix}\frac{\omega_1^2}{\omega_1^2+\eta}\\\frac{\omega_2^2}{\omega_2^2+\eta}\\\ldots \\\frac{\omega_k^2}{\omega_k^2+\eta}\end{bmatrix}
\end{align*}
We thus arrive at
\begin{align*}
&\min_{\vct{\alpha}}\text{ }\min_{ \vct{b}_\ell}\text{ }\max_{\alpha_0\ge 0}\text{ }\max_{\beta\ge 0}\text{ }\min_{\tau\ge 0}\text{ }\text{ }\frac{\gamma\beta}{2\tau}\left(\pi_\ell\vct{\nu}_\ell\left(\frac{\beta}{\tau}\right) +  \begin{bmatrix} \alphab^T & b_\ell \end{bmatrix} \mtx{A}\left(\frac{\beta}{\tau}\right)  \begin{bmatrix} \alphab \\ b_\ell  \end{bmatrix} - 2 \pi_\ell\vct{\nu}_\ell\left(\frac{\beta}{\tau}\right) \cb_\ell^T \begin{bmatrix} \alphab \\ b_\ell  \end{bmatrix}\right)\\
&\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad+\frac{\gamma\beta}{2\tau }\sigma^2\left(\vct{\pi}^T\vct{\nu}\left(\frac{\beta}{\tau}\right)\right)\alpha_0^2-\alpha_0\sigma\beta\sqrt{\gamma}+\frac{\beta\tau}{2}
%+\frac{\twonorm{\vct{u}}^2}{2n}
\end{align*}
Setting the derivative of the above with respect to $\alpha_0$ to zero we arrive at
\begin{align*}
\frac{\gamma\beta}{\tau }\sigma^2\left(\vct{\pi}^T\vct{\nu}\left(\frac{\beta}{\tau}\right)\right)\alpha_0-\sigma\beta\sqrt{\gamma}=0\quad\Rightarrow\quad \alpha_0=\frac{\tau}{\sigma\sqrt{\gamma}\left(\vct{\pi}^T\vct{\nu}\left(\frac{\beta}{\tau}\right)\right)}
\end{align*}
Note that the above objective has the form
\begin{align*}
f\left(\frac{\beta}{\tau}\right)-\alpha_0\sigma\beta\sqrt{\gamma}+\frac{\beta\tau}{2}
\end{align*}
with
\begin{align*}
f(\eta):=\frac{\eta\gamma}{2}\left(\pi_\ell\vct{\nu}_\ell(\eta) +  \begin{bmatrix} \alphab^T & b_\ell \end{bmatrix} \mtx{A}(\eta)  \begin{bmatrix} \alphab \\ b_\ell  \end{bmatrix} - 2 \pi_\ell\vct{\nu}_\ell(\eta) \cb_\ell^T \begin{bmatrix} \alphab \\ b_\ell  \end{bmatrix}\right)+\frac{\gamma\eta}{2 }\sigma^2\left(\vct{\pi}^T\vct{\nu}(\eta)\right)\alpha_0^2.
\end{align*}
Thus, the derivatives with respect to $\beta$ and $\tau$ to zero we have
\begin{align*}
\frac{1}{\tau}f'\left(\frac{\beta}{\tau}\right)-\alpha_0\sigma\sqrt{\gamma}+\frac{\tau}{2}=0\quad\Rightarrow\quad f'\left(\frac{\beta}{\tau}\right)-\alpha_0\sigma\sqrt{\gamma}\tau+\frac{\tau^2}{2}=0\quad\Rightarrow\quad f'\left(\frac{\beta}{\tau}\right)=\tau^2\left(\frac{1}{\vct{\pi}^T\vct{\nu}\left(\frac{\beta}{\tau}\right)}-\frac{1}{2}\right)
\end{align*}
and
\begin{align*}
-\frac{\beta}{\tau^2}f'\left(\frac{\beta}{\tau}\right)+\frac{\beta}{2}=0\quad\Rightarrow\quad \tau^2=2f'\left(\frac{\beta}{\tau}\right)
\end{align*}
Combining the latter two we conclude that $\vct{\pi}^T\vct{\nu}\left(\frac{\beta}{\tau}\right)=1$.  Thus, $\eta=\frac{\beta}{\tau}$ is the solution to $\vct{\pi}^T\vct{\nu}\left(\eta\right)=1$. To calculate $\tau$ and hence $\alpha_0$ we calculate $f'$ which is equal to
\begin{align*}
f'(\eta)=&\frac{\gamma}{2}\left(\pi_\ell\vct{\nu}_\ell(\eta) +  \begin{bmatrix} \alphab^T & b_\ell \end{bmatrix} \mtx{A}(\eta)  \begin{bmatrix} \alphab \\ b_\ell  \end{bmatrix} - 2 \pi_\ell\vct{\nu}_\ell(\eta) \cb_\ell^T \begin{bmatrix} \alphab \\ b_\ell  \end{bmatrix}\right)+\frac{\gamma}{2 }\sigma^2\left(\vct{\pi}^T\vct{\nu}(\eta)\right)\alpha_0^2+\frac{\gamma\eta}{2 }\sigma^2\alpha_0^2(\vct{\pi}^T\vct{\nu}'(\eta))\\
&+\frac{\gamma\eta}{2}\left(\pi_\ell\vct{\nu}_\ell'(\eta) +  \begin{bmatrix} \alphab^T & b_\ell \end{bmatrix} \mtx{A}'(\eta)  \begin{bmatrix} \alphab \\ b_\ell  \end{bmatrix} - 2 \pi_\ell\vct{\nu}_\ell'(\eta) \cb_\ell^T \begin{bmatrix} \alphab \\ b_\ell  \end{bmatrix}\right)
\end{align*}
Where
\begin{align*}
\vct{\nu}'(\eta)=-\frac{1}{\gamma}\begin{bmatrix}\frac{\omega_1^2}{(\omega_1^2+\eta)^2}\\\frac{\omega_2^2}{(\omega_2^2+\eta)^2}\\\ldots \\\frac{\omega_k^2}{(\omega_k^2+\eta)^2}\end{bmatrix}\quad\text{and}\quad \mtx{A}'(\eta):=&\begin{bmatrix} \sigma^2\left(\vct{\pi}^T\vct{\nu}'(\eta)\right)\mtx{I}+\Sigmab\Vb^T\text{diag}\left(\vct{\pi}\right)\text{diag}\left(\vct{\nu}'(\eta)\right)\Vb\Sigmab & \Sigmab\Vb^T\text{diag}\left(\vct{\nu}'(\eta)\right)\vct{\pi} \\ 
\vct{\pi}^T\text{diag}\left(\vct{\nu}'(\eta)\right)\Vb\Sigmab & \vct{\pi}^T\vct{\nu}'(\eta) \end{bmatrix}\nonumber\\
\cb_\ell :=& \begin{bmatrix} \Sigmab\Vb^T\eb_\ell \\ 1 \end{bmatrix}
\end{align*}
Now note that at the optimal point we have
\begin{align*}
f'(\eta)=\frac{\tau^2}{2}=\frac{\gamma}{2 }\sigma^2\left(\vct{\pi}^T\vct{\nu}(\eta)\right)\alpha_0^2
\end{align*}
Thus from the above we can conclude that
\begin{align*}
\alpha_0^2=&-\frac{1}{\eta\sigma^2(\vct{\pi}^T\vct{\nu}'(\eta))}\left(\pi_\ell\vct{\nu}_\ell(\eta) +  \begin{bmatrix} \alphab^T & b_\ell \end{bmatrix} \mtx{A}(\eta)  \begin{bmatrix} \alphab \\ b_\ell  \end{bmatrix} - 2 \pi_\ell\vct{\nu}_\ell(\eta) \cb_\ell^T \begin{bmatrix} \alphab \\ b_\ell  \end{bmatrix}\right)\\
&-\frac{1}{\sigma^2(\vct{\pi}^T\vct{\nu}'(\eta))}\left(\pi_\ell\vct{\nu}_\ell'(\eta) +  \begin{bmatrix} \alphab^T & b_\ell \end{bmatrix} \mtx{A}'(\eta)  \begin{bmatrix} \alphab \\ b_\ell  \end{bmatrix} - 2 \pi_\ell\vct{\nu}_\ell'(\eta) \cb_\ell^T \begin{bmatrix} \alphab \\ b_\ell  \end{bmatrix}\right)
\end{align*}
Thus the AO optimization problem reduces to
\begin{align*}
\min_{ \vct{b}_\ell}\text{ }\min_{\vct{\alpha}}\text{ }\frac{\eta\gamma}{2}\left(\pi_\ell\vct{\nu}_\ell +  \begin{bmatrix} \alphab^T & b_\ell \end{bmatrix} \A  \begin{bmatrix} \alphab \\ b_\ell  \end{bmatrix} - 2 \pi_\ell\vct{\nu}_\ell \cb_\ell^T \begin{bmatrix} \alphab \\ b_\ell  \end{bmatrix}\right)
\end{align*}
where $\eta$ is the solution to
\begin{align*}
\sum_{\ell=1}^k\frac{\pi_\ell\omega_\ell^2}{\omega_\ell^2+\eta}=\gamma
\end{align*}
and
\begin{align}\label{eq:Amatnew22}
\A(\eta):=&\begin{bmatrix} \sigma^2\Iden_r+\Sigmab\Vb^T\text{diag}\left(\vct{\pi}\odot\vct{\nu}\right)\Vb\Sigmab & \Sigmab\Vb^T\left(\vct{\pi}\odot\vct{\nu}\right) \\ 
\left(\vct{\pi}\odot\vct{\nu}\right)^T\Vb\Sigmab & 1 \end{bmatrix}\nonumber\\
\cb_\ell :=& \begin{bmatrix} \Sigmab\Vb^T\eb_\ell \\ 1 \end{bmatrix}
\end{align}
where
\begin{align*}
\vct{\nu}:=\frac{1}{\gamma}\begin{bmatrix}\frac{\omega_1^2}{\omega_1^2+\eta}\\\frac{\omega_2^2}{\omega_2^2+\eta}\\\ldots \\\frac{\omega_k^2}{\omega_k^2+\eta}\end{bmatrix}
\end{align*}

First, note that the matrix $\A$ is positive definite. This can be checked by computing the Schur complement of $\A$:
\begin{align}\label{eq:Deltab_def2}
\Deltab:=\sigma^2\Iden_r+\Sigmab\Vb^T\Pb\Vb\Sigmab:=\sigma^2\Iden_r+\Sigmab\Vb^T\left(\diag{\pib\odot\vct{\nu}}-\left(\pib\odot\vct{\nu}\right)\left(\pib\odot\vct{\nu}\right)^T\right)\Vb\Sigmab \succ \zero_{r\times r}.
\end{align}
Positive definiteness above holds because $\Pb:=\left(\diag{\pib\odot\vct{\nu}}-\left(\pib\odot\vct{\nu}\right)\left(\pib\odot\vct{\nu}\right)^T\right)\succeq \zero_{k\times k}$. Thus the objective is a strictly convex quadratic and is jointly convex in its arguments. We proceed by minimizing the objective over $(\alphab,b_\ell)$ which is equal to
\bea
\begin{bmatrix} \widehat\alphab \\ \widehat b_\ell \end{bmatrix} = \pi_\ell\nu_\ell \A^{-1} \cb_\ell = \pi_\ell \nu_\ell\begin{bmatrix} -\Deltab^{-1}\Sigmab\Vb^T(\pib\odot\vct{\nu}-\eb_\ell) \\ 1+\left(\pib\odot\vct{\nu}\right)^T\Vb\Sigmab\Deltab^{-1}\Sigmab\Vb^T(\pib\odot\vct{\nu}-\eb_\ell) \end{bmatrix}\label{eq:alphab_1t}
%\\
%&= \pi_\ell \begin{bmatrix} -\Sigmab^{-1}\Vb^T\left(\Vb\Sigmab^{-2}\Vb^T+\Pb\right)^{-1}(\pib-\eb_\ell) \\ 1+\pib^T\left(\Vb\Sigmab^{-2}\Vb^T+\Pb\right)^{-1}(\pib-\eb_\ell), \end{bmatrix}\nn\\
%&= \pi_\ell \begin{bmatrix} -\Sigmab^{-1}\Vb^T\left(\Vb\Sigmab^{-2}\Vb^T+\Pb\right)^{-1}(\pib-\eb_\ell) \\ \frac{1-\pib^T\left(\Vb\Sigmab\Vb^T+\diag{\pib}\right)^{-1}\eb_\ell}{1-\pib^T\left(\Vb\Sigmab\Vb^T+\diag{\pib}\right)^{-1}\pib}, 
%\end{bmatrix}
\end{align}
%where the last two equalities follow from the Matrix inversion formula  and some algebra (see Lemma \ref{lem:pi_vec}). 
Thus, the minimum value attained is
\begin{align}
&-\pi_\ell^2\nu_\ell^2  \begin{bmatrix} -\left(\pib\odot\vct{\nu} - \eb_\ell\right)^T\Vb\Sigmab && 1 \end{bmatrix} \begin{bmatrix} \Deltab^{-1} & \zero \\ \zero^T & 1 \end{bmatrix}\begin{bmatrix} -\Sigmab\Vb^T \left(\pib\odot\vct{\nu} - \eb_\ell\right) \\ 1 \end{bmatrix} \\
&= - \pi_\ell^2\nu_\ell^2\left(1+\left(\pib\odot\vct{\nu} - \eb_\ell\right)^T\Vb\Sigmab \Deltab^{-1} \Sigmab\Vb^T \left(\pib\odot\vct{\nu} - \eb_\ell\right)\right).  \nn%\nn\\
%&= - \pi_\ell^2\left(1+\left(\pib - \eb_\ell\right)^T \left(\Vb^T\Sigmab^{-2}\Vb^T+\Pb\right)^{-1} \left(\pib - \eb_\ell\right)\right) .
\end{align}
Thus the objective reduces to
\begin{align}
\frac{\eta \gamma}{2}\left(\pi_\ell\nu_\ell - \pi_\ell^2\nu_\ell^2\left(\pib\odot\vct{\nu} - \eb_\ell\right)^T\Vb\Sigmab \Deltab^{-1} \Sigmab\Vb^T \left(\pib\odot\vct{\nu} - \eb_\ell\right)\right).
\label{eq:final}
\end{align}
Therefore,
\begin{align*}
\alpha_0^2=&-\frac{1}{\eta\sigma^2(\vct{\pi}^T\vct{\nu}'(\eta))}\left(\pi_\ell\nu_\ell - \pi_\ell^2\nu_\ell^2\left(\pib\odot\vct{\nu} - \eb_\ell\right)^T\Vb\Sigmab \Deltab^{-1} \Sigmab\Vb^T \left(\pib\odot\vct{\nu} - \eb_\ell\right)\right)\\
&-\frac{1}{\sigma^2(\vct{\pi}^T\vct{\nu}'(\eta))}\left(\pi_\ell\vct{\nu}_\ell'(\eta) +  \begin{bmatrix} \alphab^T & b_\ell \end{bmatrix} \mtx{A}'(\eta)  \begin{bmatrix} \alphab \\ b_\ell  \end{bmatrix} - 2 \pi_\ell\vct{\nu}_\ell'(\eta) \cb_\ell^T \begin{bmatrix} \alphab \\ b_\ell  \end{bmatrix}\right)\\
=&-\frac{\zeta}{\sigma^2}\left(\pi_\ell\nu_\ell - \pi_\ell^2\nu_\ell^2\left(\pib\odot\vct{\nu} - \eb_\ell\right)^T\Vb\Sigmab \Deltab^{-1} \Sigmab\Vb^T \left(\pib\odot\vct{\nu} - \eb_\ell\right)\right)
\end{align*}
%{\color{blue} Need to check that the term in the square-root is non-negative}
where
\begin{align*}
\zeta:=\frac{1}{(\vct{\pi}^T\vct{\nu}'(\eta))}\left(\frac{1}{\eta}+\frac{\left(\pi_\ell\vct{\nu}_\ell'(\eta) +  \begin{bmatrix} \widehat\alphab \\ \widehat b_\ell \end{bmatrix}^T \mtx{A}'(\eta)  \begin{bmatrix} \widehat\alphab \\ \widehat b_\ell \end{bmatrix} - 2 \pi_\ell\vct{\nu}_\ell'(\eta) \cb_\ell^T\begin{bmatrix} \widehat\alphab \\ \widehat b_\ell \end{bmatrix}\right)}{\left(\pi_\ell\nu_\ell - \pi_\ell^2\nu_\ell^2\left(\pib\odot\vct{\nu} - \eb_\ell\right)^T\Vb\Sigmab \Deltab^{-1} \Sigmab\Vb^T \left(\pib\odot\vct{\nu} - \eb_\ell\right)\right)}\right)
\end{align*}
with 
\begin{align*}
\begin{bmatrix} \widehat\alphab \\ \widehat b_\ell \end{bmatrix}  = \pi_\ell \nu_\ell\begin{bmatrix} -\Deltab^{-1}\Sigmab\Vb^T(\pib\odot\vct{\nu}-\eb_\ell) \\ 1+\left(\pib\odot\vct{\nu}\right)^T\Vb\Sigmab\Deltab^{-1}\Sigmab\Vb^T(\pib\odot\vct{\nu}-\eb_\ell) \end{bmatrix}
\end{align*}
and
\begin{align*}
\vct{\nu}'(\eta)=-\frac{1}{\gamma}\begin{bmatrix}\frac{\omega_1^2}{(\omega_1^2+\eta)^2}\\\frac{\omega_2^2}{(\omega_2^2+\eta)^2}\\\ldots \\\frac{\omega_k^2}{(\omega_k^2+\eta)^2}\end{bmatrix}\quad\text{and}\quad \mtx{A}'(\eta):=&\begin{bmatrix} \sigma^2\left(\vct{\pi}^T\vct{\nu}'(\eta)\right)\mtx{I}+\Sigmab\Vb^T\text{diag}\left(\vct{\pi}\right)\text{diag}\left(\vct{\nu}'(\eta)\right)\Vb\Sigmab & \Sigmab\Vb^T\text{diag}\left(\vct{\nu}'(\eta)\right)\vct{\pi} \\ 
\vct{\pi}^T\text{diag}\left(\vct{\nu}'(\eta)\right)\Vb\Sigmab & \vct{\pi}^T\vct{\nu}'(\eta) \end{bmatrix}
\end{align*}
\vp
\noindent\textbf{Asymptotic predictions.}~~First, from \eqref{eq:alphab_1t} the bias term converges as follows:
$$
\widehat{b}_\ell \rP \pi_\ell\nu_\ell\left(1+\left(\pib\odot\vct{\nu}\right)^T\Vb\Sigmab\Deltab^{-1}\Sigmab\Vb^T(\pib\odot\vct{\nu}-\eb_\ell)\right).
$$
Thus,
\begin{align*}
\widehat{\vct{b}}\rP\left(\mtx{I}_k-\mtx{P}\Vb\Sigmab\Deltab^{-1}\Sigmab\Vb^T \right)\left(\pib\odot \vct{\nu}\right)
\end{align*}
 Recall that $\alphab = \Ub^T\w_\ell$. Thus, the correlations $\inp{\mub_i}{\w_\ell},~i\in[k]$ converge as follows:
\begin{align}
\M^T\w_\ell = \Vb\Sigmab\Ub^T\w_\ell \rP \Vb\Sigmab\widehat\alphab = -\pi_\ell\nu_\ell\Vb\Sigmab\Deltab^{-1}\Sigmab\Vb^T\left(\pib\odot\vct{\nu}-\eb_\ell\right).\quad
\end{align}
Here, convergence applies element-wise to the entries of the involved random vectors. Moreover, from the analysis above we can predict the limit of the norm $\twonorm{\w_\ell}$. For this, note that $\twonorm{\w_\ell}^2 = \widehat{\alpha}_0^2 + \widehat{\alphab}^T\widehat{\alphab}$. To continue further note that based on \eqref{myalphahat} we have
\begin{align*}
\widehat{\alpha}_0=\frac{\sqrt{\gamma}\tau}{\frac{\sigma}{n} \text{trace}\left(\left(\mtx{I}+\frac{\beta}{\tau}\mtx{D}^{-2}\right)^{-1}\right)}\rP\frac{\widehat{\tau}}{\sigma \sqrt{\gamma}}
\end{align*}
 Thus,
\begin{align}\label{eq:norm_lim}
\twonorm{\w_\ell}^2 \rP \frac{\zeta}{\sigma^2}\pi_\ell(1-\pi_\ell)  + \pi_\ell^2 \left(\pib - \eb_\ell\right)^T\Vb\Sigmab \Deltab^{-1} \left(\Deltab^{-1} - \frac{\zeta}{\sigma^2}\Iden_{r}\right) \Sigmab\Vb^T \left(\pib - \eb_\ell\right) 
\end{align}






\newpage
Setting the derivative with respect to $\alpha_0$ to zero we have
\begin{align}
\label{myalphahat}
\widehat{\alpha}_0=\frac{\sqrt{\gamma}\tau}{\frac{\sigma}{n} \text{trace}\left(\left(\mtx{I}+\frac{\beta}{\tau}\mtx{D}^{-2}\right)^{-1}\right)}
\end{align}
Plugging the above we arrive at
\begin{align*}
&\min_{ \vct{b}_\ell}\text{ }\max_{\beta\ge 0}\text{ }\min_{\vct{\alpha}}\text{ }\min_{\tau\ge 0}\text{ }\text{ }\text{ }\frac{\beta}{2\tau n}\sigma^2\twonorm{\vct{\alpha}}^2\text{trace}\left(\left(\mtx{I}+\frac{\beta}{\tau}\mtx{D}^{-2}\right)^{-1}\right)+\frac{\beta\tau}{2}\left(1-\frac{\gamma}{\frac{1}{n} \text{trace}\left(\left(\mtx{I}+\frac{\beta}{\tau}\mtx{D}^{-2}\right)^{-1}\right)}\right)\\
&\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad +\frac{\beta}{2\tau n}\text{trace}\left(\left(\mtx{Y}^T\left(\mtx{V}\mtx{\Sigma}\vct{\alpha}-\vct{e}_\ell\right)+b_\ell\vct{1}_n\right)^T\left(\mtx{I}+\frac{\beta}{\tau}\mtx{D}^{-2}\right)^{-1}\left(\mtx{Y}^T\left(\mtx{V}\mtx{\Sigma}\vct{\alpha}-\vct{e}_\ell\right)+b_\ell\vct{1}_n\right)\right)
%+\frac{\twonorm{\vct{u}}^2}{2n}
\end{align*}
To continue further we shall assume $\mtx{D}=\text{diag}\left(\mtx{Y}^T\vct{\omega}\right)$. Note that in this case
\begin{align*}
\frac{1}{n} \text{trace}\left(\left(\mtx{I}+\frac{\beta}{\tau}\mtx{D}^{-2}\right)^{-1}\right)=\frac{1}{n}\sum_{i=1}^n \frac{(\vct{y}_i^T\vct{\omega})^2}{(\vct{y}_i^T\vct{\omega})^2+\frac{\beta}{\tau}}=\sum_{\ell=1}^k \frac{n_\ell}{n}\frac{\omega_\ell^2}{\omega_\ell^2+\frac{\beta}{\tau}}\text{ }\rP\text{ }\sum_{\ell=1}^k\frac{\pi_\ell\omega_\ell^2}{\omega_\ell^2+\frac{\beta}{\tau}}
\end{align*}
Also
\begin{align*}
&\frac{1}{n}\text{trace}\left(\left(\mtx{Y}^T\left(\mtx{V}\mtx{\Sigma}\vct{\alpha}-\vct{e}_\ell\right)+b_\ell\vct{1}_n\right)^T\left(\mtx{I}+\frac{\beta}{\tau}\mtx{D}^{-2}\right)^{-1}\left(\mtx{Y}^T\left(\mtx{V}\mtx{\Sigma}\vct{\alpha}-\vct{e}_\ell\right)+b_\ell\vct{1}_n\right)\right)\\
&=\frac{1}{n}\text{trace}\left(\left(\mtx{V}\mtx{\Sigma}\vct{\alpha}-\vct{e}_\ell\right)^T\mtx{Y}\left(\mtx{I}+\frac{\beta}{\tau}\mtx{D}^{-2}\right)^{-1}\mtx{Y}^T\left(\mtx{V}\mtx{\Sigma}\vct{\alpha}-\vct{e}_\ell\right)\right)\\
&\quad+\frac{2}{n}b_\ell\vct{1}_n^T\left(\mtx{I}+\frac{\beta}{\tau}\mtx{D}^{-2}\right)^{-1}\mtx{Y}^T\left(\mtx{V}\mtx{\Sigma}\vct{\alpha}-\vct{e}_\ell\right)+\frac{b_\ell^2}{n} \text{trace}\left(\left(\mtx{I}+\frac{\beta}{\tau}\mtx{D}^{-2}\right)^{-1}\right)\\
&\rP\text{ }\text{trace}\left(\left(\mtx{V}\mtx{\Sigma}\vct{\alpha}-\vct{e}_\ell\right)^T\text{diag}\left(\frac{\pi_1\omega_1^2}{\omega_1^2+\frac{\beta}{\tau}},\frac{\pi_2\omega_2^2}{\omega_2^2+\frac{\beta}{\tau}},\ldots,\frac{\pi_k\omega_k^2}{\omega_k^2+\frac{\beta}{\tau}}\right)\left(\mtx{V}\mtx{\Sigma}\vct{\alpha}-\vct{e}_\ell\right)\right)\\
&\quad+2b_\ell\begin{bmatrix}\frac{\pi_1\omega_1^2}{\omega_1^2+\frac{\beta}{\tau}}&\frac{\pi_2\omega_2^2}{\omega_2^2+\frac{\beta}{\tau}}&\ldots &\frac{\pi_k\omega_k^2}{\omega_k^2+\frac{\beta}{\tau}}\end{bmatrix}\left(\mtx{V}\mtx{\Sigma}\vct{\alpha}-\vct{e}_\ell\right)+b_\ell^2\left(\sum_{\ell=1}^k\frac{\pi_\ell\omega_\ell^2}{\omega_\ell^2+\frac{\beta}{\tau}}\right)\\
\end{align*}
Next define 
\begin{align}\label{eq:Amatnew2}
\A(\eta):=&\begin{bmatrix} \sigma^2\left(\vct{\pi}^T\vct{\nu}(\eta)\right)\Iden_r+\Sigmab\Vb^T\text{diag}\left(\vct{\pi}\right)\text{diag}\left(\vct{\nu}(\eta)\right)\Vb\Sigmab & \Sigmab\Vb^T\text{diag}\left(\vct{\nu}(\eta)\right)\vct{\pi} \\ 
\vct{\pi}^T\text{diag}\left(\vct{\nu}(\eta)\right)\Vb\Sigmab & \vct{\pi}^T\vct{\nu}(\eta) \end{bmatrix}\nonumber\\
\cb_\ell :=& \begin{bmatrix} \Sigmab\Vb^T\eb_\ell \\ 1 \end{bmatrix}
\end{align}
where
\begin{align*}
\vct{\nu}(\eta)=\frac{1}{\gamma}\begin{bmatrix}\frac{\omega_1^2}{\omega_1^2+\eta}\\\frac{\omega_2^2}{\omega_2^2+\eta}\\\ldots \\\frac{\omega_k^2}{\omega_k^2+\eta}\end{bmatrix}
\end{align*}
We thus arrive at
\begin{align*}
&\min_{ \vct{b}_\ell}\text{ }\max_{\beta\ge 0}\text{ }\min_{\vct{\alpha}}\text{ }\min_{\tau\ge 0}\text{ }\text{ }\frac{\beta}{2\tau}\gamma\left(\pi_\ell\vct{\nu}_\ell\left(\frac{\beta}{\tau}\right) +  \begin{bmatrix} \alphab^T & b_\ell \end{bmatrix} \A\left(\frac{\beta}{\tau}\right)  \begin{bmatrix} \alphab \\ b_\ell  \end{bmatrix} - 2 \pi_\ell\vct{\nu}_\ell\left(\frac{\beta}{\tau}\right) \cb_\ell^T \begin{bmatrix} \alphab \\ b_\ell  \end{bmatrix}\right)+\frac{\beta\tau}{2}\left(1-\frac{1}{\vct{\pi}^T\vct{\nu}\left(\frac{\beta}{\tau}\right)}\right)%+\frac{\twonorm{\vct{u}}^2}{2n}
\end{align*}
To continue define the vector
\begin{align*}
\widetilde{\vct{\pi}}(\eta)=\frac{1}{\vct{\pi}^T\vct{\nu}(\eta)}\vct{\nu}(\eta)\odot \vct{\pi}
\end{align*}
Then the above reduces to 
\begin{align*}
&\min_{ \vct{b}_\ell}\text{ }\max_{\beta\ge 0}\text{ }\min_{\vct{\alpha}}\text{ }\min_{\tau\ge 0}\text{ }\text{ }\frac{\beta}{2\tau}\gamma(\vct{\pi}^T\vct{\nu}(\eta))\left(\widetilde{\pi}_\ell\left(\frac{\beta}{\tau}\right) +  \begin{bmatrix} \alphab^T & b_\ell \end{bmatrix} \widetilde{\A}\left(\frac{\beta}{\tau}\right)  \begin{bmatrix} \alphab \\ b_\ell  \end{bmatrix} - 2 \widetilde{\pi}_\ell\left(\frac{\beta}{\tau}\right) \cb_\ell^T \begin{bmatrix} \alphab \\ b_\ell  \end{bmatrix}\right)+\frac{\beta\tau}{2}\left(1-\frac{1}{\vct{\pi}^T\vct{\nu}\left(\frac{\beta}{\tau}\right)}\right)%+\frac{\twonorm{\vct{u}}^2}{2n}
\end{align*}
where
\begin{align*}
\widetilde{\A}(\eta):=&\begin{bmatrix} \sigma^2\Iden_r+\Sigmab\Vb^T\text{diag}\left(\widetilde{\vct{\pi}}(\eta)\right)\Vb\Sigmab & \Sigmab\Vb^T\widetilde{\vct{\pi}}(\eta) \\ 
\widetilde{\vct{\pi}}(\eta)^T\Vb\Sigmab & 1\end{bmatrix}
\end{align*}
First, note that the matrix $\widetilde{\A}$ is positive definite. This can be checked by computing the Schur complement of $\widetilde{\A}$:
\begin{align}\label{eq:Deltab_def2tt}
\Deltab:=\sigma^2\Iden_r+\Sigmab\Vb^T\Pb\Vb\Sigmab:=\sigma^2\Iden_r+\Sigmab\Vb^T\left(\diag{\widetilde{\vct{\pi}}(\eta)}-\left(\widetilde{\vct{\pi}}(\eta)\right)\left(\widetilde{\vct{\pi}}(\eta)\right)^T\right)\Vb\Sigmab \succ \zero_{r\times r}.
\end{align}
Positive definiteness above holds because $\Pb:=\left(\diag{\widetilde{\vct{\pi}}(\eta)}-\left(\widetilde{\vct{\pi}}(\eta)\right)\left(\widetilde{\vct{\pi}}(\eta)\right)^T\right)\succeq \zero_{k\times k}$. Thus the objective is a strictly convex quadratic and is jointly convex in its arguments. We proceed by minimizing the objective over $(\alphab,b_\ell)$ which is equal to
\bea
\begin{bmatrix} \widehat\alphab \\ \widehat b_\ell \end{bmatrix} = \widetilde{\pi}_\ell(\eta) \left(\widetilde{\A}(\eta)\right)^{-1} \cb_\ell = \widetilde{\pi}_\ell(\eta)\begin{bmatrix} -\Deltab^{-1}\Sigmab\Vb^T(\widetilde{\vct{\pi}}(\eta)-\eb_\ell) \\ 1+\left(\widetilde{\vct{\pi}}(\eta)\right)^T\Vb\Sigmab\Deltab^{-1}\Sigmab\Vb^T(\widetilde{\vct{\pi}}(\eta)-\eb_\ell) \end{bmatrix}\label{eq:alphab_1ttt}
%\\
%&= \pi_\ell \begin{bmatrix} -\Sigmab^{-1}\Vb^T\left(\Vb\Sigmab^{-2}\Vb^T+\Pb\right)^{-1}(\pib-\eb_\ell) \\ 1+\pib^T\left(\Vb\Sigmab^{-2}\Vb^T+\Pb\right)^{-1}(\pib-\eb_\ell), \end{bmatrix}\nn\\
%&= \pi_\ell \begin{bmatrix} -\Sigmab^{-1}\Vb^T\left(\Vb\Sigmab^{-2}\Vb^T+\Pb\right)^{-1}(\pib-\eb_\ell) \\ \frac{1-\pib^T\left(\Vb\Sigmab\Vb^T+\diag{\pib}\right)^{-1}\eb_\ell}{1-\pib^T\left(\Vb\Sigmab\Vb^T+\diag{\pib}\right)^{-1}\pib}, 
%\end{bmatrix}
\end{align}
%where the last two equalities follow from the Matrix inversion formula  and some algebra (see Lemma \ref{lem:pi_vec}). 
Thus, the minimum value attained is
\begin{align}
&-\left(\widetilde{\pi}_\ell(\eta)\right)^2 \begin{bmatrix} -\left(\widetilde{\vct{\pi}}(\eta) - \eb_\ell\right)^T\Vb\Sigmab && 1 \end{bmatrix} \begin{bmatrix} \Deltab^{-1} & \zero \\ \zero^T & 1 \end{bmatrix}\begin{bmatrix} -\Sigmab\Vb^T \left(\widetilde{\vct{\pi}}(\eta) - \eb_\ell\right) \\ 1 \end{bmatrix} \\
&= -\left(\widetilde{\pi}_\ell(\eta)\right)^2\left(1+\left(\widetilde{\vct{\pi}}(\eta) - \eb_\ell\right)^T\Vb\Sigmab \Deltab^{-1} \Sigmab\Vb^T \left(\widetilde{\vct{\pi}}(\eta) - \eb_\ell\right)\right).  \nn%\nn\\
%&= - \pi_\ell^2\left(1+\left(\pib - \eb_\ell\right)^T \left(\Vb^T\Sigmab^{-2}\Vb^T+\Pb\right)^{-1} \left(\pib - \eb_\ell\right)\right) .
\end{align}
Thus the objective reduces to
\begin{align*}
&\max_{\beta\ge 0}\text{ }\min_{\tau\ge 0}\text{ }\text{ }\frac{\beta}{2\tau}\gamma\left(\vct{\pi}^T\vct{\nu}\left(\frac{\beta}{\tau}\right)\right)\left(\widetilde{\pi}_\ell\left(\frac{\beta}{\tau}\right)  -\left(\widetilde{\pi}_\ell\left(\frac{\beta}{\tau}\right)\right)^2- \left(\widetilde{\pi}_\ell\left(\frac{\beta}{\tau}\right)\right)^2\left( \widetilde{\vct{\pi}}\left(\frac{\beta}{\tau}\right)- \eb_\ell\right)^T\Vb\Sigmab \Deltab^{-1} \Sigmab\Vb^T \left(\widetilde{\vct{\pi}}\left(\frac{\beta}{\tau}\right) - \eb_\ell\right)\right)\\
&\quad\quad\quad\quad+\frac{\beta\tau}{2}\left(1-\frac{1}{\vct{\pi}^T\vct{\nu}\left(\frac{\beta}{\tau}\right)}\right)%+\frac{\twonorm{\vct{u}}^2}{2n}
\end{align*}
We now rewriting the objective above as
\begin{align*}
f_1\left(\frac{\beta}{\tau}\right)+\tau^2 f_2\left(\frac{\beta}{\tau}\right)
\end{align*}
with 
\begin{align*}
f_1(\eta):=&\frac{\eta\gamma}{2}\left(\vct{\pi}^T\vct{\nu}(\eta)\right)\left(\widetilde{\pi}_\ell(\eta) -\left(\widetilde{\pi}_\ell(\eta)\right)^2- \left(\widetilde{\pi}_\ell(\eta)\right)^2\left( \widetilde{\vct{\pi}}(\eta)- \eb_\ell\right)^T\Vb\Sigmab \Deltab^{-1} \Sigmab\Vb^T \left(\widetilde{\vct{\pi}}(\eta) - \eb_\ell\right)\right)\\
f_2(\eta):=&\frac{1}{2}\eta\left(1-\frac{1}{\vct{\pi}^T\vct{\nu}\left(\eta\right)}\right)
\end{align*}


Setting the derivatives with respect to $\beta$ and $\tau$ to zero we have
\begin{align*}
\frac{1}{\tau}f_1'\left(\frac{\beta}{\tau}\right)+\tau f_2'\left(\frac{\beta}{\tau}\right)=&0\\
-\frac{\beta}{\tau^2}f_1'\left(\frac{\beta}{\tau}\right)+2\tau f_2\left(\frac{\beta}{\tau}\right)-\beta f_2'\left(\frac{\beta}{\tau}\right)=&0
\end{align*}
Multiplying the first identity by $\frac{\beta}{\tau}$ and summing it with the second we conclude that
\begin{align*}
\beta f_2\left(\frac{\beta}{\tau}\right)=0\quad \Rightarrow\quad \beta=0\quad\text{or}\quad \vct{\pi}^T\vct{\nu}\left(\frac{\beta}{\tau}\right)=1
\end{align*}
Thus $\widehat{\eta}:=\frac{\widehat{\beta}}{\widehat{\tau}}$ is the solution to $\vct{\pi}^T\vct{\nu}(\eta)=\frac{1}{\gamma}\left(\sum_{\ell=1}^k\frac{\pi_\ell\omega_\ell^2}{\omega_\ell^2+\eta}\right)=1$. 

Next let us attempt to solve for $\tau$ using the first equation above combined with the fact $f_2\left(\frac{\beta}{\tau}\right)=0$ we conclude that
\begin{align*}
\frac{1}{\tau}f_1'\left(\frac{\beta}{\tau}\right)+\tau f_2'\left(\frac{\beta}{\tau}\right)=0\quad\Rightarrow\quad  f_1'(\eta)+\tau^2 f_2'(\eta)=0\quad\Rightarrow\quad \widehat{\tau}=\sqrt{-\frac{f_1'(\widehat{\eta})}{ f_2'(\widehat{\eta})}}
\end{align*}
Using Lhupital's rule it is easy to see that
\begin{align*}
\frac{\widehat{\tau}}{\sqrt{\gamma}}=\sqrt{-\lim_{\eta\rightarrow \widehat{\eta}}\frac{F_1(\eta)}{F_2(\eta)}}
\end{align*}
where
\begin{align*}
F_1(\eta):=&\left(\vct{\pi}^T\vct{\nu}(\eta)\right)^2\left(\widetilde{\pi}_\ell(\eta) -\left(\widetilde{\pi}_\ell(\eta) \right)^2- \left(\widetilde{\pi}_\ell(\eta)\right)^2\left( \widetilde{\vct{\pi}}(\eta)- \eb_\ell\right)^T\Vb\Sigmab \Deltab^{-1} \Sigmab\Vb^T \left(\widetilde{\vct{\pi}}(\eta) - \eb_\ell\right)\right)\\
F_2(\eta):=&\left(\vct{\pi}^T\vct{\nu}\left(\eta\right)-1\right)
\end{align*}









\newpage
Rewriting the objective above as
\begin{align*}
f_1\left(\frac{\beta}{\tau}\right)+\beta\tau f_2\left(\frac{\beta}{\tau}\right)
\end{align*}
Setting the derivatives with respect to $\beta$ and $\tau$ to zero we have
\begin{align*}
\frac{1}{\tau}f_1'\left(\frac{\beta}{\tau}\right)+\tau f_2\left(\frac{\beta}{\tau}\right)+\beta f_2'\left(\frac{\beta}{\tau}\right)=&0\\
-\frac{\beta}{\tau^2}f_1'\left(\frac{\beta}{\tau}\right)+\beta f_2\left(\frac{\beta}{\tau}\right)-\frac{\beta}{\tau^2}f_2'\left(\frac{\beta}{\tau}\right)=&0
\end{align*}
Multiplying the first identity by $\frac{\beta}{\tau}$ and summing it with the second we conclude that
\begin{align*}
\beta f_2\left(\frac{\beta}{\tau}\right)=0\quad \Rightarrow\quad \beta=0\quad\text{or}\quad \vct{\pi}^T\vct{\nu}\left(\frac{\beta}{\tau}\right)=1
\end{align*}
Thus $\eta:=\frac{\widehat{\beta}}{\widehat{\tau}}$ is the solution to $\vct{\pi}^T\vct{\nu}(\eta)=\frac{1}{\gamma}\left(\sum_{\ell=1}^k\frac{\pi_\ell\omega_\ell^2}{\omega_\ell^2+\eta}\right)=1$. 


\newpage
Next let us attempt to solve for $\tau$ using the first equation above combined with the fact $f_2\left(\frac{\beta}{\tau}\right)=0$ we conclude that
\begin{align*}
\frac{1}{\tau}f_1'\left(\frac{\beta}{\tau}\right)+\beta f_2'\left(\frac{\beta}{\tau}\right)=0\quad\Rightarrow\quad  f_1'(\eta)+\tau^2\eta f_2'(\eta)=0\quad\Rightarrow\quad \widehat{\tau}=\sqrt{-\frac{f_1'(\eta)}{\eta f_2'(\eta)}}
\end{align*}
So we need to calculate $f_1'(\eta)$ and $f_2'(\eta)$. To do this note that
\begin{align*}
f_1(\eta)=\frac{\gamma}{2}\eta \left(\pi_\ell\vct{\nu}_\ell\left(\eta\right) +  \begin{bmatrix} \alphab^T & b_\ell \end{bmatrix} \A\left(\eta\right)  \begin{bmatrix} \alphab \\ b_\ell  \end{bmatrix} - 2 \pi_\ell\vct{\nu}_\ell\left(\eta\right) \cb_\ell^T \begin{bmatrix} \alphab \\ b_\ell  \end{bmatrix}\right).
\end{align*}
Thus,
\begin{align*}
f_1'(\eta)=&\frac{\gamma}{2} \left(\pi_\ell\vct{\nu}_\ell\left(\eta\right) +  \begin{bmatrix} \alphab^T & b_\ell \end{bmatrix} \A\left(\eta\right)  \begin{bmatrix} \alphab \\ b_\ell  \end{bmatrix} - 2 \pi_\ell\vct{\nu}_\ell\left(\eta\right) \cb_\ell^T \begin{bmatrix} \alphab \\ b_\ell  \end{bmatrix}\right)\\
&+\frac{\eta}{2} \left(\pi_\ell\vct{\nu}_\ell'\left(\eta\right) +  \begin{bmatrix} \alphab^T & b_\ell \end{bmatrix} \A'\left(\eta\right)  \begin{bmatrix} \alphab \\ b_\ell  \end{bmatrix} - 2 \pi_\ell\vct{\nu}_\ell'\left(\eta\right) \cb_\ell^T \begin{bmatrix} \alphab \\ b_\ell  \end{bmatrix}\right)\\
=&\frac{\gamma}{2} \left(\pi_\ell\vct{\nu}_\ell\left(\eta\right) +  \begin{bmatrix} \alphab^T & b_\ell \end{bmatrix} \A\left(\eta\right)  \begin{bmatrix} \alphab \\ b_\ell  \end{bmatrix} - 2 \pi_\ell\vct{\nu}_\ell\left(\eta\right) \cb_\ell^T \begin{bmatrix} \alphab \\ b_\ell  \end{bmatrix}\right)\\
&+\frac{\eta\gamma}{2} \left(\pi_\ell\nu_\ell'(\eta) +  \begin{bmatrix} \alphab^T & b_\ell \end{bmatrix} \A'\left(\eta\right)  \begin{bmatrix} \alphab \\ b_\ell  \end{bmatrix} - 2 \pi_\ell\nu_\ell'(\eta)  \cb_\ell^T \begin{bmatrix} \alphab \\ b_\ell  \end{bmatrix}\right)
\end{align*}
where
\begin{align*}
\vct{\nu}'(\eta)=-\frac{1}{\gamma}\begin{bmatrix}\frac{\omega_1^2}{(\omega_1^2+\eta)^2}\\\frac{\omega_2^2}{(\omega_2^2+\eta)^2}\\\ldots \\\frac{\omega_k^2}{(\omega_k^2+\eta)^2}\end{bmatrix}\quad\text{and}\quad \A'(\eta):=&\begin{bmatrix} \sigma^2\left(\vct{\pi}^T\vct{\nu}'(\eta)\right)\Iden_r+\Sigmab\Vb^T\text{diag}\left(\vct{\pi}\right)\text{diag}\left(\vct{\nu}'(\eta)\right)\Vb\Sigmab & \Sigmab\Vb^T\text{diag}\left(\vct{\nu}'(\eta)\right)\vct{\pi} \\ 
\vct{\pi}^T\text{diag}\left(\vct{\nu}'(\eta)\right)\Vb\Sigmab & \vct{\pi}^T\vct{\nu}'(\eta) \end{bmatrix}
\end{align*}
Also
\begin{align*}
f_2(\eta):=\frac{1}{2}\left(1-\frac{1}{\vct{\pi}^T\vct{\nu}(\eta)}\right)\quad\Rightarrow\quad f_2'(\eta)=\frac{\vct{\pi}^T\vct{\nu}'(\eta)}{2(\vct{\pi}^T\vct{\nu}(\eta))^2}=\frac{\vct{\pi}^T\vct{\nu}'(\eta)}{2}
\end{align*}
Thus,
{\tiny
\begin{align}
\label{tauhat}
\widehat{\tau}=\sqrt{-\frac{2}{\eta(\vct{\pi}^T\vct{\nu}'(\eta))}\left(\frac{\gamma}{2} \left(\pi_\ell\vct{\nu}_\ell\left(\eta\right) +  \begin{bmatrix} \alphab^T & b_\ell \end{bmatrix} \A\left(\eta\right)  \begin{bmatrix} \alphab \\ b_\ell  \end{bmatrix} - 2 \pi_\ell\vct{\nu}_\ell\left(\eta\right) \cb_\ell^T \begin{bmatrix} \alphab \\ b_\ell  \end{bmatrix}\right)+\frac{\eta\gamma}{2} \left(\pi_\ell\nu_\ell'(\eta) +  \begin{bmatrix} \alphab^T & b_\ell \end{bmatrix} \A'\left(\eta\right)  \begin{bmatrix} \alphab \\ b_\ell  \end{bmatrix} - 2 \pi_\ell\nu_\ell'(\eta)  \cb_\ell^T \begin{bmatrix} \alphab \\ b_\ell  \end{bmatrix}\right)\right)}
\end{align}
}

Thus the AO optimization problem reduces to
\begin{align*}
\min_{ \vct{b}_\ell}\text{ }\min_{\vct{\alpha}}\text{ }\frac{\eta\gamma}{2}\left(\pi_\ell\vct{\nu}_\ell +  \begin{bmatrix} \alphab^T & b_\ell \end{bmatrix} \A  \begin{bmatrix} \alphab \\ b_\ell  \end{bmatrix} - 2 \pi_\ell\vct{\nu}_\ell \cb_\ell^T \begin{bmatrix} \alphab \\ b_\ell  \end{bmatrix}\right)
\end{align*}
where $\eta$ is the solution to
\begin{align*}
\sum_{\ell=1}^k\frac{\pi_\ell\omega_\ell^2}{\omega_\ell^2+\eta}=\gamma
\end{align*}
and
\begin{align}\label{eq:Amatnew22}
\A(\eta):=&\begin{bmatrix} \sigma^2\Iden_r+\Sigmab\Vb^T\text{diag}\left(\vct{\pi}\odot\vct{\nu}\right)\Vb\Sigmab & \Sigmab\Vb^T\left(\vct{\pi}\odot\vct{\nu}\right) \\ 
\left(\vct{\pi}\odot\vct{\nu}\right)^T\Vb\Sigmab & 1 \end{bmatrix}\nonumber\\
\cb_\ell :=& \begin{bmatrix} \Sigmab\Vb^T\eb_\ell \\ 1 \end{bmatrix}
\end{align}
where
\begin{align*}
\vct{\nu}:=\frac{1}{\gamma}\begin{bmatrix}\frac{\omega_1^2}{\omega_1^2+\eta}\\\frac{\omega_2^2}{\omega_2^2+\eta}\\\ldots \\\frac{\omega_k^2}{\omega_k^2+\eta}\end{bmatrix}
\end{align*}

First, note that the matrix $\A$ is positive definite. This can be checked by computing the Schur complement of $\A$:
\begin{align}\label{eq:Deltab_def2}
\Deltab:=\sigma^2\Iden_r+\Sigmab\Vb^T\Pb\Vb\Sigmab:=\sigma^2\Iden_r+\Sigmab\Vb^T\left(\diag{\pib\odot\vct{\nu}}-\left(\pib\odot\vct{\nu}\right)\left(\pib\odot\vct{\nu}\right)^T\right)\Vb\Sigmab \succ \zero_{r\times r}.
\end{align}
Positive definiteness above holds because $\Pb:=\left(\diag{\pib\odot\vct{\nu}}-\left(\pib\odot\vct{\nu}\right)\left(\pib\odot\vct{\nu}\right)^T\right)\succeq \zero_{k\times k}$. Thus the objective is a strictly convex quadratic and is jointly convex in its arguments. We proceed by minimizing the objective over $(\alphab,b_\ell)$ which is equal to
\bea
\begin{bmatrix} \widehat\alphab \\ \widehat b_\ell \end{bmatrix} = \pi_\ell\nu_\ell \A^{-1} \cb_\ell = \pi_\ell \nu_\ell\begin{bmatrix} -\Deltab^{-1}\Sigmab\Vb^T(\pib\odot\vct{\nu}-\eb_\ell) \\ 1+\left(\pib\odot\vct{\nu}\right)^T\Vb\Sigmab\Deltab^{-1}\Sigmab\Vb^T(\pib\odot\vct{\nu}-\eb_\ell) \end{bmatrix}\label{eq:alphab_1t}
%\\
%&= \pi_\ell \begin{bmatrix} -\Sigmab^{-1}\Vb^T\left(\Vb\Sigmab^{-2}\Vb^T+\Pb\right)^{-1}(\pib-\eb_\ell) \\ 1+\pib^T\left(\Vb\Sigmab^{-2}\Vb^T+\Pb\right)^{-1}(\pib-\eb_\ell), \end{bmatrix}\nn\\
%&= \pi_\ell \begin{bmatrix} -\Sigmab^{-1}\Vb^T\left(\Vb\Sigmab^{-2}\Vb^T+\Pb\right)^{-1}(\pib-\eb_\ell) \\ \frac{1-\pib^T\left(\Vb\Sigmab\Vb^T+\diag{\pib}\right)^{-1}\eb_\ell}{1-\pib^T\left(\Vb\Sigmab\Vb^T+\diag{\pib}\right)^{-1}\pib}, 
%\end{bmatrix}
\end{align}
%where the last two equalities follow from the Matrix inversion formula  and some algebra (see Lemma \ref{lem:pi_vec}). 
Thus, the minimum value attained is
\begin{align}
&-\pi_\ell^2\nu_\ell^2  \begin{bmatrix} -\left(\pib\odot\vct{\nu} - \eb_\ell\right)^T\Vb\Sigmab && 1 \end{bmatrix} \begin{bmatrix} \Deltab^{-1} & \zero \\ \zero^T & 1 \end{bmatrix}\begin{bmatrix} -\Sigmab\Vb^T \left(\pib\odot\vct{\nu} - \eb_\ell\right) \\ 1 \end{bmatrix} \\
&= - \pi_\ell^2\nu_\ell^2\left(1+\left(\pib\odot\vct{\nu} - \eb_\ell\right)^T\Vb\Sigmab \Deltab^{-1} \Sigmab\Vb^T \left(\pib\odot\vct{\nu} - \eb_\ell\right)\right).  \nn%\nn\\
%&= - \pi_\ell^2\left(1+\left(\pib - \eb_\ell\right)^T \left(\Vb^T\Sigmab^{-2}\Vb^T+\Pb\right)^{-1} \left(\pib - \eb_\ell\right)\right) .
\end{align}
Thus the objective reduces to
\begin{align}
\frac{\eta \gamma}{2}\left(\pi_\ell\nu_\ell - \pi_\ell^2\nu_\ell^2\left(\pib\odot\vct{\nu} - \eb_\ell\right)^T\Vb\Sigmab \Deltab^{-1} \Sigmab\Vb^T \left(\pib\odot\vct{\nu} - \eb_\ell\right)\right).
\label{eq:final}
\end{align}

%{\color{blue} Need to check that the term in the square-root is non-negative}

\vp
\noindent\textbf{Asymptotic predictions.}~~First, from \eqref{eq:alphab_1t} the bias term converges as follows:
$$
\widehat{b}_\ell \rP \pi_\ell\nu_\ell\left(1+\left(\pib\odot\vct{\nu}\right)^T\Vb\Sigmab\Deltab^{-1}\Sigmab\Vb^T(\pib\odot\vct{\nu}-\eb_\ell)\right).
$$
Thus,
\begin{align*}
\widehat{\vct{b}}\rP\left(\mtx{I}_k-\mtx{P}\Vb\Sigmab\Deltab^{-1}\Sigmab\Vb^T \right)\left(\pib\odot \vct{\nu}\right)
\end{align*}
 Recall that $\alphab = \Ub^T\w_\ell$. Thus, the correlations $\inp{\mub_i}{\w_\ell},~i\in[k]$ converge as follows:
\begin{align}
\M^T\w_\ell = \Vb\Sigmab\Ub^T\w_\ell \rP \Vb\Sigmab\widehat\alphab = -\pi_\ell\nu_\ell\Vb\Sigmab\Deltab^{-1}\Sigmab\Vb^T\left(\pib\odot\vct{\nu}-\eb_\ell\right).\quad
\end{align}
Here, convergence applies element-wise to the entries of the involved random vectors. Moreover, from the analysis above we can predict the limit of the norm $\twonorm{\w_\ell}$. For this, note that $\twonorm{\w_\ell}^2 = \widehat{\alpha}_0^2 + \widehat{\alphab}^T\widehat{\alphab}$. To continue further note that based on \eqref{myalphahat} we have
\begin{align*}
\widehat{\alpha}_0=\frac{\sqrt{\gamma}\tau}{\frac{\sigma}{n} \text{trace}\left(\left(\mtx{I}+\frac{\beta}{\tau}\mtx{D}^{-2}\right)^{-1}\right)}\rP\frac{\widehat{\tau}}{\sigma \sqrt{\gamma}}
\end{align*}


 Thus,
\begin{align}\label{eq:norm_lim}
\twonorm{\w_\ell}^2 \rP \frac{\gamma}{(1-\gamma)\sigma^2}\pi_\ell(1-\pi_\ell)  + \pi_\ell^2 \left(\pib - \eb_\ell\right)^T\Vb\Sigmab \Deltab^{-1} \left(\Deltab^{-1} - \frac{\gamma}{(1-\gamma)\sigma^2}\Iden_{r}\right) \Sigmab\Vb^T \left(\pib - \eb_\ell\right) 
\end{align}



\subsection{Computing cross-correlations}\label{sec:cross_LS_GM}
In the previous section we used the CGMT to predict the bias $\widehat{b}_\ell$, the correlations $\inp{\mub_i}{\wh_\ell},~i[k]$ and the norm $\twonorm{\wh_\ell}$ for all $\ell\in[k]$ members of the multi-output classifier. Here, we show how to compute the limits of the cross-correlations $\inp{\wh_\ell}{\wh_j}, \ell\neq j\in [k]$.

\begin{lemma}\label{lem:joint_LS}
For $\ell\neq j\in[k]$ let $\wh_\ell$ $\wh_j$ be solutions to the least-squares minimization \eqref{eq:LS_def}, i.e.,
$$
(\wh_\ell,\wh_j,\widehat{b}_\ell,\widehat{b}_j) =  \arg\min_{\w_\ell, \w_j, b_\ell, b_j} \left\{ \frac{1}{2n}\twonorm{\Y_{\ell} - \X^T \w_\ell - b_\ell\one_n }^2 + \frac{1}{2n}\twonorm{\Y_{j} - \X^T \w_j - b_j\one_n }^2\right\}.
$$
 Denote $\wh_{\ell,j}:=\wh_\ell+\wh_j$ and $\widehat{b}_{\ell,j}:=\widehat{b}_\ell+\widehat{b}_j$. Then, $(\wh_{\ell,j},\widehat{b}_{\ell,j})$ is a minimizer in the following least-squares problem:
\begin{align}\label{eq:joint_LS}
(\wh_{\ell,j},\widehat{b}_{\ell,j}) = \arg\min_{\w, b} \frac{1}{2n}\twonorm{\Y_{\ell} + \Y_{j} - \X^T \w - b\one_n }^2
\end{align}
\end{lemma}
\begin{proof}
Clearly the minimization in \eqref{eq:joint_LS} is convex. Thus, it suffices to prove that $\wh_\ell+\wh_j$ satisfies the KKT conditions. First, by optimality of $\wh_\ell$, we have that 
$$
\X\left(\Y_\ell-\X^T\wh_\ell-\widehat{b}_\ell\one_n\right) = 0
$$
Similarly, for $\wh_j$:
$$
\X\left(\Y_j-\X^T\wh_j-\widehat{b}_j\one_n\right) = 0.
$$
Adding the equations on the above displays we find that
$$
\X\left(\Y_\ell+\Y_j-\X^T(\wh_j+\wh_\ell)-(\widehat{b}_j+\widehat{b}_\ell)\one_n\right) = 0.
$$
Recognize that this coincides with the optimality condition for \eqref{eq:joint_LS}. Thus, the proof is complete.
\end{proof}


Thanks to Lemma \ref{lem:joint_LS}, we can use the CGMT to characterize the limiting behavior of $\twonorm{\wh_\ell+\wh_j}$. Observe that this immediately gives the limit of $\inp{\wh_\ell}{\wh_j}$ since 
\begin{align}\label{eq:inp_from_norms}
\inp{\wh_\ell}{\wh_j} = \frac{\twonorm{\wh_\ell+\wh_j}^2-\twonorm{\wh_\ell}^2-\twonorm{\wh_j}^2}{2}.
\end{align} 

The analysis of \eqref{eq:joint_LS} is very similar to that of \eqref{eq:LS_PO}; thus, most details are omitted. Similar to \eqref{eq:scal_AO} we can relate \eqref{eq:joint_LS} with the following AO problem:
\begin{align}
\bar\phi_{AO,\ell,j}(\g,\h)&:=  \min_{\beta_0\geq 0, \vct{\beta}\in\R^r, b_{\ell,j}}\text{ } \frac{1}{\sqrt{n}}\twonorm{ \sigma\sqrt{\beta_0^2 + \twonorm{\vct{\beta}}^2}\,\vct{g}+\mtx{Y}^T\mtx{V}\mtx{\Sigma}\vct{\beta}  +b_{\ell,j}\vct{1}_n-\mtx{Y}_\ell - \Y_j}\nonumber\\
&\quad\quad\quad\quad\quad\quad\quad+ \sigma\sum_{i=1}^{r}{\beta_i\frac{\vct{h}^T\ub_i}{\sqrt{n}}} -\sigma\beta_0\frac{\twonorm{\h^\perp}}{\sqrt{n}},\label{eq:scal_AO_ij}
\end{align}
where we have decomposed 
$$
\w_{\ell,j} = \sum_{i=1}^{r}\beta_i \ub_i + \beta_0\w_{\ell,j}^\perp, 
$$
with $\twonorm{\w_{\ell,j}^\perp}=1$ and $\Ub^T\w_{\ell,j}^\perp=\zero_r$.

Using a calculation similar to the one leading to \eqref{eq:det_21} we can show that \eqref{eq:scal_AO_ij} converges point-wise in $\beta_0,\betab=\begin{bmatrix}\beta_1,\ldots,\beta_r\end{bmatrix}, b$ to the following:
\begin{align}
\Dc_\ell(\beta_0,\betab,b_{\ell,j}) = \sqrt{\beta_0^2\sigma^2 + \pi_\ell + \pi_j +  \begin{bmatrix} \betab^T & b_{\ell,j} \end{bmatrix} \A  \begin{bmatrix} \betab \\ b_{\ell,j}  \end{bmatrix} - 2  \db_{\ell,j}^T \begin{bmatrix} \betab \\ b_{\ell,j}  \end{bmatrix}} - \beta_0\sigma\sqrt{\gamma}\label{eq:det_2},
\end{align}
where $\A$ is as in \eqref{eq:Amat} and we have further defined
$$
\db_{\ell,j} := \begin{bmatrix} \pi_\ell\Sigmab\Vb^T\eb_\ell + \pi_j\Sigmab\Vb^T\eb_j \\ \pi_\ell+\pi_j \end{bmatrix}.
$$
Thus,  similar to \eqref{eq:alphab_1} we can compute the minimizer of the deterministic 
\bea
\begin{bmatrix} \widehat\betab \\ \widehat b_{\ell,j} \end{bmatrix} = \begin{bmatrix} - \Deltab^{-1}\Sigmab\Vb^T\left(\pi_\ell(\pib-\eb_\ell) + \pi_j (\pib-\eb_j)\right) \\ \pi_\ell + \pi_j +\pib^T\Vb\Sigmab\Deltab^{-1}\Sigmab\Vb^T\left(\pi_\ell(\pib-\eb_\ell) +\pi_j(\pib-\eb_j) \right) \end{bmatrix}
%\\
%&= \pi_\ell \begin{bmatrix} -\Sigmab^{-1}\Vb^T\left(\Vb\Sigmab^{-2}\Vb^T+\Pb\right)^{-1}(\pib-\eb_\ell) \\ 1+\pib^T\left(\Vb\Sigmab^{-2}\Vb^T+\Pb\right)^{-1}(\pib-\eb_\ell), \end{bmatrix}\nn\\
%&= \pi_\ell \begin{bmatrix} -\Sigmab^{-1}\Vb^T\left(\Vb\Sigmab^{-2}\Vb^T+\Pb\right)^{-1}(\pib-\eb_\ell) \\ \frac{1-\pib^T\left(\Vb\Sigmab\Vb^T+\diag{\pib}\right)^{-1}\eb_\ell}{1-\pib^T\left(\Vb\Sigmab\Vb^T+\diag{\pib}\right)^{-1}\pib}, 
%\end{bmatrix}
\end{align}
and 
\begin{align}
\widehat\beta_0 =\frac{1}{\sigma} \sqrt\frac{\gamma}{1-\gamma}\sqrt{\pi_\ell+\pi_j - (\pi_\ell+\pi_j)^2 - \left(\pi_\ell\left(\pib - \eb_\ell\right)+\pi_j\left(\pib - \eb_j\right)\right)^T\Vb\Sigmab \Deltab^{-1} \Sigmab\Vb^T \left(\pi_\ell\left(\pib - \eb_\ell\right)+\pi_j\left(\pib - \eb_j\right)\right)},
\end{align}
where recall that $\Deltab$ is as in \eqref{eq:Deltab_def}.

From the CGMT, we have that 
$\twonorm{\wh_{\ell}+\wh_{j}}^2 \rP \widehat\betab_0^2+\twonorm{\betab}^2.$ 
Combining this with the calculations above, we conclude that
\begin{align}\label{eq:joint_norm_lim}
\twonorm{\wh_{\ell}+\wh_{j}}^2 &\rP \frac{\gamma}{(1-\gamma)\sigma^2}\left(\pi_\ell+\pi_j\right)\left(1-\pi_\ell-\pi_j\right)\nn \\&+  \left(\pi_\ell\left(\pib - \eb_\ell\right)+\pi_j\left(\pib - \eb_j\right)\right)^T\Vb\Sigmab \Deltab^{-1} \left(\Deltab^{-1} - \frac{\gamma}{(1-\gamma)\sigma^2}\Iden_r\right) \Sigmab\Vb^T \left(\pi_\ell\left(\pib - \eb_\ell\right)+\pi_j\left(\pib - \eb_j\right)\right)
\end{align}

Finally, using \eqref{eq:joint_norm_lim} and \eqref{eq:norm_lim} in \eqref{eq:inp_from_norms} it follows that
\begin{align}
\inp{\w_\ell}{\w_j} \rP \pi_\ell\pi_j\left( - \frac{\gamma}{(1-\gamma)\sigma^2}  +  \left(\pib - \eb_\ell\right)^T\Vb\Sigmab \Deltab^{-1} \left(\Deltab^{-1} - \frac{\gamma}{(1-\gamma)\sigma^2}\Iden_r\right) \Sigmab\Vb^T \left(\pib - \eb_j\right) \right).
\end{align}

\section{Random idea}
We are interested in
$$
(\wh_\ell,\wh_j,\widehat{b}_\ell,\widehat{b}_j) =  \arg\min_{\w_\ell, \w_j, b_\ell, b_j} \left\{ \frac{1}{2n}\twonorm{\mtx{D}_\ell\left(\Y_{\ell} - \X^T \w_\ell - b_\ell\one_n \right)}^2 + \frac{1}{2n}\twonorm{\mtx{D}_j\left(\Y_{j} - \X^T \w_j - b_j\one_n\right) }^2\right\}.
$$
How about rewriting the loss above in the form

$$
(\wh,\widehat{\vct{\omega}},\widehat{b},\widehat{\beta}) =  \arg\min_{\w,\vct{\omega},b,\beta} \left\{ \frac{1}{2n}\twonorm{\mtx{D}_\ell\left(\Y_{\ell} - \X^T (\w+\vct{\omega}) - (b+\beta)\one_n \right)}^2 + \frac{1}{2n}\twonorm{\mtx{D}_j\left(\Y_{j} - \X^T(\w-\vct{\omega}) - (b-\beta)\one_n\right) }^2\right\}.
$$


==> WLS_MLM_backup.tex <==
\section{Weighted LS -- MLM}

Let $\Db$ be a diagonal matrix with non-zero diagonal entries.
and consider the weighted least-squares (WLS) solution:
\begin{align}
(\widehat\w_\ell,\widehat b) = \arg\min_{\w,b}\mathcal{L}_{PO}\left(\w,b\right):=\frac{1}{2n}\twonorm{\Db\left(\X^T\w+b\vct{1}_n-\mtx{Y}_\ell\right)}^2\nn
\end{align}
In fact, it is convenient to rewrite the above as folows:
\begin{align}\label{eq:PO_WLS}
(\widehat\w_\ell,\widehat b) = \arg\min_{\w,b,\ub}~\max_{\s}~\frac{1}{n}\left(\s^T\Db\X^T\w+b\s^T\Db\vct{1}_n\s^T\Db\mtx{Y}_\ell -\s^T\ub + \frac{\twonorm{\ub}^2}{2}\right).
\end{align}

\subsubsection{Identifying the AO.}%\label{sec:MLM_AO}
The PO in \eqref{eq:PO_WLS} is very similar to \eqref{eq:LS_log_PO}. In particular, following step by step the same decomposition trick as in Section \ref{sec:MLM_AO}, it can be shown that the AO corresponding to \eqref{eq:PO_WLS} becomes (cf. \eqref{eq:MLM_AO}) 
\begin{align*}
\min_{\vct{w}_\ell, \vct{b}_\ell,\ub}\text{ }\max_{\vct{s}}\text{ }\frac{1}{n}\left( \twonorm{\Pb^\perp\vct{w}_\ell}\vct{g}^T\Db\vct{s}+ \twonorm{\Db\vct{s}}\vct{h}^T\Pb^\perp\vct{w}_\ell+ \vct{s}^T\Db\Gt^T\Ub^T\vct{w}_\ell+b_\ell\vct{s}^T\Db\vct{1}_n-\vct{s}^T\Db\mtx{Y}_\ell - \ub^T\s + \frac{\twonorm{\vct{\ub}}^2}{2}\right), 
\end{align*}
where we use the same notation as in Section \ref{sec:MLM_AO} for $\Pb^\perp, \Ub, \Gt, \g$ and $\h$. Recall also the relation of $\Y_\ell$ to $\Gt$ in \eqref{eq:Y_to_gt}.

\subsubsection{Scalarization of the AO.}%\label{sec:MLM_AO}
We start the process of simplifying the AO by setting $\beta:=\twonorm{\Db\s}\big/\sqrt{n}$ and optimizing over the direction of $\Db\s$ to equivalently write the AO as
\begin{align}\label{eq:koko_WLS}
\min_{\vct{w}_\ell, \vct{b}_\ell,\ub}\text{ }\max_{\beta\geq0}\text{ }\frac{1}{\sqrt{n}}\left( \beta\twonorm{ \twonorm{\Pb^\perp\vct{w}_\ell}\vct{g}+ \Gt^T\Ub^T\vct{w}_\ell+b_\ell\vct{1}_n-\mtx{Y}_\ell - \Db^{-1}\ub} + \beta \vct{h}^T\Pb^\perp\vct{w}_\ell \right) + \frac{\twonorm{\vct{\ub}}^2}{2n}, 
\end{align}
Next, focus on the minimization over $\w_\ell$. Let us denote
$$
\ab:=\Ub^T\w_\ell\quad\text{and}\quad \alpha_0 = \twonorm{\Pb^\perp\w_\ell}.
$$
Notice that $\ab\perp \Pb^\perp\w_\ell$ and thus the orthogonal decomposition $\w_\ell=\Ub\ab + \Pb^\perp\w_\ell$. With this observation, note that the optimal direction of $\Pb^T\w_\ell$ in \eqref{eq:koko_WLS} aligns with $\Pb^T\h$ for all values of $\beta$. Therefore, \eqref{eq:koko_WLS} reduces to 
\begin{align}\label{eq:koko_WLS_1}
\min_{\ab, \alpha_0\geq0, \vct{b}_\ell,\ub}\text{ }\max_{\beta\geq0}\text{ }\frac{1}{\sqrt{n}}\left( \beta\twonorm{ \alpha_0\vct{g}+ \Gt^T\ab+b_\ell\vct{1}_n-\mtx{Y}_\ell - \Db^{-1}\ub}  - \beta\alpha_0 \twonorm{\Pb^\perp\h} \right)+ \frac{\twonorm{\vct{\ub}}^2}{2n}, 
\end{align}
Continuing let us denote $\tb:=\alpha_0\vct{g}+ \Gt^T\ab+b_\ell\vct{1}_n-\mtx{Y}_\ell$ for convenience and rewrite $\twonorm{\tb-\Db^{-1}\ub}$ as follows
$$
\frac{\twonorm{\tb-\Db^{-1}\ub}}{\sqrt{n}} = \min_{\tau>0}~\frac{\tau}{2} + \frac{\twonorm{\tb-\Db^{-1}\ub}^2}{2\tau n}.
$$
Note that the resulting minimization is convex in $\ub$ and concave in $\beta$. Also, by considering the bounded AO (such that $\beta$ is bounded \CT{Need to explain more}), we can flip the order of min-max and optimize over $\ub$ first. In particular, $\ub$ minimizes the following strictly convex quadratic
\bea
\min_{\ub}\left\{ \frac{1}{n}\left(\frac{\beta}{2\tau}\twonorm{\Db^{-1}\ub} + \frac{1}{2}\twonorm{\ub}^2 - \frac{\beta}{\tau}\tb^T\Db^{-1}\ub \right) = \frac{1}{2n}\ub^T\left(\frac{\beta}{\tau}\Db^{-2} + \Iden_n \right)\ub-\frac{\beta}{\tau n}\tb^T\Db^{-1}\ub  \right\}.\nn
\end{align}
In particular,
$$
\ub = \frac{\beta}{\tau}\left(\frac{\beta}{\tau}\Db^{-2}+\Iden\right)^{-1} \Db^{-1} \tb = \left(\Db^{-1}+\frac{\tau}{\beta}\Db\right)^{-1}\left(\alpha_0\vct{g}+ \Gt^T\ab+b_\ell\vct{1}_n-\mtx{Y}_\ell\right)
$$
Putting things together, the new objective function of \eqref{eq:koko_WLS_1} becomes \CT{Check convexity}
\bea
&\min_{\ab,\alpha_0\geq0 ,b_\ell,\tau>0}~~\max_{\beta\geq 0}~~\Rc(\ab,\alpha_0,b_\ell,\tau,\beta)\label{eq:koko2_WLS}\\
&\qquad\text{where}~~\Rc(\ab,\alpha_0,b_\ell,\tau,\beta):=\frac{\beta\tau}{2n}+ \frac{\beta}{2\tau n}\twonorm{\tb}^2 -\frac{\beta}{2\tau n} \tb^T\left(\Iden + \frac{\tau}{\beta}\Db^2\right)^{-1}\tb - \frac{{\beta\alpha_0}}{\sqrt{n}}\twonorm{\Pb^\perp\h}\nn.
\end{align}

\subsubsection{Convergence of the AO}
After having simplified the AO into an optimization problem over $r+4$ variables, we are ready to study its asymptotic behavior. First, we argue on point-wise convergence of $\Rc$ in \eqref{eq:koko2_WLS}. Fix $\ab,\alpha_0,\bb_\ell,\tau$ and $\beta$. From the WLLN, $\frac{1}{\sqrt{n}} \twonorm{\Pb^\perp\h}\rP\sqrt{\gamma}$ and as in \eqref{eq:t_conv}
\bea\nn
\frac{1}{n}\twonorm{ \tb}^2 = \frac{1}{n}\sum_{i=1}^n\left({\alpha_0\g_i+\ab^T\gt_i+b_\ell-[\Y_\ell]_i}\right)^2 \rP \E\left[\left({\alpha_0G_0+\ab^T\g+\bb_\ell-Y_\ell}\right)^2\right],
\end{align}
where the expectation is over $\g\sim\Nn(\zero_r,\Iden_r)$ (with some abuse of notation) and 
\begin{align}
Y_\ell \sim{\rm Bern}(V_\ell)\quad\text{and}\quad V_\ell=\frac{e^{\eb_\ell^T\Vb\Sigmab\g}}{\sum_{\ell^\prime=1}^{r}e^{\eb_{\ell^\prime}\Vb\Sigmab\g}}.\label{eq:Y_ell_log_WLS}
\end{align}
Furthermore,
\bea
\frac{1}{n}\tb^T\left(\Iden + \frac{\tau}{\beta}\Db^2\right)^{-1}\tb  = \frac{1}{n}\sum_{i=1}^{n}\frac{\left({\alpha_0\g_i+\ab^T\gt_i+b_\ell-[\Y_\ell]_i}\right)^2 }{1+\frac{\tau}{\beta}\left(\omega[\Y_\ell]_{i}+1\right)} \rP \E\left[\frac{\left({\alpha_0G_0+\ab^T\g+\bb_\ell-Y_\ell}\right)^2}{1+\frac{\tau}{\beta}\left(\omega Y_\ell+1\right)}\right] \nn
\end{align}


 Therefore, point-wise on $\ab,\alpha_0,\bb_\ell,\tau$ and $\beta$, the objective $\Rc$ of the AO converges to 
\begin{align}
\Dc_\ell(\alpha_0,\alphab,b_\ell,\tau,\beta)&:=\frac{\beta\tau}{2} + \frac{\beta}{2\tau}\E\left[\left({\alpha_0G_0+\ab^T\g+\bb_\ell-Y_\ell}\right)^2\right] - \frac{\beta}{2\tau} \E\left[\frac{\left({\alpha_0G_0+\ab^T\g+\bb_\ell-Y_\ell}\right)^2}{1+\frac{\tau}{\beta}\left(\omega Y_\ell+1\right)}\right] - \beta\alpha_0 \sqrt{\gamma}\nn\\
&=\frac{\beta\tau}{2} + \frac{1}{2} \E\left[\frac{\left(\omega Y_\ell+1\right)\left({\alpha_0G_0+\ab^T\g+\bb_\ell-Y_\ell}\right)^2}{1+\frac{\tau}{\beta}\left(\omega Y_\ell+1\right)}\right] - \beta\alpha_0 \sqrt{\gamma}\nn\\
&=\frac{\beta\tau}{2} + \frac{1}{2} \E\left[\frac{\left({\alpha_0G_0+\ab^T\g+\bb_\ell-Y_\ell}\right)^2}{\left(\omega Y_\ell+1\right)^{-1}+\left({\tau}/{\beta}\right)}\right] - \beta\alpha_0 \sqrt{\gamma}.\label{eq:det_log_WLS}
\end{align}

It can be checked that the function above is jointly convex in $(\alpha_0,\alphab,b_\ell,\tau)$ and concave in $\beta$ \CT{Need to check joint convexity. Convexity with $\tau$ and $\beta$ checked by differentiation.}

{\color{blue} Use convexity to argue uniform convergence}


\subsection{Deterministic Analysis of the AO}

\subsubsection{}
\begin{align}\label{eq:Db_ell}
\Db = \diag{ \omega \Y_\ell + \one_n },\quad \omega\geq 0.
\end{align}


It can be checked that the first order optimality conditions of $\Dc_\ell(\alpha_0,\alphab,b_\ell,\tau,\beta)$ with respect to $\beta$ and $\tau>0$ are given as follows:
\bea
\beta^2 &= \E\left[\frac{\left({\alpha_0G_0+\ab^T\g+\bb_\ell-Y_\ell}\right)^2}{\left(\left(\omega Y_\ell+1\right)^{-1}+\left({\tau}/{\beta}\right)\right)^2}\right]\quad\text{or}\quad \beta = 0, \nn\\
\alpha_0\sqrt{\gamma} &= \frac{\tau}{2} + \frac{\tau}{2\beta^2}\cdot\E\left[\frac{\left({\alpha_0G_0+\ab^T\g+\bb_\ell-Y_\ell}\right)^2}{\left(\left(\omega Y_\ell+1\right)^{-1}+\left({\tau}/{\beta}\right)\right)^2}\right].
\end{align}
Thus, at optimality either $\beta=0$ or $\tau=\alpha_0\sqrt{\gamma}$. 
In what follows, consider the solution $\tau=\alpha_0\sqrt{\gamma}$. We will show that this leads to the true saddle point of $\Dc$.



Moreover, by denoting $\eta:=\frac{\tau}{\beta}$ and recalling from \eqref{eq:Y_ell_log_WLS} that $Y_\ell={\rm Bern}(V_\ell)$, we can express $\Dc_\ell(\alpha_0,\alphab,b_\ell,\tau,\beta)$ as follows
\begin{align}\label{eq:beta2_WLS}
\frac{\beta\tau}{2} +  \frac{\alpha_0^2}{2}\E\left[\frac{1}{\frac{1}{\omega Y_\ell+1}+\eta}\right] - \beta\alpha_0\sqrt\gamma + \frac{1}{2}\begin{bmatrix} \ab^T & \bb_\ell \end{bmatrix}\cdot\A\left(\eta\right)\cdot \begin{bmatrix} \ab \\ \bb_\ell \end{bmatrix} - \cb^T\left(\eta\right) \begin{bmatrix} \ab^T \\ \bb_\ell \end{bmatrix} + \frac{1}{2}\E\left[\frac{Y_\ell^2}{\frac{1}{\omega Y_\ell+1}+\eta}\right],
%\frac{\beta_\ell^2}{2}\E\left[\frac{1}{\frac{1}{\omega Y_\ell+1}+\eta}\right] - \beta_\ell \E\left[\frac{{Y_\ell-\ab^T\g}}{\frac{1}{\omega Y_\ell+1}+\eta}\right]
% \frac{1}{2} \E\left[\frac{\left({\alpha_0G_0+\ab^T\g+\bb_\ell-Y_\ell}\right)^2}{\frac{1}{\omega Y_\ell+1}+\eta}\right] - \beta\alpha_0 \sqrt{\gamma}\nn\\
\end{align}
where
\begin{align}
\A\left(\eta\right)&:= \begin{bmatrix} \E\left[\frac{\g\g^T}{\frac{1}{\omega Y_\ell+1}+\eta}\right] 
&
\E\left[\frac{\g}{\frac{1}{\omega Y_\ell+1}+\eta}\right] 
\\
\E\left[\frac{\g^T}{\frac{1}{\omega Y_\ell+1}+\eta}\right] 
&
\E\left[\frac{1}{\frac{1}{\omega Y_\ell+1}+\eta}\right] 
\end{bmatrix} = \left(\frac{1}{\frac{1}{\omega+1} + \eta}\right) \underbrace{ \E\left[\begin{bmatrix} \g \\ 1 \end{bmatrix}\begin{bmatrix} \g^T & 1 \end{bmatrix} V_\ell \right] }_{=:\A_1}+ \left(\frac{1}{1 + \eta}\right) \underbrace{\E\left[\begin{bmatrix} \g \\ 1 \end{bmatrix}\begin{bmatrix} \g^T & 1 \end{bmatrix} (1-V_\ell) \right]}_{=:\A_2}
\\
\cb\left(\eta\right)&:= \begin{bmatrix} \E\left[\frac{\g Y_\ell}{\frac{1}{\omega Y_\ell+1}+\eta}\right] \\
 \E\left[\frac{Y_\ell}{\frac{1}{\omega Y_\ell+1}+\eta}\right]  
\end{bmatrix} = \left(\frac{1}{\frac{1}{\omega+1} + \eta}\right) \underbrace{\E\left[\begin{bmatrix} \g \\ 1 \end{bmatrix} V_\ell \right]}_{=:\cb_1}.
\end{align}
we have the following first-order optimality conditions for $\alpha_0,\ab$ and $\bb_\ell$:
%By direct differentiation, we can compute the optimal values of $\alpha_0$ and $\bb_\ell$:
\bea
\begin{bmatrix}
\ab \\ \bb_\ell
\end{bmatrix} &= \A^{-1}\left(\eta\right)\cdot \cb\left(\eta\right)\label{eq:WLS_ab}\\
\alpha_0 &= \beta\sqrt{\gamma}\Big/ \E\left[\frac{1}{\frac{1}{\omega Y_\ell+1}+\eta}\right].\label{eq:E12}
\end{align}
%Here $\beta\geq0, \tau>0$ are the solutions to the following min-max optimization:
%\bea
%\min_{\tau>0}\max_{\beta\geq0}~\frac{\beta\tau}{2} - \frac{\beta^2 \gamma}{2\E\left[\frac{1}{\frac{1}{\omega Y_\ell+1}+\frac{\tau}{\beta}}\right]} +  \frac{1}{2}\E\left[\frac{1}{\frac{1}{\omega Y_\ell+1}+\frac{\tau}{\beta}}\right] - \frac{1}{2}  \cb^T\left(\eta\right) \cdot\A^{-1}\left(\eta\right)\cdot \cb\left(\eta\right)
%\end{align}


Rearranging \eqref{eq:E12} and using $\tau=\alpha_0\sqrt{\gamma}$ gives the following equation for $\eta$:
\bea
\frac{\alpha_0\sqrt{\gamma}}{\beta}  \E\left[\frac{1}{\frac{1}{\omega Y_\ell+1}+\eta}\right] = \gamma \stackrel{\tau=\alpha_0\sqrt{\gamma}}{\implies}~ \E\left[\frac{\eta}{\frac{1}{\omega Y_\ell+1}+\eta}\right] = \gamma .\label{eq:key_eta}
\end{align}
Recalling \eqref{eq:Y_ell_log_WLS}, we may rewrite the RHS above as 
\bea
\frac{\eta \E\left[V_\ell\right]}{\frac{1}{\omega +1}+\eta} +  \frac{\eta\left(1-E\left[V_\ell\right]\right)}{1+\eta} = \gamma \implies \eta^2(1-\gamma) (1+\omega) + \eta\left(1-\gamma(2+\omega)+\E[V_\ell]\omega\right) - \gamma = 0.
\end{align}
Since $\gamma<1$, the quadratic equation above has one nonnegative solution and we can deduce that
\bea\label{eq:etaopt}
\eta = \frac{-\left(1-2\gamma+\left(\E[V_\ell]-\gamma\right)\omega\right) + \sqrt{1+2\left(E[V_\ell]+\gamma-2E[V_\ell]\gamma\right)\omega + \left(\E[V_\ell]-\gamma\right)^2\omega^2}}{2(1-\gamma)(1+\omega)}
\end{align}
%
%Putting these together, $\beta,\alpha_0,\ab,\bb_\ell$ solve the following system of $r+3$ equations in $r+3$ unknowns:
%\begin{subequations}
%\begin{align}
%\beta^2 &= \E\left[\frac{\left({\alpha_0G_0+\ab^T\g+\bb_\ell-Y_\ell}\right)^2}{\left(\left(\omega Y_\ell+1\right)^{-1}+\eta\right)^2}\right] \\
%\begin{bmatrix}
%\ab \\ \bb_\ell
%\end{bmatrix} &= \A^{-1}\left(\eta\right)\cdot \cb\left(\eta\right)\\
%\eta &= {\gamma}\Big/ \E\left[\frac{1}{\frac{1}{\omega Y_\ell+1}+\eta}\right]\\
%\frac{\alpha_0\sqrt{\gamma}}{\beta} &= \eta
%\end{align}
%\end{subequations}

Thus, the optimal values of $\ab$ and $\bb_\ell$ are found by \eqref{eq:WLS_ab} for $\eta$ as in \eqref{eq:etaopt}. To solve for $\alpha_0$, we combine \eqref{eq:E12} and \eqref{eq:beta2_WLS} which leads to 
\bea
\alpha_0^2 \left( \frac{\gamma}{\eta^2} - \E\left[\left(\frac{1}{(\omega Y_\ell+1)^{-1}+\eta}\right)^2\right] \right) = \E\left[\frac{\left({\ab^T\g+\bb_\ell-Y_\ell}\right)^2}{\left(\left(\omega Y_\ell+1\right)^{-1}+\eta\right)^2}\right],
\end{align}
where we have also used the RHS of \eqref{eq:key_eta}. Finally, the RHS above can be computed as 
$$
\frac{\begin{bmatrix} \ab^T & \bb_\ell \end{bmatrix} \A_1 \begin{bmatrix} \ab \\ \bb_\ell \end{bmatrix} - 2\begin{bmatrix} \ab^T & \bb_\ell \end{bmatrix} \cb_1 + \E\left[V_\ell \right]}{\left((\omega+1)^{-1}+\eta\right)^2} ~+~ \frac{\begin{bmatrix} \ab^T & \bb_\ell \end{bmatrix} \A_2 \begin{bmatrix} \ab \\ \bb_\ell \end{bmatrix} }{\left(1+\eta\right)^2}
$$
and note that 
$$
\E\left[\left(\frac{1}{(\omega Y_\ell+1)^{-1}+\eta}\right)^2\right]  = \frac{\E[V_\ell]}{\left((\omega+1)^{-1}+\eta\right)^2} + \frac{1-\E[V_\ell]}{\left(1+\eta\right)^2}.
$$


\begin{lemma}
Let $V_\ell = \frac{e^{r G_\ell}}{\sum e^{r G_i}},$ where $G_1,\ldots,G_k\simiid\Nn(0,1)$.
\begin{align}
E\left[G_c G_j V_\ell\right] &= 2r^2\E\left[\frac{e^{r G_c}e^{r G_j}e^{r G_\ell}}{\left(\sum e^{r G_i}\right)^3}\right] ,\quad c\neq j \neq \ell \\
E\left[G_c^2 V_\ell\right] &= \E\left[\frac{e^{r G_\ell}}{\sum e^{r G_i}}\right] + 2r^2\E\left[\frac{\left(e^{r G_c}\right)^2e^{r G_\ell}}{\left(\sum e^{r G_i}\right)^3}\right]  - r^2\E\left[\frac{e^{r G_\ell}e^{r G_c}}{\left(\sum e^{r G_i}\right)^2}\right],\quad c\neq \ell, \quad\\
E\left[G_\ell G_c V_\ell\right] &= 2r^2\E\left[\frac{\left(e^{r G_\ell}\right)^2e^{r G_c}}{\left(\sum e^{r G_i}\right)^3}\right]  - r^2\E\left[\frac{e^{r G_\ell}e^{r G_c}}{\left(\sum e^{r G_i}\right)^2}\right],\quad c\neq \ell\\
E\left[G_\ell^2 V_\ell\right] &= (1+r^2)\E\left[\frac{e^{r G_\ell}}{\sum e^{r G_i}}\right] -3r^2\E\left[\left(\frac{e^{r G_\ell}}{\sum e^{r G_i}}\right)^2\right] + 2r^2\E\left[\left(\frac{e^{r G_\ell}}{\sum e^{r G_i}}\right)^3\right]
\end{align}
\end{lemma}

==> abstract.tex <==
Contemporary machine learning applications often involve classification tasks with many classes. Despite their wide use a precise understanding of the statistical properties and behavior of these algorithms is still missing especially in modern regimes where the number of classes are rather large. In this paper we take a step in this direction by providing the first asymptotically precise analysis of linear multiclass classification. Our precise asymptotic allows us to precisely characterize how the test error varies for different losses, training data distributions, as well as the number of classes and problem dimensions.


For Gaussian Mixture Models, we identify the Bayes estimator and show that it corresponds to class conditional averaging. We then derive the exact asymptotics of the least-squares loss and connect it to the averaging estimator. We demonstrate that the estimator performance is highly distribution-dependent. Our analysis on a planted softmax regression model reveals that least-squares can provably outperform the averaging estimator. Our theoretical toolset for multiclass asymptotics opens the door for further research and can be of independent interest.


==> app_numerics.tex <==

\section{Numerical Results}

\begin{figure}[h]
\begin{center}
\includegraphics[width=.5\textwidth]{Example.eps}
\end{center}
\caption{}
\end{figure}

%\begin{figure}[h]
%\begin{center}
%\includegraphics[width=.5\textwidth]{example2.eps}
%\end{center}
%\caption{Test error of LS vs averaging method for equal-energy and orthogonal means for the logistic model. Here $k=4$, $r_1=1$, $r_2=r_3=2$, $r_4=3$ and $d=100$ and averaging over 25 realizations.}
%\end{figure}

\begin{figure}[t!]
	\centering
	\begin{subfigure}{1.8in}
	\begin{tikzpicture}
	\node at (0,0) {\includegraphics[scale=0.22]{gmm_figures/dim_300_energy_15_class_9_subcl_3_scale_1_corr_0_overall}};
	\node at (-2.35,0) [rotate=90,scale=1.]{Prob of Error};
	\node at (0,-1.8) [scale=1.]{$\gamma$};
	\end{tikzpicture}\vspace{-3pt}\caption{Orthogonal, $k=9$, Equal prior, $\tn{\bmu_i}^2=15$}\label{fig:covariance}\vspace{-0.2cm}
	\end{subfigure}
	\begin{subfigure}{1.8in}
	\begin{tikzpicture}
	\node at (0,0) {\includegraphics[scale=0.22]{gmm_figures/dim_300_energy_15_class_9_subcl_3_scale_2_corr_0_overall}};
	\node at (-2.35,0) [rotate=90,scale=1.]{Prob of Error};
	\node at (0,-1.8) [scale=1.]{$\gamma$};
	\end{tikzpicture}\vspace{-3pt}\caption{Orthogonal, Different Prior $\pi_{7,8,9}=2\pi_{4,5,6}=4\pi_{1,2,3}=4/21$}\label{fig:positive}\vspace{-0.2cm}
	\end{subfigure}
	\begin{subfigure}{1.8in}
	\begin{tikzpicture}
	\node at (0,0) {\includegraphics[scale=0.22]{gmm_figures/dim_300_energy_15_class_9_subcl_3_scale_2_corr_1_overall}};
	\node at (-2.35,0) [rotate=90,scale=1.]{Prob of Error};
	\node at (0,-1.8) [scale=1.]{$\gamma$};
	\end{tikzpicture}\vspace{-3pt}\caption{Correlated, Different prior}\label{fig:negative}\vspace{-0.2cm}
		\end{subfigure}
		\caption{}
\end{figure}

\begin{figure}[t!]
	\centering
	\begin{subfigure}{1.8in}
	\begin{tikzpicture}
	\node at (0,0) {\includegraphics[scale=0.22]{gmm_figures/dim_300_energy_15_class_9_subcl_3_scale_1_corr_0_gam_0p1166407465007776.eps}};
	\node at (-2.35,0) [rotate=90,scale=1.]{Conditional Error};
	\node at (0,-1.8) [scale=1.]{Class ID};
	\end{tikzpicture}\vspace{-3pt}\caption{Orthogonal, Equal prior, $\tn{\bmu_i}^2=15$}\label{fig:covariance}\vspace{-0.2cm}
	\end{subfigure}
	\begin{subfigure}{1.8in}
	\begin{tikzpicture}
	\node at (0,0) {\includegraphics[scale=0.22]{gmm_figures/dim_300_energy_15_class_9_subcl_3_scale_2_corr_0_gam_0p1166407465007776.eps}};
	\node at (-2.35,0) [rotate=90,scale=1.]{};
	\node at (0,-1.8) [scale=1.]{Class ID};
	\end{tikzpicture}\vspace{-3pt}\caption{Orthogonal, Different Prior}\label{fig:positive}\vspace{-0.2cm}
	\end{subfigure}
	\begin{subfigure}{1.8in}
	\begin{tikzpicture}
	\node at (0,0) {\includegraphics[scale=0.22]{gmm_figures/dim_300_energy_15_class_9_subcl_3_scale_2_corr_1_gam_0p1166407465007776.eps}};
	\node at (-2.35,0) [rotate=90,scale=1.]{};
	\node at (0,-1.8) [scale=1.]{Class ID};
	\end{tikzpicture}\vspace{-3pt}\caption{Correlated, Different prior}\label{fig:negative}\vspace{-0.2cm}
		\end{subfigure}
		\caption{}
\end{figure}
\begin{figure}[t!]
	\centering
	\begin{subfigure}{1.8in}
	\begin{tikzpicture}
	\node at (0,0) {\includegraphics[scale=0.22]{gmm_figures/dim_50_energy_15_scale_1_corr_0_gam_0p55_overall_k.pdf}};
	\node at (-2.35,0) [rotate=90,scale=1.]{Probability of Error};
	\node at (0,-1.8) [scale=1.]{\# of Classes};
	\end{tikzpicture}\vspace{-3pt}\caption{$d=50,~K\gamma=20/11$, $\tn{\bmu_i}^2=15$}\label{fig:covariance}\vspace{-0.2cm}
	\end{subfigure}
	\begin{subfigure}{1.8in}
	\begin{tikzpicture}
	\node at (0,0) {\includegraphics[scale=0.22]{gmm_figures/dim_100_energy_15_scale_1_corr_0_gam_0p55_overall_k.pdf}};
	\node at (-2.35,0) [rotate=90,scale=1.]{};
	\node at (0,-1.8) [scale=1.]{\# of Classes};
	\end{tikzpicture}\vspace{-3pt}\caption{$d=100,~K\gamma=20/11$}\label{fig:positive}\vspace{-0.2cm}
	\end{subfigure}
	\begin{subfigure}{1.8in}
	\begin{tikzpicture}
	\node at (0,0) {\includegraphics[scale=0.22]{gmm_figures/dim_200_energy_15_scale_1_corr_0_gam_0p55_overall_k.pdf}};
	\node at (-2.35,0) [rotate=90,scale=1.]{};
	\node at (0,-1.8) [scale=1.]{\# of Classes};
	\end{tikzpicture}\vspace{-3pt}\caption{$d=200,~K\gamma=20/11$}\label{fig:negative}\vspace{-0.2cm}
		\end{subfigure}
		\caption{}
\end{figure}
\begin{figure}[t!]
	\centering
	\begin{subfigure}{1.8in}
	\begin{tikzpicture}
	\node at (0,0) {\includegraphics[scale=0.22]{gmm_figures/dim_50_energy_15_scale_1_corr_0_gam_0p55_ratio_k.pdf}};
	\node at (-2.35,0) [rotate=90,scale=1.]{Probability of Error};
	\node at (0,-1.8) [scale=1.]{\# of Classes / p};
	\end{tikzpicture}\vspace{-3pt}\caption{$d=50,~K\gamma=20/11$, $\tn{\bmu_i}^2=15$}\label{fig:covariance}\vspace{-0.2cm}
	\end{subfigure}
	\begin{subfigure}{1.8in}
	\begin{tikzpicture}
	\node at (0,0) {\includegraphics[scale=0.22]{gmm_figures/dim_100_energy_15_scale_1_corr_0_gam_0p55_ratio_k.pdf}};
	\node at (-2.35,0) [rotate=90,scale=1.]{};
	\node at (0,-1.8) [scale=1.]{\# of Classes / p};
	\end{tikzpicture}\vspace{-3pt}\caption{$d=100,~K\gamma=20/11$}\label{fig:positive}\vspace{-0.2cm}
	\end{subfigure}
	\begin{subfigure}{1.8in}
	\begin{tikzpicture}
	\node at (0,0) {\includegraphics[scale=0.22]{gmm_figures/dim_200_energy_15_scale_1_corr_0_gam_0p55_ratio_k.pdf}};
	\node at (-2.35,0) [rotate=90,scale=1.]{};
	\node at (0,-1.8) [scale=1.]{\# of Classes / p};
	\end{tikzpicture}\vspace{-3pt}\caption{$d=200,~K\gamma=20/11$}\label{fig:negative}\vspace{-0.2cm}
		\end{subfigure}
		\caption{}
\end{figure}

\begin{figure}[t!]
	\centering
	\begin{subfigure}{1.8in}
	\begin{tikzpicture}
	\node at (0,0) {\includegraphics[scale=0.22]{gmm_figures/dim_200_energy_15_class_9_subcl_3_scale_1_corr_0_overall_LGT.pdf}};
	\node at (-2.35,0) [rotate=90,scale=1.]{Probability of Error};
	\node at (0,-1.8) [scale=1.]{$\gamma$};
	\end{tikzpicture}\vspace{-3pt}\caption{Orthogonal, Same Prior $\rho=10$}\label{fig:covariance}\vspace{-0.2cm}
	\end{subfigure}
	\begin{subfigure}{1.8in}
	\begin{tikzpicture}
	\node at (0,0) {\includegraphics[scale=0.22]{gmm_figures/dim_200_energy_10_class_9_subcl_3_scale_2_corr_0_overall_LGT.pdf}};
	\node at (-2.35,0) [rotate=90,scale=1.]{};
	\node at (0,-1.8) [scale=1.]{$\gamma$};
	\end{tikzpicture}\vspace{-3pt}\caption{Orthogonal, Different norms $\rho_{7,8,9}=2\rho_{4,5,6}=4\rho_{1,2,3}=40$}\label{fig:positive}\vspace{-0.2cm}
	\end{subfigure}
	\begin{subfigure}{1.8in}
	\begin{tikzpicture}
	\node at (0,0) {\includegraphics[scale=0.22]{gmm_figures/dim_200_energy_10_class_9_subcl_3_scale_2_corr_0_gam_0p11668611435239207_LGT.pdf}};
	\node at (-2.35,0) [rotate=90,scale=1.]{Marginal Prob Error};
	\node at (0,-1.8) [scale=1.]{Class ID};
	\end{tikzpicture}\vspace{-3pt}\caption{Orthogonal, Different norms $\rho_{7,8,9}=2\rho_{4,5,6}=4\rho_{1,2,3}=40$}\label{fig:negative}\vspace{-0.2cm}
		\end{subfigure}
		\caption{}
\end{figure}


\begin{figure}[t!]
	\centering
	\begin{subfigure}{1.8in}
	\begin{tikzpicture}
	\node at (0,0) {\includegraphics[scale=0.22]{gmm_figures/dim_100_energy_10_gam_0p55_overall_k_LGT}};
	\node at (-2.35,0) [rotate=90,scale=1.]{Probability of Error};
	\node at (0,-1.8) [scale=1.]{\# of Classes / p};
	\end{tikzpicture}\vspace{-3pt}\caption{$d=50,~K\gamma=20/11$, $\tn{\bmu_i}=10$}\label{fig:covariance}\vspace{-0.2cm}
	\end{subfigure}
	\begin{subfigure}{1.8in}
	\begin{tikzpicture}
	\node at (0,0) {\includegraphics[scale=0.22]{gmm_figures/dim_100_energy_10_gam_0p55_ratio_k_LGT}};
	\node at (-2.35,0) [rotate=90,scale=1.]{Ratio of Error Prob};
	\node at (0,-1.8) [scale=1.]{\# of Classes / p};
	\end{tikzpicture}\vspace{-3pt}\caption{$d=50,~K\gamma=20/11$, $\tn{\bmu_i}=10$}\label{fig:positive}\vspace{-0.2cm}
	\end{subfigure}
	\begin{subfigure}{1.8in}
	\begin{tikzpicture}
	\node at (0,0) {\includegraphics[scale=0.22]{gmm_figures/dim_50_energy_10_scale_1_corr_0_gam_0p55_ratio_k_LGT}};
	\node at (-2.35,0) [rotate=90,scale=1.]{};
	\node at (0,-1.8) [scale=1.]{\# of Classes / p};
	\end{tikzpicture}\vspace{-3pt}\caption{$d=100,~K\gamma=20/11$, $\tn{\bmu_i}=10$}\label{fig:negative}\vspace{-0.2cm}
		\end{subfigure}
		\caption{}
\end{figure}

==> ave_backup.tex <==
\section{Averaging Estimator}

Consider the following simple averaging estimator:

\begin{align}
\Wh:=\frac{1}{n}\Y\X^T \qquad\text{and} \qquad \bh:= \frac{1}{n}\Y\one
\end{align}

The following high-dimensional limits hold for all $i,j\in[k]$:
\begin{subequations}\label{eq:ave0}
\bea
\bh_i &\rP \pi_i \label{eq:ave01}\\
\inp{\wh_i}{\mub_j} &\rP \pi_i \cdot \inp{\mub_i}{\mub_j}
 \\
\inp{\wh_i}{\wh_j} &\rP \begin{cases} \pi_i\pi_j\cdot \inp{\mub_i}{\mub_j} &, i\neq j,
\\
\pi_i^2 \|\mub_i\|^2 + \pi_i \gamma &, i=j.
\end{cases}
\end{align}
\end{subequations}


\begin{proof}[of \eqref{eq:ave0}]
The first statement \eqref{eq:ave01} follows directly from the fact that $\frac{1}{n}\one^T\Y_i = \frac{n_i}{n} \rP \pi_i.$ For the next two statements note that
\begin{align}
\wh_i = \frac{1}{n}\M\Y \Y_i + \frac{1}{n} \Zb \Y_i =\frac{1}{n}\sum_{j=1}^k \mub_j(\Y_j^T\Y_i) + \frac{1}{n} \Zb \Y_i = \frac{\twonorm{\Y_i}^2}{n}\mub_i + \frac{1}{n} \Zb \Y_i,
\end{align}
where in the last line we used orthogonality of the rows $\Y_j$ of the matrix $\Y$:
\bea\label{eq:ortho}
\inp{\Y_i}{\Y_j} = 0, \forall i\neq j\in[k].
\end{align}
 To conclude use the facts that for all $i\in[k]$: 
 \begin{enumerate}
\item[(i)] $\frac{\twonorm{\Y_i}^2}{n}=\frac{n_i}{n}\rP\pi_i$.
 \item[(ii)] $\Zb \Y_i \sim \twonorm{\Y_i}\g_i$ with $\g_i\simiid\Nn(0,\Id_d)$ because of \eqref{eq:ortho}
 \item[(iii)] $\frac{\twonorm{\g_i}}{\sqrt{n}}\rP \sqrt{\gamma}$ and $\frac{1}{\sqrt{n}}\inp{\g_i}{\mub_j}\rP 0$.
 \end{enumerate}
\end{proof}



\noindent Instead, let 
\begin{align}
\Wh:=\frac{1}{n}(\Y -\bh\one_n^T)\X^T \Longleftrightarrow\wh_i := \X(\Y_i-\bh_i\one_n),~i\in[k]  \qquad\text{and} \qquad \bh:= \frac{1}{n}\Y\one_k
\end{align}

The following high-dimensional limits hold for all $i,j\in[k]$:
\begin{subequations}\label{eq:ave}
\bea
\bh_i &\rP \pi_i \label{eq:ave1}\\
\inp{\wh_i}{\mub_j} &\rP \pi_i \cdot \inp{\mub_i}{\mub_j}
 \\
\inp{\wh_i}{\wh_j} &\rP \begin{cases} \pi_i\pi_j\cdot \inp{\mub_i}{\mub_j} &, i\neq j,
\\
\pi_i^2 \|\mub_i\|^2 + \pi_i \gamma &, i=j.
\end{cases}
\end{align}
\end{subequations}

\begin{proof}[of \eqref{eq:ave}]
The first statement \eqref{eq:ave1} follows directly from the fact that $\frac{1}{n}\one^T\Y_i = \frac{n_i}{n} \rP \pi_i.$ For the next two statements note that
\begin{align}
\wh_i &= \frac{1}{n}\M\Y (\Y_i-\bh_i\one_n) + \frac{1}{n} \Zb (\Y_i-\bh_i\one_n) =\frac{1}{n}\sum_{j=1}^k \mub_j(\Y_j^T\Y_i-\bh_i \inp{\Y_j}{\one_n}) + \frac{1}{n} \Zb (\Y_i-\bh_i\one_n)\nn \\
 &= \left(\frac{\twonorm{\Y_i}^2}{n} - \bh_i \frac{\inp{\Y_i}{\one_n}}{n}\right) \mub_i + \frac{1}{n} \Zb (\Y_i-\bh_i\one_n),
\end{align}
where in the last line we used orthogonality of the rows $\Y_j$ of the matrix $\Y$:
\bea\label{eq:ortho}
\inp{\Y_i}{\Y_j} = 0, \forall i\neq j\in[k].
\end{align}
For convenience, let $\g_i:=\frac{1}{n}\Zb (\Y_i-\bh_i\one_n),~i\in[k]$. Clearly, the $\g_i$'s are Gaussian and we can readily computed that:
$$
\inp{\g_i}{\g_j} \rP \gamma\,( \delta_{ij} - \pi_i\pi_j).
$$
\noindent To continue use \eqref{eq:ave1} and the facts that for all $i\in[k]$: $\frac{\twonorm{\Y_i}^2}{n}=\frac{n_i}{n}\rP\pi_i$ and $\frac{\inp{\Y_i}{\one_n}}{n}\rP \pi_i$ to see that:
$$
\frac{\twonorm{\Y_i}^2}{n} - \bh_i \frac{\inp{\Y_i}{\one_n}}{n} \rP \pi_i(1-\pi_i).
$$
Also, note that $\inp{\g_i}{\mub_j}\rP0, \forall i,j\in[k]$. 

Using all the above we find that
$$
\inp{\wh_i}{\wh_j} \rP \pi_i\pi_j(1-\pi_i)(1-\pi_j)\inp{\mub_i}{\mub_j} + \gamma(\delta_{ij}-\pi_i\pi_j),
$$
and
$$
\inp{\wh_i}{\mu_j} =\rP\pi_i(1-\pi_i)\inp{\mub_i}{\mub_j}.
$$

\end{proof}




\subsection{Special cases}

\subsubsection{Two classes}
We compute the conditional probabilities $\P_1,\P_2$ as in \eqref{eq:condP}.
Specifically using \eqref{eq:ave}, we compute 
 \bea
 \Sc_1 = \twonorm{\pi_1\mub_1 - \pi_2\mub_2}^2 + \gamma\qquad\text{and}\qquad t_1=(\pi_2-\pi_1) + \pi_2\inp{\mub_1}{\mub_2} - \pi_1\twonorm{\mub_1}^2.
 \end{align}
 Thus, from \eqref{eq:condP}:
 $$
 \P_1 = Q\left(\frac{\pi_1\twonorm{\mub_1}^2 - \pi_2\inp{\mub_1}{\mub_2} + \pi_1 - \pi_2}{\sqrt{\twonorm{\pi_1\mub_1 - \pi_2\mub_2}^2 + \gamma}}\right)\,.
 $$

\vp
\noindent\textbf{Equal priors:} If $\pi_1=\pi_2=1/2$, then
 $$
 \P_1 = Q\left(\frac{\twonorm{\mub_1}^2 - \inp{\mub_1}{\mub_2}}{\sqrt{\twonorm{\mub_1 - \mub_2}^2 + 4\gamma}}\right)
 $$
 
\subsubsection{Orthogonal means and equal priors}
Assume $\inp{\mub_i}{\mub_j}=0,~i,j\in[k]$ and $\pi_i=\pi,~i\in[k]$.

In this case,
$
\P\left( \text{error} \,|\, \y = \e_c \right) = 1 - \P\left( \Sb_c^{{1}/{2}}\, \z > \tb \right),
$
with 
$$\Sb_c=\pi(\pi+\gamma)(\Id + \one\one^T)
\qquad\text{and}\qquad
\tb = \pi\one.
$$ 


==> commands.tex <==
\newcommand{\vct}[1]{\bm{#1}}
\newcommand{\mtx}[1]{\bm{#1}}

\newcommand{\Wh}{\widehat\W}


\def\wh{\widehat{\vct{w}}}
\def\bh{\widehat{b}}


\usepackage{breqn}
  
 %%%%%%%%%%%%%%%%%

\newcommand{\thetao}{\overline{\theta}}

\newcommand{\go}{\overline{g}}
\newcommand{\etao}{\overline{\eta}}

\newcommand{\Scb}{\mathbf{\Sc}^{(n)}}
\newcommand{\ksit}{\widetilde{\ksi}}
\newcommand{\qt}{\widetilde{q}}

\newcommand{\Ell}{L}

\newcommand{\betah}{\widehat{\beta}}

\newcommand{\betabs}{\mathbf{\betab}_\star}
\newcommand{\yh}{\hat{y}}
\newcommand{\Rce}{\widehat{\mathcal{R}}_{\rm emp}}
\newcommand{\Rcex}{\mathcal{R}_{\rm excess}}
\newcommand{\Rct}{\mathcal{R}_{\rm train}}
\newcommand{\Ecsep}{\Ec_{\rm{sep}}}

\newcommand{\Rad}[1]{{\rm{Rad}}\left(#1\right)}

\newcommand{\BSC}{{\rm{BSC}}}
\newcommand{\BSCe}{{\rm{BSC}}_{\eps}}
\newcommand{\mathleft}{\@fleqntrue\@mathmargin0pt}
\newcommand{\mathcenter}{\@fleqnfalse}
\newcommand{\corr}[2]{{\rm{corr}}\left(\,{#1}\,;\,{#2}\,\right)}
\newcommand{\coss}[2]{{\rm{cos}}(\,{#1}\,,\,{#2}\,)}
\newcommand{\err}[2]{{\rm{Err}}(\,{#1}\,,\,{#2}\,)}

\DeclareMathOperator{\argmin}{argmin}

%%% Proximal and Moreau
\newcommand{\env}[3]{\mathcal{M}_{{#1}}\left({#2};{#3}\right)}
\newcommand{\prox}[3]{\mathrm{prox}_{{#1}}\left({#2};{#3}\right)}
\newcommand{\proxri}[3]{p_{#1}\left({#2},{#3}\right)}
\newcommand{\proxr}[2]{p\left({#1},{#2}\right)}
\newcommand{\ellprox}[3]{L_{#1}\left({#2},{#3}\right)}

\newcommand{\ellp}{\ell^\prime}


\newcommand{\eenvl}[2]{\overline{\mathcal{M}_{\ell}}\left({#1};{#2}\right)}
\newcommand{\envl}[2]{\mathcal{M}_{\ell}\left({#1};{#2}\right)}
\newcommand{\proxl}[2]{\mathrm{prox}_{\ell}\left({#1};{#2}\right)}



% derivatives
\newcommand{\elldd}{\ell^{''}}
\newcommand{\elld}{\ell^\prime}
\newcommand{\rhod}{f}

\newcommand{\envdx}[3]{\mathcal{M}^\prime_{{#1},1}\left({#2};{#3}\right)}
\newcommand{\envdla}[3]{\mathcal{M}^\prime_{{#1},2}\left({#2};{#3}\right)}
\newcommand{\envddx}[3]{\mathcal{M}^{''}_{{#1},1}\left({#2};{#3}\right)}

\newcommand{\ourx}{\al G + \mu S Y}

\newcommand{\func}{(\cdot)}

\newcommand{\R}{\mathbb{R}}

%% Greek
\newcommand{\al}{\alpha}
 \newcommand{\om}{\omega}
% \newcommand{\betabh}{\hat{\boldsymbol\beta}}
    \newcommand{\gammab}{\boldsymbol\gamma}
%        \newcommand{\etab}{\boldsymbol\eta}
 \newcommand{\chib}{\boldsymbol\chi}
 \newcommand{\Sigb}{\boldsymbol\Sigma}
  \newcommand{\mub}{\boldsymbol\mu}



% starred
\newcommand{\las}{\la_{\star}}
\newcommand{\als}{\al_{\star}}
\newcommand{\mus}{\mu_{\star}}


% hats, tildes
\newcommand{\betabh}{\boldsymbol{\widehat{\beta}}}
\newcommand{\xh}{\widehat{\x}}
\newcommand{\yo}{\overline{y}}


\newcommand{\rP}{\stackrel{{P}}{\rightarrow}}
%\newcommand{\ras}{\stackrel{\text{a.s.}}{\longrightarrow}}
\newcommand{\ras}{\xrightarrow[]{a.s.}}


\newcommand{\Christos}[1]{{\color{blue}Christos: #1}}
%\newcommand{\Abla}[1]{{\color{red}Abla: #1}}
%\newcommand{\Zeyu}[1]{{\color{green}Zeyu: #1}}



\providecommand{\vu}{\vec{u}} \providecommand{\vw}{\vec{w}}
\providecommand{\vx}{\vec{x}} \providecommand{\vy}{\vec{y}}

\providecommand{\abs}[1]{\lvert#1\rvert}
\providecommand{\norm}[1]{\lVert#1\rVert}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\DeclarePairedDelimiterX{\inp}[2]{\langle}{\rangle}{#1, #2}


\newcommand{\Id}{\mathbf{I}}

\newcommand{\Xh}{\widehat{\X}}
\newcommand{\tr}[1]{\operatorname{tr{(#1)}}}


\newcommand{\etab}{\boldsymbol{\eta}}

\newcommand{\plim}{\operatorname{plim}}
\newcommand{\nlim}{\operatorname{{ n \rightarrow \infty }}}

\newcommand{\plimn}{\underset{\nlim}{\plim}}

\newcommand{\FM}{F_M}


\usepackage{dsfont}
\newcommand{\ind}[1]{{\mathds{1}}_{\{#1\}}}
\newcommand{\Cauchy}{Cauchy-Schwarz }
\newcommand{\simiid}{\stackrel{\text{iid}}{\sim}}


\newcommand{\Pro}{\mathbb{P}}


% overline
\newcommand{\xio}{\overline{\phi}}
\newcommand{\phio}{\overline{\phi}}
\newcommand{\phiScco}{\overline{\phi_{\Scc}}}


% theorems
\theoremstyle{theorem}
\newtheorem{propo}{Proposition}[section]
%\newtheorem{apppropo}{Proposition}[subsection]
%\newtheorem{conj}{Conjecture}[section]
\newtheorem{thm}{Theorem}[section]
%\newtheorem{appthm}{Theorem}[subsection]
\newtheorem{lem}{Lemma}[section]
%\newtheorem{applem}{Lemma}[subsection]
%\newtheorem{form}{Formula}
\newtheorem{cor}{Corollary}[section]
\newtheorem{ass}{Assumption}%[section]
%
\theoremstyle{remark}
\newtheorem{remark}{Remark}%[subsection]
%\newtheorem{fact}{Fact}[section]
%%\newtheorem{example}{Example}[section]
%
%
\theoremstyle{definition}
\newtheorem{defn}{Definition}[section]
%\newtheorem{appdefn}{Definition}[subsection]
%\newtheorem{prop}{Property}[section]
%\newtheorem{pro}{Problem}[section]


\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}




\newcommand{\mn}{{(n)}}
\newcommand{\Exp}{\mathbb{E}}               % expectation
\newcommand{\E}{\mathbb{E}}                    % expectation
\newcommand{\la}{{\lambda}}                     % lambda
\newcommand{\sigg}{\sigma^2}
\newcommand{\sig}{\sigma}


\newcommand{\vecc}{\mathrm{vec}}

\newcommand{\nn}{\notag}
\newcommand{\Rb}{\mathbb{R}}







%bold upper
%\newcommand{\M}{\mathbf{M}}
%\newcommand{\Z}{{Z}}

%\newcommand{\Ub}{\mathbf{U}}
%\newcommand{\Gb}{\mathbf{G}}
%\newcommand{\Hb}{\mathbf{H}}
%\newcommand{\G}{\mathbf{G}}
%\newcommand{\Sb}{\mathbf{S}}
%\newcommand{\X}{\mathbf{X}}
%\newcommand{\XXb}{\overline{\mathbf{X}}}
%\newcommand{\A}{\mathbf{A}}
%\newcommand{\Lb}{\mathbf{L}}
%\newcommand{\Y}{\mathbf{Y}}
%\newcommand{\Vb}{\mathbf{V}}
%\newcommand{\Sb}{\mathbf{S}}
\newcommand{\W}{\mathbf{W}}
\newcommand{\M}{{M}}
\newcommand{\Z}{{Z}}
\newcommand{\Ub}{{U}}
\newcommand{\G}{\mathbf{G}}

\newcommand{\Hb}{{H}}
%\newcommand{\G}{{G}}
\newcommand{\Sb}{{S}}
\newcommand{\X}{{X}}
\newcommand{\XXb}{\overline{\mathbf{X}}}
\newcommand{\Lb}{{L}}
\newcommand{\Y}{{Y}}
\newcommand{\Vb}{{V}}
\newcommand{\A}{\mathbf{A}}

%Bold lower
\newcommand{\ellb}{\boldsymbol{\ell}}
\newcommand{\phib}{\boldsymbol{\phi}}
\newcommand{\x}{\mathbf{x}}
\newcommand{\ub}{\mathbf{u}}


\newcommand{\w}{\mathbf{w}}
\newcommand{\tb}{\mathbf{t}}
\newcommand{\g}{\mathbf{g}}
\newcommand{\vb}{\mathbf{v}}
\newcommand{\bb}{\mathbf{b}}
\newcommand{\e}{\mathbf{e}}
\newcommand{\y}{\mathbf{y}}
\newcommand{\s}{\mathbf{s}}
\newcommand{\z}{\mathbf{z}}
\newcommand{\zo}{\overline{\mathbf{z}}}
\newcommand{\bseta}{{\boldsymbol{\eta}}}
\newcommand{\Iden}{\mathbf{I}}
\newcommand{\cb}{\mathbf{c}}  
\newcommand{\ab}{\mathbf{a}}
\newcommand{\oneb}{\mathbf{1}}
\newcommand{\h}{\mathbf{h}}
\newcommand{\f}{\mathbf{f}}
\newcommand{\betab}{\boldsymbol{\beta}}
%\newcommand{\tb}{\mathbf{t}}


%Calligraphic
\newcommand{\Fc}{\mathcal{F}}
\newcommand{\Mc}{\mathcal{M}}
\newcommand{\Ps}{\mathcal{P}}
\newcommand{\Rs}{\mathcal{R}}
\newcommand{\Tc}{{\mathcal{T}}}
\newcommand{\Sc}{{\mathcal{S}}}
\newcommand{\Bc}{{\mathcal{B}}}
\newcommand{\Yc}{\mathcal{Y}}
\newcommand{\Dc}{\mathcal{D}}
\newcommand{\Xc}{\mathcal{X}}
\newcommand{\Zc}{\mathcal{Z}}
%\newcommand{\Ic}{\mathcal{I}}
\newcommand{\Uc}{\mathcal{U}}
\newcommand{\Kc}{\mathcal{K}}
\newcommand{\Nc}{\mathcal{N}}
\newcommand{\Rc}{\mathcal{R}}
\newcommand{\Nn}{\mathcal{N}}
\newcommand{\Lc}{\mathcal{L}}
\newcommand{\Cc}{\mathcal{C}}
\newcommand{\Gc}{{\mathcal{G}}}
\newcommand{\Ac}{\mathcal{A}}
\newcommand{\Pc}{\mathcal{P}}
\newcommand{\Ec}{\mathcal{E}}
\newcommand{\Hc}{\mathcal{H}}
\newcommand{\Qc}{\mathcal{Q}}
\newcommand{\Oc}{\mathcal{O}}
\newcommand{\Jc}{\mathcal{J}}
\newcommand{\Ic}{\mathcal{I}}

%hat, tilde, etc
\newcommand{\vh}{\hat{v}}
%\newcommand{\alh}{\hat{\al}}
\newcommand{\bh}{\hat{\beta}}
\newcommand{\thh}{\hat{\tau_{h}}}
\newcommand{\tgh}{\hat{\tau_{g}}}
%...

%Equations
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\bea}{\begin{align}}
\newcommand{\eea}{\end{align}}

\newcommand{\vp}{\vspace{4pt}}

% Misc
\newcommand{\order}[1]{\mathcal{O}\left(#1\right)}
\newcommand{\li}{\left<}
\newcommand{\ri}{\right>}







==> doublePro_Gaussian.tex <==
\section{Proof of Theorem \ref{thm:kinf_LS} {\color{blue} Gaussian means, $k\rightarrow\infty$}}

In this section we assume that 
%$\M = \Gb + c\cdot\qb\one_d^T$ 
$\M = \frac{r}{\sqrt{d}}\Gb$ 
where 
$\Gb\in\R^{d\times k}$ 
has entries IID $\Nn(0,1)$. Notice that with this normalization $\E[\M^T\M] = r^2\Iden_k$, i.e., the mean vectors have  constant energy $r^2$.
%We study an asymptotic setting in which $k\rightarrow\infty$ such that $k/n\rightarrow\zeta>0$.
 
Fix any $\ell\in[k]$. The classifier parameters $\wh_\ell,\bh_\ell$ are determined by solving the following min-norm minimization problem:
\begin{align}
(\widehat\w_\ell,\widehat b_\ell) &= \arg\min_{\w,b}\mathcal{L}_{PO}\left(\w,b\right):=\frac{1}{2n}\twonorm{\mtx{Y}^T\mtx{M}^T\w+ \mtx{Z}^T\w+b\vct{1}_n-\mtx{Y}_\ell}^2 \nn \\
&=\arg\min_{\substack{\w,b \\ \tb=\M^T\w }}~\frac{1}{2n}\twonorm{\mtx{Y}^T\tb+ \mtx{Z}^T\w+b\vct{1}_n-\mtx{Y}_\ell}^2 \nn \\
&=\arg\min_{\w,b,\tb}~\max_{\ub,\s}~\frac{1}{\sqrt{n}}\s^T\left(\mtx{Y}^T\tb+ \mtx{Z}^T\w+b\vct{1}_n-\mtx{Y}_\ell\right) - \frac{\twonorm{\s}^2}{2} + \left(\ub^T\M^T\w - \ub^T\tb\right) \label{eq:bilin}
\end{align}


\noindent\textbf{Identifying the AO.}~~In \eqref{eq:bilin} we recognize the form of a PO as required by the CGMT with two bilinear terms $\s^T\Zb^T\tb$ and $\ub^T\M^T\w=\frac{r}{\sqrt{d}}\ub^T\Gb^T\w$ involving the Gaussian matrices $\Zb^T\in\R^{n\times d}$ and $\Gb^T\in\R^{k\times d}$, respectively.  
Thus, we consider the following AO problem
\begin{align}
\min_{\w,b,\tb}~\max_{\ub,\s}~\frac{1}{\sqrt{n}}\s^T\left(\mtx{Y}^T\tb+ \twonorm{\w}\g_n +b\vct{1}_n-\mtx{Y}_\ell\right) + \frac{1}{\sqrt{n}}\twonorm{\s}\h_1^T\w - \frac{\twonorm{\s}^2}{2} + \ub^T\left(\frac{r}{\sqrt{d}}\twonorm{\w}\g_k - \tb\right) + \frac{r}{\sqrt{d}}\twonorm{\ub}\h_2^T\w \label{eq:AO_inf_1}
\end{align}
where $\h_1\sim\Nn(\zero_d,\Iden_d)$, $\h_2\sim\Nn(\zero_d,\Iden_d)$, $\g_n\sim\Nn(\zero_n,\Iden_n)$ and $\g_k\sim\Nn(\zero_k,\Iden_k)$.


\vp
\noindent\textbf{Scalarization of the AO.}~~
It is straightforward to optimize over the directions of the dual variables $\ub$ and $\s$. Setting $u:={\twonorm{\ub}}$ and $s:={\twonorm{\s}}$, the AO in \eqref{eq:AO_inf_1} simplifies to the following:
\begin{align}
\min_{\w,b,\tb}~\max_{u\geq0,s\geq 0}~\frac{s}{\sqrt{n}}\twonorm{\mtx{Y}^T\tb+ \twonorm{\w}\g_n +b\vct{1}_n-\mtx{Y}_\ell} + \frac{s}{\sqrt{n}}\h_1^T\w - \frac{s^2}{2} + u\twonorm{r\twonorm{\w}\frac{\g_k}{\sqrt{d}} - \tb} + \frac{u r}{\sqrt{d}}\h_2^T\w \label{eq:AO_inf_2}.
\end{align}

Next, we optimize over the direction of $\w$. Note that for any $s,u$ the optimal direction of $\w$ is one that aligns with the vector $-\left(s\frac{\h_1}{\sqrt{n}}+u r \frac{\h_2}{\sqrt{d}}\right)$. Thus calling $\alpha=\twonorm{\w}$, we can express \eqref{eq:AO_inf_2} as follows,
\begin{align}
\min_{\alpha\geq0,b,\tb}~\max_{u\geq0,s\geq 0}~\frac{s}{\sqrt{n}}\twonorm{\mtx{Y}^T\tb+ \alpha\g_n +b\vct{1}_n-\mtx{Y}_\ell}  + {u}\twonorm{r\alpha\frac{\g_k}{\sqrt{d}} - \tb} - {\alpha}\twonorm{s\frac{\h_1}{\sqrt{n}}+u r \frac{\h_2}{\sqrt{d}}} - \frac{s^2}{2}\label{eq:AO_inf_3}.
\end{align}

At this point, note that the objective function is convex in $\tb$ and concave in $u,s$. Thus, considering the ``bounded" AO {\color{blue} to be formalized} we can first minimize over $\tb$. To further facilitate this, we use the fact that
\begin{align}\nn%\label{eq:sqrt_trick2}
\chi = \min_{\tau>0} \,\frac{\tau}{2} + \frac{\chi^2}{2\tau},~\chi> 0.
\end{align}
With this, optimization over $\tb$ boils down to minimizing the following convex quadratic
\begin{align}
\min_{\tb} ~ &\frac{1}{2}\tb^T\left(\frac{s}{\tau_1}\frac{\Y\Y^T}{n}+\frac{u}{\tau_2}{\Iden_k}\right)\tb - \left(\frac{u\alpha r}{\tau_2 \sqrt{k}} {\g_k} - \frac{s}{\tau_1 {n}} \Y\left(\alpha \g_n + b \one_n - \Y_\ell\right)\right)^T\tb \nn\\
&\qquad\quad+ \frac{s}{2\tau_1}\frac{\twonorm{\alpha \g_n + b \one_n - \Y_\ell}^2}{n} + \frac{ur^2\alpha^2}{2\tau_2}\frac{\twonorm{\g_k}^2}{k} + \frac{s\tau_1}{2} + \frac{u\tau_2}{2}.
\end{align}
Clearly, the optimal value of $\tb$ is 
\begin{align}\label{eq:t_opt}
\tb &= \left(\frac{s}{\tau_1}\frac{\Y\Y^T}{n}+\frac{u}{\tau_2}{\Iden_k}\right)^{-1}\left(\frac{u\alpha r}{\tau_2} \frac{\g_k}{\sqrt{d}} - \frac{s}{\tau_1} \frac{\Y\left(\alpha \g_n + b \one_n - \Y_\ell\right)}{n}\right) \\
&=  \left(\frac{s}{\tau_1}\diag{\frac{n_1}{n},\ldots,\frac{n_k}n}+\frac{u}{\tau_2}{\Iden_k}\right)^{-1}\left(\frac{u\alpha r}{\tau_2} \frac{\g_k}{\sqrt{d}} - \frac{s}{\tau_1} \frac{\Y\left(\alpha \g_n + b \one_n - \Y_\ell\right)}n\right),
\end{align}
{\color{red}So here: $n_i/n=O(1/k)\rightarrow 0$, so the diag term will disappear.}
where $\alpha\geq0, b, s\geq 0, u\geq 0, \tau_1>0$ and $\tau_2>0$ solve the following min-max problem
\begin{align}
&\min_{\substack{\alpha\geq0,b,\\ \tau_1>0,\tau_2>0}}~\max_{u\geq0,s\geq 0}~ 
\frac{s}{2\tau_1n}\twonorm{\alpha \g_n + b \one_n - \Y_\ell}^2 
+ \frac{ur^2\alpha^2}{2\tau_2k}\twonorm{\g_k}^2 + \frac{s\tau_1}{2} + \frac{u\tau_2}{2} - \frac{s^2}{2} - {\alpha}\twonorm{s\frac{\h_1}{\sqrt{n}}+ur\frac{\h_2}{\sqrt{k}}} \nn\\
&-\frac{1}{2} \left(\frac{u\alpha r}{\tau_2} \frac{\g_k}{\sqrt{d}} - \frac{s}{\tau_1} \frac{\Y\left(\alpha \g_n + b \one_n - \Y_\ell\right)}n\right)^T\left(\frac{s}{\tau_1}\diag{\frac{n_1}{n},\ldots,\frac{n_k}n}+\frac{u}{\tau_2}{\Iden_k}\right)^{-1}\left(\frac{u\alpha r}{\tau_2} \frac{\g_k}{\sqrt{d}} - \frac{s}{\tau_1} \frac{\Y\left(\alpha \g_n + b \one_n - \Y_\ell\right)}n\right)
\label{eq:AO_inf_scal}.
\end{align}
{\color{blue}where I need to justify bringing the min over $\tau_1$ and $\tau_2$ inside}



\vp
\noindent\textbf{Convergence of the AO.}~ For simplicity let us assume a balanced setting, i.e., $$n_1=n_2=\ldots=n_k=n/k.$$

\noindent\textbf{\color{blue} Asymptotic \#1:} consider the following asymptotic regime:
\bea
n,k,d\rightarrow\infty,~~\frac{d}{k} \rightarrow\delta>0,~~\frac{kd}{n}\rightarrow\gamma.
\end{align}
For fixed $\alpha\geq0, b, s\geq 0, u\geq 0, \tau_1>0$ and $\tau_2>0$ the following limits follow from the WLLN:
\begin{subequations}
\begin{align}
\frac{1}{n}\twonorm{\alpha \g_n + b \one_n - \Y_\ell}^2  &\rP \alpha^2 + b^2,\\ %+ \pi_\ell - 2 b \pi_\ell ,  \\
\frac{1}{k}\twonorm{\g_k}^2 \rP 1 , \\
\twonorm{s\frac{\h_1}{\sqrt{n}}+ur\frac{\h_2}{\sqrt{d}}} &\rP \sqrt{s^2 \delta_{d,n} + u^2r^2}  = u r,\\
\left(\frac{s}{\tau_1}\diag{\frac{n_1}{n},\ldots,\frac{n_k}n}+\frac{u}{\tau_2}\frac{\Iden_k}k\right)^{-1} & \rP \frac{\tau_2}{u}\Iden_k,
\\
\left(\frac{u\alpha r}{\tau_2} \frac{\g_k}{\sqrt{d}} - \frac{s}{\tau_1} \frac{\Y\left(\alpha \g_n + b \one_n - \Y_\ell\right)}n\right)&\rD \frac{u\alpha r}{\tau_2} \g_k - \frac{sb}{\tau_1} - \frac{s}{\tau_1}\eb_\ell,
\\
\frac{1}{k}\twonorm{\frac{u\alpha r}{\tau_2} \frac{\g_k}{k} - \frac{s}{\tau_1} \frac{\Y\left(\alpha \g_n + b \one_n - \Y_\ell\right)}n}^2&\rP \frac{u^2\alpha^2 r^2}{\tau_2^2} + \frac{s^2b^2}{\tau_1^2},
\end{align}
\end{subequations}


\noindent\textbf{\color{blue} Asymptotic \#2:} consider the following asymptotic regime:
\bea
n,k,d\rightarrow\infty,~~\frac{d}{k} \rightarrow\delta>0,~~\frac{d}{n}\rightarrow\gamma\in(0,1).
\end{align}
For fixed $\alpha\geq0, b, s\geq 0, u\geq 0, \tau_1>0$ and $\tau_2>0$ the following limits follow from the WLLN:
\begin{subequations}
\begin{align}
\frac{1}{n}\twonorm{\alpha \g_n + b \one_n - \Y_\ell}^2  &\rP \alpha^2 + b^2,\\ %+ \pi_\ell - 2 b \pi_\ell ,  \\
\frac{1}{k}\twonorm{\g_k}^2 \rP 1 , \\
\twonorm{s\frac{\h_1}{\sqrt{n}}+ur\frac{\h_2}{\sqrt{d}}} &\rP \sqrt{s^2 \delta_{d,n} + u^2r^2}  = \sqrt{s^2\gamma + u^2 r^2},\\
\frac{1}{k}\left(\frac{s}{\tau_1}\diag{\frac{n_1}{n},\ldots,\frac{n_k}n}+\frac{u}{\tau_2}\frac{\Iden_k}k\right)^{-1} & \rP \left(\frac{s}{\tau_1}+\frac{u}{\tau_2}\right)^{-1}\Iden_k,
\\
k\left(\frac{u\alpha r}{\tau_2} \frac{\g_k}{k} - \frac{s}{\tau_1} \frac{\Y\left(\alpha \g_n + b \one_n - \Y_\ell\right)}n\right)&\rD \frac{u\alpha r}{\tau_2} \g_k - \frac{s\alpha}{\tau_1} \sqrt{\frac{\gamma}{\delta}} \widetilde\g_k - \frac{sb}{\tau_1} - \frac{s}{\tau_1}\eb_\ell,
\\
\frac{1}{k}\twonorm{\frac{u\alpha r}{\tau_2} \frac{\g_k}{k} - \frac{s}{\tau_1} \frac{\Y\left(\alpha \g_n + b \one_n - \Y_\ell\right)}n}^2&\rP \frac{u^2\alpha^2 r^2}{\tau_2^2} + \frac{s^2\alpha^2}{\tau_1^2}\frac{\gamma}{\delta} + \frac{s^2b^2}{\tau_1^2},
\end{align}
\end{subequations}
where in the second to last line $\g_k,\widetilde{\g}_k$ are iid standard normal vectors in $\R^k$.





==> facts.tex <==
\section{Useful Facts}

\begin{propo}[\cite{sathe1980note}]\label{propo:equicorrelated_bound}
 Let $\X:=(X_1,\ldots,X_n)\sim \Nn(0,\Sc)$ with $\Sc=(1-\rho)\Id_n+\rho \one\one^T$ for some $\rho\in[0,1)$. Define $b=(1-\rho)$, $c=1+(n-1)\rho$ and for fixed $\x=(x_1,\ldots,x_n)$ let $\xbar=\frac{1}{n}\sum_{i=1}^{n}x_i$ and $s^2 = \sum_{i=1}^n(x_i-\xbar)$. Consider the tail probability $\P(\x):=\P(\X\geq\x)=\P(\forall i: X_i\geq x_i)$. The following two bounds are true.
\bea
\P(\x) \geq \sqrt{\frac{b}{c}} \cdot \exp\left({-\frac{n \rho \xbar^2}{ 2c^2}}\right)\cdot \prod_{i=1}^n Q\left( \frac{x_i}{\sqrt{b}} - \frac{n\xbar\rho}{c\sqrt{b}} \right),
\end{align}
and
\bea
\P(\x) \leq \left({\frac{c}{b}}\right)^\frac{n-1}{2} \cdot \exp\left({\frac{n \rho s^2}{ 2b^2}}\right)\cdot \prod_{i=1}^n Q\left( \frac{x_i\sqrt{c}}{{b}} - \frac{n\xbar\rho}{b\sqrt{c}} \right).
\end{align}
\end{propo}

==> introold.tex <==
\section{Introduction}

%Deep learning has a dramatic impact on 
%With the growing popularity of deep learning, there is a g
%As the influence of machine learning penetrates 
%As deep learning penetrates more domains, 
% (e.g.~ Image recognition tasks such as ImageNet challenge may contain requires ImageNet con recognition models 
%Growing list of machine learning tasks are classification tasks with huge number of classes
%\subsection{Motivation}
A large number of real-world machine learning applications demand the ability to automatically distinguish between thousands of different classes. Besides intuitive settings such as image recognition, applications of multiclass classification include essentially any problem with categorical outputs such as natural language processing \cite{sutskever2014sequence}, where a seq2seq decoder has to choose the correct word token, reinforcement learning \cite{jang2016categorical,mei2020global}, where the agent has to choose the correct action, and recommendation systems, where the model should recommend the correct movie out of many other options. For instance, YouTube's recommendation system is modeled as an extreme multiclass problem with more than a million classes where each video corresponds to a viable class \cite{covington2016deep}.

These growing list of applications motivate an in-depth exploration of the multiclass classification algorithms. Asymptotic analysis provides a promising toolbox for understanding the exact high-dimensional performance of machine learning algorithms as a function of problem variables. While there is a rich literature on high-dimensional estimation, multiclass classification is an under-explored venue possibly due to the difficulty of capturing the intricate dependencies between the classes. Perhaps surprisingly, even linear classification presents significant challenges and we don't have satisfactory answers to fundamental questions. For instance, to the best of our knowledge, this is the first work that identifies the Bayes optimal classifier for multiclass Gaussian mixtures (see Section \ref{gmm sec}).



\subsection{Contributions}

Our work takes a step towards a refined understanding of multiclass classification algorithms by providing the first asymptotically exact analysis of linear multiclass classification and characterizing the role of loss functions and the data distributions. We study classification performance of least-squares for multiclass classification under the following two popular models.
\begin{itemize}
\item \textbf{Gaussian mixture model (GMM):} A discriminative model that models the class conditional probabilities of the feature vectors with Gaussians.
\item \textbf{Softmax model:} A generative model which models the marginal probability of the labels given the feature vectors with the softmax function. 
\end{itemize}

For both distributions, we provide the exact asymptotics of the least-squares estimator when there are constant number of classes. For Gaussian mixture models, we identify the Bayes estimator and show that it corresponds to class conditional averaging. We then derive the exact asymptotics of the least-squares loss and connect it to the averaging estimator. Our results on the softmax model reveals that the estimator performance is highly distribution-dependent. For softmax model, we demonstrate that weighted least-squares provably outperforms the averaging estimator. Finally, we identify surprising shifts in asymptotic behavior as the number of classes is allowed to grow. We empirically demonstrate that in this regime, cross-entropy estimator outperforms the averaging estimator.\dots


We can get pairwise correlations!!!



\subsection{Notation}
We use $[k]$ to denote $\{1,2,\ldots,k\}$. We write $\eb_\ell\in\R^k$ for the $\ell$-th standard basis vector in $\R^k$. For a sequence of random variables $\mathcal{X}_{n,d}$ that converges in probability (resp., in distribution) to some constant $c$ (resp., to a random variable $X$)  in this limit, we simply write ${X}_{n,d}\rP c$ (resp., ${X}_{n,d}\rD X$). For a vector $\vct{c}\in\R^k$ we write $\arg\max \vct{c}$ to denote the index of the largest entry of $\vct{c}$ i.e.~$\arg\max \vct{c}=\underset{j\in[k]}{\arg\max}\text{ }\vct{c}_i$. We use the q-function $Q(x)$ given by $Q(x)=\frac{1}{\sqrt{2\pi}}\int_x^{+\infty}e^{-\frac{u^2}{2}}du$.

==> misc_proofs.tex <==
\section{Proof of \eqref{eq:uls}}
\noindent\textbf{Equal energy \& equal priors.}~~Further assume that $r_i=r, \forall i\in[k]$ and $\pi_i=\pi=1/k,\forall i\in[k]$.  In this case,
$
\P\left( \text{error} \,|\, \y = \e_c \right) = 1 - \P\left( \Sb_c^{{1}/{2}}\, \z > \tb \right),
$
with 
$$\Sb_c=\frac{\pi}{1+\pi r^2}\left(\frac{\pi r^2}{1+\pi r^2}+\frac{\gamma}{1-\gamma}\right)(\Id + \one\one^T)
\qquad\text{and}\qquad
\tb = -\frac{\pi r^2}{1+\pi r^2}\one.
$$ 
Thus, setting 
\bea\label{eq:uls}
u_{\rm LS}:=r^2\sqrt{ \frac{\pi}{ \pi r^2 + \left(\frac{\gamma}{1-\gamma}\right) \left({1+\pi r^2}\right)}}=r^2\sqrt{ \frac{1-\gamma}{r^2+\gamma/\pi}},
\end{align}
 the probability of error is given by:
$$
\P_e = \P\left(  G_0 + \max_{j\in[k-1]} G_j \geq u_{\rm LS} \right),\quad G_0,G_1,\ldots,G_{k-1}\simiid\Nn(0,1)\,.
$$
%The union bound \eqref{eq:UB} gives:
%\bea
%\P_e = \P_c \leq (k-1) \cdot Q\left( \frac{u_{\rm LS}}{\sqrt{2}} \right) %= (k-1) \cdot Q\left( \frac{r}{\sqrt{2\left(1+\frac{\gamma k}{ r^2}\right)}} \right)
%\end{align}
Directly comparing \eqref{eq:uls} to \eqref{eq:uave}, it can be seen that $$u_{LS} = u_{ave}\sqrt{1-\gamma}\,<\,u_{ave}\Longrightarrow \P_{c,\rm ave} < \P_{c,\rm LS}\,,$$ for all values of $k, \gamma<1$ and $r^2$. Thus, for orthogononal means of equal energy and balanced classes, \emph{the averaging estimator strictly outperforms LS for all $\gamma<1$ and $k\geq 2$.}



\section{Test error: Averaging estimator}
{\color{blue}Should probably remove this section.}
\vp
\noindent\textbf{Slepian's bound.}~
We may rewrite \eqref{eq:Pe1} as:
\bea
\P_c  = \P\left( \bigcup_{ j\neq c } \left\{z_{j} \geq -[\tb_c]_j\right\}  \right), \qquad [z_1,\ldots,z_{k-1}] \sim \Nn(0,\Sb_c).\label{eq:cond_4_slepian}
\end{align}
Assume that
$$
s_c = \min_{i\neq j\in[k-1]} \Sc_{ij} \geq 0
$$
and note that 
$$
\Sb \geq \left({\rm diag}(\Sb_c) - s_c\Id\right)\,\Id + s_c\one\one^T,
$$
where the inequality holds element-wise and equality is true for the diagonal elements. Then, one can apply Slepian's lemma to upper bound the conditional probability of error in \eqref{eq:cond_4_slepian} with:
\bea
\P_c \leq \P\left( \bigcup_{j\in[k-1]} \left\{\,G_0 + G_{j} \sqrt{\frac{[\Sb_c]_{jj}}{s_c}}  \geq -\frac{[\tb_c]_j}{s_c} \,\right\}  \right),\qquad G_0,G_1,\ldots,G_{k-1}\simiid\Nn(0,1)\,.
\end{align}



\vp
\noindent\textbf{Union bound.}~ In \eqref{eq:condP}, the conditional probabilities are expressed in terms of the tail of a multivariate Gaussian distribution. This probability can be numerically computed using Monte-carlo averaging of available software for relatively small values of number $k$ of classes. However, for analysis, the expressions can be somewhat unwiedly. A standard way to simplify is via the union bound:
\bea
\P_c &\leq \sum_{j\neq c} \P_{G\sim\Nn(0,1)}\left( \twonorm{\wh_j - \wh_c} G \leq \inp{\wh_j-\wh_c}{\mub_c} + (\bh_j-\bh_c)   \right)\nn\\
&=  \sum_{j\neq c} Q\left( \inp{\frac{\wh_c-\wh_j}{\twonorm{\wh_c - \wh_j}}}{\mub_c} + \frac{\bh_c-\bh_j}{\twonorm{\wh_c - \wh_j}} \right) = \sum_{j\neq c} Q\left( \frac{[\tb_c]_j}{\sqrt{[\Sb_c]_{j,j}}}\right) \label{eq:UB}
\\
&\leq (k-1)\cdot Q\left( d_{\min} \right),
\end{align}
where in the last line, we denote $d_{\min}:=\min_{j\neq c} \left\{{[\tb_c]_j}\Big/{\sqrt{[\Sb_c]_{j,j}}}\right\}.$



\vp
\noindent\textbf{Oracle bound.}~ Assume that the means $\mu_i,~i\in[n]$ are known. Then the problem of classifying a fresh sample $\x$ is a $k$-ary hypothesis testing problem with Gaussian conditionals. Denote $\P_{\rm genie , Bayes}$ the Bayes error of this hypothesis testing problem. Clearly $\P_{\rm genie , Bayes}$ is a lower bound on the error of any classifier that is trained on data. The paper \cite{wisler2016empirically} further lower bounds $\P_{\rm genie , Bayes}$ in terms of the Bayesian probability of errors between every two classes as follows:
\bea
\P_e \geq \P_{\rm genie , Bayes} &\geq \frac{2}{k}\sum_{i\neq j}\pi_i  \P_{\rm genie , ij} \\
&= \frac{2}{k}\sum_{i\neq j}\frac{\pi_i}{\pi_i+\pi_j} \left( \pi_i \cdot Q\left( \frac{\twonorm{\mu_i-\mu_j}}{2} + \frac{\log(\pi_i/\pi_j)}{\twonorm{\mu_i-\mu_j}} \right) + \pi_j \cdot Q\left( \frac{\twonorm{\mu_i-\mu_j}}{2} - \frac{\log(\pi_i/\pi_j)}{\twonorm{\mu_i-\mu_j}} \right)  \right).\nn
\end{align}
where $\P_{\rm genie , ij}$ is the Bayesian error between classes $i$ and $j$ with priors $\frac{\pi_i}{\pi_i+\pi_j}$ and $\frac{\pi_j}{\pi_i+\pi_j}$. For the last equality we have used the well-known formula for the Bayesian probability of binary Gaussian hypothesis testing. In the case of equal-priors the genie lower bound above simplifies to:
\bea\label{eq:genie_LB}
\P_e \geq \frac{2}{k}\sum_{i\neq j}{\pi_i}\cdot Q\left( \frac{\twonorm{\mu_i-\mu_j}}{2}  \right) .
\end{align}



==> proofLS_GM_over.tex <==
\section{Proof of Theorem \ref{thm:LS_GM_over}}

In this section, we analyze the min-norm LS solution in the overparameterized regime $\gamma>1$.


Fix any $\ell\in[k]$. The classifier parameters $\wh_k,\bh_k$ are determined by solving the following min-norm minimization problem:
\begin{align}
\Phi_{PO,\ell}(\Zb) &= \min_{\w,b}\max_{\ub} \twonorm{\w}^2 + \ub^T\left(\Y^T\M^T\w + \Zb^T\w + b\one_n - \Y_\ell\right) \\
&= \min_{\w,b}\max_{\ub}~\ub^T\Zb\w + \twonorm{\w}^2 + \ub^T\left(\Y^T\M^T\w + b\one_n - \Y_\ell\right),
\end{align}
and the corresponding AO problem
\begin{align}
\phi_{AO,\ell}(\g,\h) &= \min_{\w,b}\max_{\ub}~\twonorm{\w}\ub^T\g + \twonorm{\ub}\w^T\h + \twonorm{\w}^2 + \ub^T\left(\Y^T\M^T\w + b\one_n - \Y_\ell\right).\label{eq:AO_over}
\end{align}

\noindent\textbf{Scalarization of the AO}
Let $\beta=\twonorm{\ub}$ and optimize over the direction of $\ub$ to rewrite the AO in \eqref{eq:AO_over} as follows:
\begin{align}
\min_{\w,b}\max_{\beta\geq 0}~ \beta\twonorm{ \twonorm{\w}\g+\Y^T\M^T\w + b\one_n - \Y_\ell } + \beta\w^T\h + \twonorm{\w}^2 .\label{eq:AO_over}
\end{align}
{\color{blue}Argue about flipping the order here}. Next, we optimize over the direction $\wb^\perp$ of the component of $\wb$ that is orthogonal to the subspace spanned by the mean vectors. For this purpose, consider the SVD decomposition $\M=\Ub\Sigmab\Vb^T$ in \eqref{eq:M_SVD} and write 
$$
\w_\ell = \sum_{i=1}^{r}\alpha_i \ub_i + \alpha_0\w_\ell^\perp, 
$$
where $\twonorm{\w_\ell^\perp}=1$ and $\Ub^T\w_\ell^\perp = \mathbf{0}$, $\alpha_0\geq 0$ and  we denote
\bea\label{eq:alphab_def_over}
\alpha_i := \ub_i^T\w_\ell, i\in[r].
\end{align}
Thus we have
\begin{align}
\phi_{AO,\ell}(\g,\h)= &\min_{\alpha_0\geq 0, \alphab, b}\text{ } {\alpha_0^2} + {\twonorm{\alphab}^2}\label{eq:scal_AO_gen_over}\\
&~~~\text{sub. to}~~~~ R_\ell(\g,\h;\alpha_0,\alphab,b) \leq 0,\nn
\end{align}
where we also performed the optimization over $\beta\geq 0$ and we defined:
\begin{align}\label{eq:R_def}
\Rc_\ell(\g,\h;\alpha_0,\alphab,b):=\frac{1}{\sqrt{n}}\twonorm{ \sqrt{\alpha_0^2 + \sum_{i=1}^r\alpha_i^2}\,\vct{g}+\sum_{i=1}^{r}\alpha_i\sigma_i\mtx{Y}^T\vb_i  +b\vct{1}_n-\mtx{Y}_\ell}+ \sum_{i=1}^{r}{\alpha_i\frac{\vct{h}^T\ub_i}{\sqrt{n}}} -\alpha_0\frac{\twonorm{\h^\perp}}{\sqrt{n}},
\end{align}
with $\alphab=\begin{bmatrix}\alpha_1,\ldots,\alpha_r\end{bmatrix}^T\in\R^r$.

\vp
\noindent\textbf{Convergence of the AO.}~~
Recall the definition of the matrix $\A$ and vector $\cb_\ell$ in \eqref{eq:Amat}, as well as the function $\Dc(\alpha_0,\alphab,b)$:
\begin{align}
\Dc_\ell(\alpha_0,\alphab,b) = \sqrt{\alpha_0^2 + \pi_\ell +  \begin{bmatrix} \alphab^T & b \end{bmatrix} \A  \begin{bmatrix} \alphab \\ b  \end{bmatrix} - 2 \pi_\ell \cb_\ell^T \begin{bmatrix} \alphab \\ b  \end{bmatrix}} - \alpha_0\sqrt{\gamma}\label{eq:det_2_over}.
\end{align}
 Using \label{eq:Y_limits} it can be checked that
\begin{align}
\Rc_\ell(\g,\h;\alpha_0,\alphab,b) \rP \Dc_\ell(\alpha_0,\alphab,b),\label{eq:uniAO_gen}
\end{align}
uniformly over all $(\alpha_0,\alphab,\beta)\in\Cc$ {\color{blue} Argue boundedness -- define $\Cc$}. The convergence is uniform because the function $\Dc_\ell(\alpha_0,\alphab,b)$ is jointy convex in its arguments and the constraint  set $\Cc$ is compact.

\vp
\noindent\textbf{Deterministic analysis of the AO.}~~The uniform convergence in \eqref{eq:uniAO_gen} motivates studying the following deterministic optimization equivalent of \eqref{eq:scal_AO_gen_over}:
\begin{align}
&\min_{\alpha_0\geq 0, \alphab, b}\text{ } {\alpha_0^2} + {\twonorm{\alphab}^2}
\label{eq:det_AO_over}\\
&~~\text{sub. to}~~ \Dc_\ell(\alpha_0,\alphab,b) \leq 0,\nn
\end{align}
which is in turn equivalent to 
\begin{align}
&\min_{\alpha_0\geq 0, \alphab, b}\text{ } {\alpha_0^2} + {\twonorm{\alphab}^2}
\label{eq:det_AO_over_2}\\
&~~\text{sub. to}~~ \alpha_0 \geq \sqrt{\frac{1}{\gamma-1}}\sqrt{\begin{bmatrix} \alphab^T & b \end{bmatrix} \A  \begin{bmatrix} \alphab \\ b  \end{bmatrix} - 2 \pi_\ell \cb_\ell^T\begin{bmatrix} \alphab \\ b  \end{bmatrix}+\pi_\ell},\nn
\end{align}
Clearly, the optimal value of $\alpha_0$ is attained when the constraint holds with equality. Thus, $(\alphab,b)$ solves the following strictly convex quadratic program:
\begin{align}
&\min_{\alphab, b}\text{ } \begin{bmatrix} \alphab^T & b \end{bmatrix} \left(\A + \begin{bmatrix} \left(\gamma -1 \right) \Iden_r &\zero_r \\ \zero_r &0 \end{bmatrix} \right) \begin{bmatrix} \alphab \\ b  \end{bmatrix} - 2 \pi_\ell \cb_\ell^T\begin{bmatrix} \alphab \\ b  \end{bmatrix}+\pi_\ell.\nn
\end{align}
Setting (recall \eqref{eq:Deltab_def})
\bea
\Delta_\gamma:=\left(\gamma-1\right)\Iden_r + \Delta \succ 0, \label{eq:Delta_gamma}
\end{align}
this gives
\bea
\begin{bmatrix} \widehat\alphab \\ \widehat b \end{bmatrix} &= \pi_\ell \begin{bmatrix} \Iden & \zero \\ -\pib^T\Vb\Sigmab & 1 \end{bmatrix}\begin{bmatrix} \Deltab_\gamma^{-1} & \zero \\ \zero^T & 1 \end{bmatrix} \begin{bmatrix} \Iden & -\Sigmab\Vb^T\pib \\ \zero^T & 1 \end{bmatrix}\begin{bmatrix} \Sigmab\Vb^T\eb_\ell \\ 1\end{bmatrix}\nn\\
&= \pi_\ell \begin{bmatrix} -\Deltab_\gamma^{-1}\Sigmab\Vb^T(\pib-\eb_\ell) \\ 1+\pib^T\Vb\Sigmab\Deltab_\gamma^{-1}\Sigmab\Vb^T(\pib-\eb_\ell). \end{bmatrix}\label{eq:alphab_1}
\end{align}
%\begin{align}
%-\pi_\ell^2  \begin{bmatrix} -\left(\pib - \eb_\ell\right)^T\Vb\Sigmab && 1 \end{bmatrix} \begin{bmatrix} \Deltab^{-1} & \zero \\ \zero^T & 1 \end{bmatrix}\begin{bmatrix} -\Sigmab\Vb^T \left(\pib - \eb_\ell\right) \\ 1 \end{bmatrix} &= - \pi_\ell^2\left(1+\left(\pib - \eb_\ell\right)^T\Vb\Sigmab \Deltab^{-1} \Sigmab\Vb^T \left(\pib - \eb_\ell\right)\right).  \nn%\nn\\
%%&= - \pi_\ell^2\left(1+\left(\pib - \eb_\ell\right)^T \left(\Vb^T\Sigmab^{-2}\Vb^T+\Pb\right)^{-1} \left(\pib - \eb_\ell\right)\right) .
%\end{align}
Plugging this value in the RHS of the constraint in \eqref{eq:det_AO_over_2} and recalling we further find the optimal value of $\alpha_0$ is:
\begin{align}
\widehat\alpha_0 = \sqrt\frac{1}{\gamma-1}\sqrt{\pi_\ell\left(1-\pi_\ell\right) - \pi_\ell^2\left(\pib - \eb_\ell\right)^T\Vb\Sigmab \Deltab_\gamma^{-1}\left( \Iden_r - \left(\gamma-1\right)\Deltab_\gamma^{-1} \right) \Sigmab\Vb^T \left(\pib - \eb_\ell\right)}.
\end{align}

%
%It is convenient to define
%\begin{align}
%\widetilde\B:=\begin{bmatrix} \Iden_r+\Sigmab\Vb^T\diag{\pib}\Vb\Sigmab & \zero_r \\ \zero_r^T & -(\gamma-1) \end{bmatrix}\quad\text{and}\quad \widetilde\db_\ell = \begin{bmatrix} \pi_\ell\Sigmab\Vb^T\eb_\ell \\ 0 \end{bmatrix}.
%\end{align}
%In this notation, \eqref{eq:det_AO_over} becomes
%\begin{align}
%&\min_{\alpha_0\geq 0, \alphab, b}\text{ } {\alpha_0^2} + {\twonorm{\alphab}^2}
%\label{eq:det_AO_over_2}\\
%&~~\text{sub. to}~~ \begin{bmatrix} \ab^T & \alpha_0 \end{bmatrix} \widetilde\B \begin{bmatrix} \ab \\ \alpha_0 \end{bmatrix} - 2\widetilde\db_\ell^T\begin{bmatrix} \ab \\ \alpha_0 \end{bmatrix} + b^2 - 2\left(1-\pib^T\Vb\Sigmab\alphab\right) b + \pi_\ell \leq 0,\nn
%\end{align}
%Since the variable $b$ does not change the objective function, its optimal value is the one that minimizes the LHS of the constraint function:
%\begin{align}\label{eq:b_over}
%\widehat b = 1-\pib^T\Vb\Sigmab\alphab
%\end{align}
% Thus, recalling the notation $\Deltab$ in \eqref{eq:Deltab_def} and letting
%\begin{align}\label{eq:Bmat}
%\B:=\begin{bmatrix} \Deltab & \zero_r \\ \zero_r^T & -(\gamma-1) \end{bmatrix}\quad\text{and}\quad \db_\ell = \begin{bmatrix} \Sigmab\Vb^T\left(\pi_\ell\eb_\ell-\pib\right) \\ 0 \end{bmatrix}.
%\end{align}
%we have shown that \eqref{eq:det_AO_over_2} is equivalent to
%\begin{align}
%&\min_{\alpha_0\geq 0, \alphab}\text{ } {\alpha_0^2} + {\twonorm{\alphab}^2}
%\label{eq:det_AO_over_2}\\
%&~~\text{sub. to}~~ \begin{bmatrix} \ab^T & \alpha_0 \end{bmatrix} \B \begin{bmatrix} \ab \\ \alpha_0 \end{bmatrix} - 2\db_\ell^T\begin{bmatrix} \ab \\ \alpha_0 \end{bmatrix} - (1-\pi_\ell) \leq 0\nn
%\end{align}
%This is a single constrained quadratic optimization problem. Also, it is strictly feasible: the constraint is strictly negative for $\alphab = \zero_r, \alpha_0=1$ since $\gamma>1$. Thus, strong duality holds \cite[App.~B.1]{Boyd} and
% \eqref{eq:det_AO_over_2} is equal to 
%\begin{align}\nn%\label{eq:dual_over}
%&\min~\theta\quad\text{sub. to}~\la\geq 0\quad\text{and}\quad\begin{bmatrix}  \Iden_{r+1}+\la\B & \la \db_\ell\\ \la\db_\ell^T & \theta
%\end{bmatrix}\succeq \zero_{(r+2)\times(r+2)}\\
%=&\label{eq:dual_over_2}
%\min~\theta\quad\text{sub. to}~\frac{1}{\gamma-1}\geq \la\geq 0\quad\text{and}\quad\begin{bmatrix}  \Iden_{r}+\la\Deltab & \la \Sigmab\Vb^T\left(\pi_\ell\eb_\ell-\pib\right) \\ \la^T & \theta
%\end{bmatrix}\succeq \zero_{(r+2)\times(r+2)}
%\end{align}
% and the minimizers $\widehat\alphab$ and $\widehat\alpha_0$ are given as follows:
%\begin{align}\label{eq:opt_det_over}
%\widehat\alphab = \la^*\left(\Deltab+\lambda^*\Iden_r\right)^{-1}\Sigmab\Vb^T\left(\pi_\ell\eb_\ell - \pib\right)\qquad\alpha_0=0,
%\end{align}
%where 
%$$\la^*=\arg\min_{\la\geq0}\la^2\left(\pi_\ell\eb_\ell - \pib\right)^T\Vb\Sigmab\left(\Deltab+\lambda\Iden_r\right)^{-1}\Sigmab\Vb^T\left(\pi_\ell\eb_\ell - \pib\right)$$




==> proofLS_GM_over_with_b.tex <==
\section{Proof of Theorem \ref{thm:LS_GM_over} {\color{blue} Overparametrized}}

In this section, we analyze the min-norm LS solution in the overparameterized regime $\gamma>1$.


Fix any $\ell\in[k]$. The classifier parameters $\wh_\ell,\bh_\ell$ are determined by solving the following min-norm minimization problem:
\begin{align}
\Phi_{PO,\ell}(\Zb) &= \min_{\w,b}\max_{\ub} \twonorm{\w}^2 + b^2 + \ub^T\left(\Y^T\M^T\w + \Zb^T\w + b\one_n - \Y_\ell\right) \\
&= \min_{\w,b}\max_{\ub}~\ub^T\Zb\w + \twonorm{\w}^2 + b^2 + \ub^T\left(\Y^T\M^T\w + b\one_n - \Y_\ell\right),
\end{align}
and the corresponding AO problem
\begin{align}
\phi_{AO,\ell}(\g,\h) &= \min_{\w,b}\max_{\ub}~\twonorm{\w}\ub^T\g + \twonorm{\ub}\w^T\h + \twonorm{\w}^2 + b^2 + \ub^T\left(\Y^T\M^T\w + b\one_n - \Y_\ell\right).\label{eq:AO_over}
\end{align}

\noindent\textbf{Scalarization of the AO}
Let $\beta=\twonorm{\ub}$ and optimize over the direction of $\ub$ to rewrite the AO in \eqref{eq:AO_over} as follows:
\begin{align}
\min_{\w,b}\max_{\beta\geq 0}~ \beta\twonorm{ \twonorm{\w}\g+\Y^T\M^T\w + b\one_n - \Y_\ell } + \beta\w^T\h + \twonorm{\w}^2 + b^2 .\label{eq:AO_over}
\end{align}
{\color{blue}Argue about flipping the order here}. Next, we optimize over the direction $\wb^\perp$ of the component of $\wb$ that is orthogonal to the subspace spanned by the mean vectors. For this purpose, consider the SVD decomposition $\M=\Ub\Sigmab\Vb^T$ in \eqref{eq:M_SVD} and write 
$$
\w_\ell = \sum_{i=1}^{r}\alpha_i \ub_i + \alpha_0\w_\ell^\perp, 
$$
where $\twonorm{\w_\ell^\perp}=1$ and $\Ub^T\w_\ell^\perp = \mathbf{0}$, $\alpha_0\geq 0$ and  we denote
\bea\label{eq:alphab_def_over}
\alpha_i := \ub_i^T\w_\ell, i\in[r].
\end{align}
Thus we have
\begin{align}
\phi_{AO,\ell}(\g,\h)= &\min_{\alpha_0\geq 0, \alphab, b}\text{ } {\alpha_0^2} + {\twonorm{\alphab}^2} + b^2\label{eq:scal_AO_gen_over}\\
&~~~\text{sub. to}~~~~ R_\ell(\g,\h;\alpha_0,\alphab,b) \leq 0,\nn
\end{align}
where we also performed the optimization over $\beta\geq 0$ and we defined:
\begin{align}\label{eq:R_def}
\Rc_\ell(\g,\h;\alpha_0,\alphab,b):=\frac{1}{\sqrt{n}}\twonorm{ \sqrt{\alpha_0^2 + \sum_{i=1}^r\alpha_i^2}\,\vct{g}+\sum_{i=1}^{r}\alpha_i\sigma_i\mtx{Y}^T\vb_i  +b\vct{1}_n-\mtx{Y}_\ell}+ \sum_{i=1}^{r}{\alpha_i\frac{\vct{h}^T\ub_i}{\sqrt{n}}} -\alpha_0\frac{\twonorm{\h^\perp}}{\sqrt{n}},
\end{align}
with $\alphab=\begin{bmatrix}\alpha_1,\ldots,\alpha_r\end{bmatrix}^T\in\R^r$.

\vp
\noindent\textbf{Convergence of the AO.}~~
Recall the definition of the matrix $\A$ and vector $\cb_\ell$ in \eqref{eq:Amat}, as well as the function $\Dc(\alpha_0,\alphab,b)$:
\begin{align}
\Dc_\ell(\alpha_0,\alphab,b) = \sqrt{\alpha_0^2 + \pi_\ell +  \begin{bmatrix} \alphab^T & b \end{bmatrix} \A  \begin{bmatrix} \alphab \\ b  \end{bmatrix} - 2 \pi_\ell \cb_\ell^T \begin{bmatrix} \alphab \\ b  \end{bmatrix}} - \alpha_0\sqrt{\gamma}\label{eq:det_2_over}.
\end{align}
 Using \label{eq:Y_limits} it can be checked that
\begin{align}
\Rc_\ell(\g,\h;\alpha_0,\alphab,b) \rP \Dc_\ell(\alpha_0,\alphab,b),\label{eq:uniAO_gen}
\end{align}
uniformly over all $(\alpha_0,\alphab,\beta)\in\Cc$ {\color{blue} Argue boundedness -- define $\Cc$}. The convergence is uniform because the function $\Dc_\ell(\alpha_0,\alphab,b)$ is jointy convex in its arguments and the constraint  set $\Cc$ is compact.

\vp
\noindent\textbf{Deterministic analysis of the AO.}~~The uniform convergence in \eqref{eq:uniAO_gen} motivates studying the following deterministic optimization equivalent of \eqref{eq:scal_AO_gen_over}:
\begin{align}
&\min_{\alpha_0\geq 0, \alphab, b}\text{ } {\alpha_0^2} + {\twonorm{\alphab}^2} + b^2
\label{eq:det_AO_over}\\
&~~\text{sub. to}~~ \Dc_\ell(\alpha_0,\alphab,b) \leq 0,\nn
\end{align}
which is in turn equivalent to 
\begin{align}
&\min_{\alpha_0\geq 0, \alphab, b}\text{ } {\alpha_0^2} + {\twonorm{\alphab}^2} + b^2
\label{eq:det_AO_over_2}\\
&~~\text{sub. to}~~ \alpha_0 \geq \sqrt{\frac{1}{\gamma-1}}\sqrt{\begin{bmatrix} \alphab^T & b \end{bmatrix} \A  \begin{bmatrix} \alphab \\ b  \end{bmatrix} - 2 \pi_\ell \cb_\ell^T\begin{bmatrix} \alphab \\ b  \end{bmatrix}+\pi_\ell},\nn
\end{align}
Clearly, the optimal value of $\alpha_0$ is attained when the constraint holds with equality. Thus, $(\alphab,b)$ solves the following strictly convex quadratic program:
\begin{align}
&\min_{\alphab, b}\text{ } \begin{bmatrix} \alphab^T & b \end{bmatrix} \left(\A +  \left(\gamma -1 \right) \Iden_{r+1}  \right) \begin{bmatrix} \alphab \\ b  \end{bmatrix} - 2 \pi_\ell \cb_\ell^T\begin{bmatrix} \alphab \\ b  \end{bmatrix} \nn\\
= &\min_{\alphab, b}\text{ } \begin{bmatrix} \alphab^T & b \end{bmatrix} \begin{bmatrix} \gamma\Iden_{r}+\Sigmab\Vb^T\diag{\pib}\Vb\Sigmab &\Sigmab\Vb^T\pib \\ \pib^T\Vb\Sigmab & \gamma \end{bmatrix} \begin{bmatrix} \alphab \\ b  \end{bmatrix} - 2 \pi_\ell \cb_\ell^T\begin{bmatrix} \alphab \\ b  \end{bmatrix}.\nn
\end{align}
Setting 
\bea
\Delta_\gamma:=\gamma\Iden_r + \Sigmab\Vb^T\left(\diag{\pib}-\frac{1}{\gamma}\pib\pib^T\right)\Vb\Sigmab \succ 0, \label{eq:Delta_gamma}
\end{align}
this gives
\bea
\begin{bmatrix} \widehat\alphab \\ \widehat b \end{bmatrix} &= \pi_\ell \begin{bmatrix} \Iden & \zero \\ -\frac{1}{\gamma}\pib^T\Vb\Sigmab & 1 \end{bmatrix}\begin{bmatrix} \Deltab_\gamma^{-1} & \zero \\ \zero^T & \frac{1}{\gamma} \end{bmatrix} \begin{bmatrix} \Iden & -\frac{1}{\gamma}\Sigmab\Vb^T\pib \\ \zero^T & 1 \end{bmatrix}\begin{bmatrix} \Sigmab\Vb^T\eb_\ell \\ 1\end{bmatrix}\nn\\
&= \pi_\ell \begin{bmatrix} -\Deltab_\gamma^{-1}\Sigmab\Vb^T\left(\frac{\pib}\gamma-\eb_\ell\right) \\ \frac{1}{\gamma}+\frac{\pib^T}{\gamma}\Vb\Sigmab\Deltab_\gamma^{-1}\Sigmab\Vb^T\left(\frac{\pib}{\gamma}-\eb_\ell\right). \end{bmatrix}\label{eq:alphab_1}
\end{align}
%\begin{align}
%-\pi_\ell^2  \begin{bmatrix} -\left(\pib - \eb_\ell\right)^T\Vb\Sigmab && 1 \end{bmatrix} \begin{bmatrix} \Deltab^{-1} & \zero \\ \zero^T & 1 \end{bmatrix}\begin{bmatrix} -\Sigmab\Vb^T \left(\pib - \eb_\ell\right) \\ 1 \end{bmatrix} &= - \pi_\ell^2\left(1+\left(\pib - \eb_\ell\right)^T\Vb\Sigmab \Deltab^{-1} \Sigmab\Vb^T \left(\pib - \eb_\ell\right)\right).  \nn%\nn\\
%%&= - \pi_\ell^2\left(1+\left(\pib - \eb_\ell\right)^T \left(\Vb^T\Sigmab^{-2}\Vb^T+\Pb\right)^{-1} \left(\pib - \eb_\ell\right)\right) .
%\end{align}
Plugging this value in the RHS of the constraint in \eqref{eq:det_AO_over_2} we further find the optimal value of $\alpha_0$ as follows:
\begin{align}
\widehat\alpha_0 = \sqrt\frac{1}{\gamma-1}\sqrt{\pi_\ell\left(1-\frac{\pi_\ell}{\gamma}\right) - \pi_\ell^2\left(\frac{\pib}{\gamma} - \eb_\ell\right)^T\Vb\Sigmab \Deltab_\gamma^{-1}\left( \Iden_r - \left(\gamma-1\right)\Deltab_\gamma^{-1} \right) \Sigmab\Vb^T \left(\frac{\pib}{\gamma} - \eb_\ell\right)}.
\end{align}

%
%It is convenient to define
%\begin{align}
%\widetilde\B:=\begin{bmatrix} \Iden_r+\Sigmab\Vb^T\diag{\pib}\Vb\Sigmab & \zero_r \\ \zero_r^T & -(\gamma-1) \end{bmatrix}\quad\text{and}\quad \widetilde\db_\ell = \begin{bmatrix} \pi_\ell\Sigmab\Vb^T\eb_\ell \\ 0 \end{bmatrix}.
%\end{align}
%In this notation, \eqref{eq:det_AO_over} becomes
%\begin{align}
%&\min_{\alpha_0\geq 0, \alphab, b}\text{ } {\alpha_0^2} + {\twonorm{\alphab}^2}
%\label{eq:det_AO_over_2}\\
%&~~\text{sub. to}~~ \begin{bmatrix} \ab^T & \alpha_0 \end{bmatrix} \widetilde\B \begin{bmatrix} \ab \\ \alpha_0 \end{bmatrix} - 2\widetilde\db_\ell^T\begin{bmatrix} \ab \\ \alpha_0 \end{bmatrix} + b^2 - 2\left(1-\pib^T\Vb\Sigmab\alphab\right) b + \pi_\ell \leq 0,\nn
%\end{align}
%Since the variable $b$ does not change the objective function, its optimal value is the one that minimizes the LHS of the constraint function:
%\begin{align}\label{eq:b_over}
%\widehat b = 1-\pib^T\Vb\Sigmab\alphab
%\end{align}
% Thus, recalling the notation $\Deltab$ in \eqref{eq:Deltab_def} and letting
%\begin{align}\label{eq:Bmat}
%\B:=\begin{bmatrix} \Deltab & \zero_r \\ \zero_r^T & -(\gamma-1) \end{bmatrix}\quad\text{and}\quad \db_\ell = \begin{bmatrix} \Sigmab\Vb^T\left(\pi_\ell\eb_\ell-\pib\right) \\ 0 \end{bmatrix}.
%\end{align}
%we have shown that \eqref{eq:det_AO_over_2} is equivalent to
%\begin{align}
%&\min_{\alpha_0\geq 0, \alphab}\text{ } {\alpha_0^2} + {\twonorm{\alphab}^2}
%\label{eq:det_AO_over_2}\\
%&~~\text{sub. to}~~ \begin{bmatrix} \ab^T & \alpha_0 \end{bmatrix} \B \begin{bmatrix} \ab \\ \alpha_0 \end{bmatrix} - 2\db_\ell^T\begin{bmatrix} \ab \\ \alpha_0 \end{bmatrix} - (1-\pi_\ell) \leq 0\nn
%\end{align}
%This is a single constrained quadratic optimization problem. Also, it is strictly feasible: the constraint is strictly negative for $\alphab = \zero_r, \alpha_0=1$ since $\gamma>1$. Thus, strong duality holds \cite[App.~B.1]{Boyd} and
% \eqref{eq:det_AO_over_2} is equal to 
%\begin{align}\nn%\label{eq:dual_over}
%&\min~\theta\quad\text{sub. to}~\la\geq 0\quad\text{and}\quad\begin{bmatrix}  \Iden_{r+1}+\la\B & \la \db_\ell\\ \la\db_\ell^T & \theta
%\end{bmatrix}\succeq \zero_{(r+2)\times(r+2)}\\
%=&\label{eq:dual_over_2}
%\min~\theta\quad\text{sub. to}~\frac{1}{\gamma-1}\geq \la\geq 0\quad\text{and}\quad\begin{bmatrix}  \Iden_{r}+\la\Deltab & \la \Sigmab\Vb^T\left(\pi_\ell\eb_\ell-\pib\right) \\ \la^T & \theta
%\end{bmatrix}\succeq \zero_{(r+2)\times(r+2)}
%\end{align}
% and the minimizers $\widehat\alphab$ and $\widehat\alpha_0$ are given as follows:
%\begin{align}\label{eq:opt_det_over}
%\widehat\alphab = \la^*\left(\Deltab+\lambda^*\Iden_r\right)^{-1}\Sigmab\Vb^T\left(\pi_\ell\eb_\ell - \pib\right)\qquad\alpha_0=0,
%\end{align}
%where 
%$$\la^*=\arg\min_{\la\geq0}\la^2\left(\pi_\ell\eb_\ell - \pib\right)^T\Vb\Sigmab\left(\Deltab+\lambda\Iden_r\right)^{-1}\Sigmab\Vb^T\left(\pi_\ell\eb_\ell - \pib\right)$$




==> setting.tex <==
%\section{Gaussian-mixture model}

%\begin{assumption}[Gaussian Mixture Model]\label{ass:gaussian}
%
%\end{assumption}





%\noindent\textbf{Test error.}~

%Let $\Wh,\bh$ denote the parameters of a trained classifier. For a fresh data sample $(\x,\y)$ we decide that $\x$ belongs to class $c\in[k]$ when $\inp{\wh_c}{\x} > \max_{j\neq c}\inp{\wh_j}{\x}$. Therefore, the conditional probability of error of the classifier for each class $c\in[k]$ is given by:
%\bea
%\P\left( \text{error} \,|\, \y = \e_c \right) = 1 - \P\left( \inp{\wh_c}{\x} + \bh_c \geq \max_{j\neq c}\inp{\wh_j}{\x} + \bh_j  \right).\nn
%\end{align}
%Recall that $\x = \Mu\y + \z \stackrel{(\y=\e_c)}{=} \mub_c+\z$, $\z\sim\Nn(0,\Id_d)$. Hence,
%\bea
%\P\left( \text{error} \,|\, \y = \e_c \right)  
%&= \P\left( \exists j\neq c~:~ \inp{\wh_c-\wh_j}{\z} \leq  \inp{\wh_j-\wh_c}{\mub_c} +  (\bh_j-\bh_c)   \right) \nn\\
%&= 1 - \P\left( \forall j\neq c~:~ \inp{\wh_c-\wh_j}{\z} \geq  \inp{\wh_j-\wh_c}{\mub_c} +  (\bh_j-\bh_c)   \right).\label{eq:Pe1}
%\end{align}
%Let $\Sb_c\in\R^{{(k-1)}\times{(k-1)}}$ be a symmetric matrix such that its $i,j$ element is $[\Sb_c]_{ij}:=\inp{\wh_c-\wh_j}{\wh_c-\wh_i}$ and $\tb_c\in\R^{k-1}$ a vector with entries $[\tb_c]_i:=\inp{\wh_i-\wh_c}{\mub_c} +  (\bh_i-\bh_c).$ Then, we can rewrite \eqref{eq:Pe1} as
%\bea\label{eq:condP}
%\P_c:=\P\left( \text{error} \,|\, \y = \e_c \right) = 1 - \P\left( \Sb_c^{{1}/{2}}\, \z \geq \tb_c \right),
%\end{align}
%where the inequality in the rightmost expression applies entry-wise. Obviously, in terms of the conditionals, the test-error is computed as
%$
%\P_e = \sum_{i=1}^{k} \pi_c \P_c.
%$

\subsection{Test error}
\vp
\noindent\textbf{Slepian's bound.}~
We may rewrite \eqref{eq:Pe1} as:
\bea
\P_c  = \P\left( \bigcup_{ j\neq c } \left\{z_{j} \geq -[\tb_c]_j\right\}  \right), \qquad [z_1,\ldots,z_{k-1}] \sim \Nn(0,\Sb_c).\label{eq:cond_4_slepian}
\end{align}
Assume that
$$
s_c = \min_{i\neq j\in[k-1]} \Sc_{ij} \geq 0
$$
and note that 
$$
\Sb \geq \left({\rm diag}(\Sb_c) - s_c\Id\right)\,\Id + s_c\one\one^T,
$$
where the inequality holds element-wise and equality is true for the diagonal elements. Then, one can apply Slepian's lemma to upper bound the conditional probability of error in \eqref{eq:cond_4_slepian} with:
\bea
\P_c \leq \P\left( \bigcup_{j\in[k-1]} \left\{\,G_0 + G_{j} \sqrt{\frac{[\Sb_c]_{jj}}{s_c}}  \geq -\frac{[\tb_c]_j}{s_c} \,\right\}  \right),\qquad G_0,G_1,\ldots,G_{k-1}\simiid\Nn(0,1)\,.
\end{align}



\vp
\noindent\textbf{Union bound.}~ In \eqref{eq:condP}, the conditional probabilities are expressed in terms of the tail of a multivariate Gaussian distribution. This probability can be numerically computed using Monte-carlo averaging of available software for relatively small values of number $k$ of classes. However, for analysis, the expressions can be somewhat unwiedly. A standard way to simplify is via the union bound:
\bea
\P_c &\leq \sum_{j\neq c} \P_{G\sim\Nn(0,1)}\left( \twonorm{\wh_j - \wh_c} G \leq \inp{\wh_j-\wh_c}{\mub_c} + (\bh_j-\bh_c)   \right)\nn\\
&=  \sum_{j\neq c} Q\left( \inp{\frac{\wh_c-\wh_j}{\twonorm{\wh_c - \wh_j}}}{\mub_c} + \frac{\bh_c-\bh_j}{\twonorm{\wh_c - \wh_j}} \right) = \sum_{j\neq c} Q\left( \frac{[\tb_c]_j}{\sqrt{[\Sb_c]_{j,j}}}\right) \label{eq:UB}
\\
&\leq (k-1)\cdot Q\left( d_{\min} \right),
\end{align}
where in the last line, we denote $d_{\min}:=\min_{j\neq c} \left\{{[\tb_c]_j}\Big/{\sqrt{[\Sb_c]_{j,j}}}\right\}.$



\vp
\noindent\textbf{Oracle bound.}~ Assume that the means $\mu_i,~i\in[n]$ are known. Then the problem of classifying a fresh sample $\x$ is a $k$-ary hypothesis testing problem with Gaussian conditionals. Denote $\P_{\rm genie , Bayes}$ the Bayes error of this hypothesis testing problem. Clearly $\P_{\rm genie , Bayes}$ is a lower bound on the error of any classifier that is trained on data. The paper \cite{wisler2016empirically} further lower bounds $\P_{\rm genie , Bayes}$ in terms of the Bayesian probability of errors between every two classes as follows:
\bea
\P_e \geq \P_{\rm genie , Bayes} &\geq \frac{2}{k}\sum_{i\neq j}\pi_i  \P_{\rm genie , ij} \\
&= \frac{2}{k}\sum_{i\neq j}\frac{\pi_i}{\pi_i+\pi_j} \left( \pi_i \cdot Q\left( \frac{\twonorm{\mu_i-\mu_j}}{2} + \frac{\log(\pi_i/\pi_j)}{\twonorm{\mu_i-\mu_j}} \right) + \pi_j \cdot Q\left( \frac{\twonorm{\mu_i-\mu_j}}{2} - \frac{\log(\pi_i/\pi_j)}{\twonorm{\mu_i-\mu_j}} \right)  \right).\nn
\end{align}
where $\P_{\rm genie , ij}$ is the Bayesian error between classes $i$ and $j$ with priors $\frac{\pi_i}{\pi_i+\pi_j}$ and $\frac{\pi_j}{\pi_i+\pi_j}$. For the last equality we have used the well-known formula for the Bayesian probability of binary Gaussian hypothesis testing. In the case of equal-priors the genie lower bound above simplifies to:
\bea\label{eq:genie_LB}
\P_e \geq \frac{2}{k}\sum_{i\neq j}{\pi_i}\cdot Q\left( \frac{\twonorm{\mu_i-\mu_j}}{2}  \right) .
\end{align}






==> weighted_LS_under.tex <==
\section{Proof of Theorem \ref{thm:LS_GM_w} {\color{blue} Weighted LS -- Underparameterized}}


%\begin{align*}
%\underset{\mtx{W}\in\R^{k\times d},\text{ }b\in\R^k}{\min}\quad \frac{1}{2n}\fronorm{\mtx{W}\mtx{X}+b\vct{1}_n^T-\mtx{Y}}^2=&\sum_{\ell=1}^k \min_{\w, b}\text{ }\frac{1}{2n}\twonorm{\mtx{X}^T\w+b\vct{1}_n-\mtx{Y}_\ell}^2\\
%=&\sum_{\ell=1}^k \min_{\w, b}\text{ }\frac{1}{2n}\twonorm{\mtx{Y}^T\mtx{M}^T\w+ \mtx{Z}^T\w+b\vct{1}_n-\mtx{Y}_\ell}^2
%\end{align*}

Let 
\begin{align}\label{eq:Db_ell}
\Db = \omega \Y_\ell + \one_n,\quad \omega\geq 0.
\end{align}
and consider the weighted least-squares (WLS) solution:
\begin{align}
(\widehat\w_\ell,\widehat b) = \arg\min_{\w,b}\mathcal{L}_{PO}\left(\w,b\right):=\frac{1}{2n}\twonorm{\Db\left(\mtx{Y}^T\mtx{M}^T\w+ \mtx{Z}^T\w+b\vct{1}_n-\mtx{Y}_\ell\right)}^2\label{eq:LS_PO}
\end{align}


\noindent\textbf{Identifying the AO.}~~Note that by duality we have {\color{red} I missed a two here in the $1/(2n)$. Check the rest...}
\begin{align*}
(\widehat\w_\ell,\widehat b) =\arg\min_{\w, b}\text{ }\mathcal{L}_{PO}\left(\w,b\right) =\min_{\w, b,\tb}\text{ }\max_{\vct{s}}\text{ }\frac{1}{n}\left(\vct{s}^T\Db\mtx{Y}^T\mtx{M}^T\w+ \vct{s}^T\Db\mtx{Z}^T\w+b\vct{s}^T\Db\vct{1}_n-\vct{s}^T\Db\mtx{Y}_\ell-\s^T\Db\tb\right) + \frac{\twonorm{\Db\vct{t}}^2}{2n}
\end{align*}
Note that the above is jointly convex in $(\w, b,\tb)$ and concave in $\vct{s}$. We consider the Auxiliary Optimization (AO) problem
\begin{align*}
\min_{\w, b,\tb}\text{ }\max_{\vct{s}}\text{ }\frac{1}{n}\left(\vct{s}^T\Db\mtx{Y}^T\mtx{M}^T\w+ \twonorm{\w}\vct{g}^T\Db\vct{s}+ \twonorm{\Db\vct{s}}\vct{h}^T\w+b\vct{s}^T\Db\vct{1}_n-\vct{s}^T\Db\mtx{Y}_\ell-\s^T\Db\tb\right) + \frac{\twonorm{\Db\vct{t}}^2}{2n}
\end{align*}

\vp
\noindent\textbf{Scalarization of the AO.}~~
Maximizing over the direction of $\Db\vct{s}$ and setting its norm $\beta=\frac{\twonorm{\Db\vct{s}}}{\sqrt{n}}$ we arrive at
\begin{align*}
&\min_{\w, b,\tb}\text{ }\max_{\beta\ge 0}\text{ } \frac{\beta}{\sqrt{n}}\twonorm{ \twonorm{\w}\vct{g}+\mtx{Y}^T\mtx{M}^T\w+b\vct{1}_n-\mtx{Y}_\ell - \tb}+ \beta\frac{\vct{h}^T\w}{\sqrt{n}} + \frac{\twonorm{\Db\vct{t}}^2}{2n} \nn\\
%&=min_{\w, b,\tb}\text{ }\max_{\beta\ge 0}~\min_{\tau>0}\text{ } &\frac{\beta\tau}{2} + \frac{\beta}{2\tau}}\twonorm{ \twonorm{\w}\vct{g}+\mtx{Y}^T\mtx{M}^T\w+b\vct{1}_n-\mtx{Y}_\ell - \tb}+ \beta\frac{\vct{h}^T\w}{\sqrt{n}} + \frac{\twonorm{\Db\vct{t}}^2}{2n} \nn\\
%&\quad\quad\quad\quad\quad\quad=\min_{\w, b}\text{ }\frac{1}{2n}\left(\twonorm{ \twonorm{\w}\vct{g}+\mtx{Y}^T\mtx{M}^T\w+b\vct{1}_n-\mtx{Y}_\ell}+ \vct{h}^T\w\right)_{+}^2\\
%&\quad\quad\quad\quad\quad\quad=\frac{1}{2}\left(\min_{\w, b}\text{ } \frac{1}{\sqrt{n}}\twonorm{ \twonorm{\w}\vct{g}+\mtx{Y}^T\mtx{M}^T\w+b\vct{1}_n-\mtx{Y}_\ell}+\frac{1}{\sqrt{n}} \vct{h}^T\w\right)_{+}^2
\end{align*}

To continue, consider the eigenvalue decomposition  
\begin{align}\label{eq:M_SVD_w}
\mtx{M}=\mtx{U}\mtx{\Sigma}\mtx{V}^T = 
\begin{bmatrix}\ub_1 & \ub_2 & \ldots & \ub_r \end{bmatrix} \diag{\sigma_1,\sigma_2,\ldots,\sigma_r} \begin{bmatrix}\vb^T_1 \\ \vb_2^T \\ \ldots \\ \vb_r^T \end{bmatrix} ,
\end{align}
with $\mtx{U}\in\R^{d\times r}$, $\mtx{\Sigma}\in\R^{r\times r}$, and $\mtx{V}\in\R^{k\times r}$ where $r=$rank$(\mtx{M})\le k$. We further decompose $\w_\ell$ in its projections on the orthogonal columns $\ub_1,\ldots,\ub_r$ of $\Ub$:
$$
\w_\ell = \sum_{i=1}^{r}\alpha_i \ub_i + \alpha_0\w_\ell^\perp, 
$$
where $\twonorm{\w_\ell^\perp}=1$ and $\Ub^T\w_\ell^\perp = \mathbf{0}$, $\alpha_0\geq 0$ and  we denote
\bea\label{eq:alphab_def_w}
\alpha_i := \ub_i^T\w_\ell, i\in[r].
\end{align}
In this notation, the AO becomes {\color{blue}Argue flipping min-max}
\begin{align}
%&\min_{\alpha_0\geq 0, \{\alpha_i\}_{i=1}^r, b ,\tb}\text{ }\max_{\beta\geq 0} \frac{\beta}{\sqrt{n}}\twonorm{ \sqrt{\alpha_0^2 + \sum_{i=1}^r\alpha_i^2}\,\vct{g}+\sum_{i=1}^{r}\alpha_i\sigma_i\mtx{Y}^T\Vb\eb_i  +b\vct{1}_n-\mtx{Y}_\ell}+ \sum_{i=1}^{r}{\beta \alpha_i\frac{\vct{h}^T\ub_i}{\sqrt{n}}} + \frac{\beta \alpha_0}{\sqrt{n}}\min_{\w_\ell^\perp}\left(\h^T\w_\ell^\perp\right) +\frac{\twonorm{\Db\tb}^2}{2}\nn\\
%&
\min_{\substack{\alpha_0\geq 0, \{\alpha_i\}_{i=1}^r, \\ b,\tb}}\text{ }\max_{\beta\geq0} \frac{\beta}{\sqrt{n}}\twonorm{ \sqrt{\alpha_0^2 + \sum_{i=1}^r\alpha_i^2}\,\vct{g}+\sum_{i=1}^{r}\alpha_i\sigma_i\mtx{Y}^T\vb_i  +b\vct{1}_n-\mtx{Y}_\ell - \tb}+ \sum_{i=1}^{r}{\beta\alpha_i\frac{\vct{h}^T\ub_i}{\sqrt{n}}} -\beta\alpha_0\frac{\twonorm{\h^\perp}}{\sqrt{n}}+\frac{\twonorm{\Db\tb}^2}{2n},\label{eq:scal_AO}
\end{align}
where we denote $\h^\perp$ the projection of $\h$ onto the complement subspace of the span of $\ub_1,\ldots,\ub_r$ and we used that $\twonorm{\w^\perp_\ell} = 1$ and $\inp{\w^\perp_\ell}{\ub_i}=0, i\in[r]$.

Next, we use the fact that 
\begin{align}\label{eq:sqrt_trick}
\chi = \min_{\tau>0} \,\frac{\tau}{2} + \frac{\chi^2}{2\tau},~\chi> 0
\end{align}
 to rewrite the AO as {\color{blue}Argue flipping max-min to bring $\min_{\tau}$ outside}
\begin{align}
&\min_{\substack{\alpha_0\geq 0, \{\alpha_i\}_{i=1}^r, \\ b,\tb, \tau>0}}\text{ }\max_{\beta\geq0} \frac{\beta\tau}{2} +  \frac{\beta}{2\tau{n}}\twonorm{ \fb - \tb}^2+ \sum_{i=1}^{r}{\beta\alpha_i\frac{\vct{h}^T\ub_i}{\sqrt{n}}} -\beta\alpha_0\frac{\twonorm{\h^\perp}}{\sqrt{n}}+\frac{\twonorm{\Db\tb}^2}{2n}, \nn\\\label{eq:scal_AO_w}
=&\min_{\substack{\alpha_0\geq 0, \{\alpha_i\}_{i=1}^r, \\ b,\tb, \tau>0}}\text{ }\max_{\beta\geq0} \frac{\beta\tau}{2} +  \frac{\beta}{2\tau{n}}\twonorm{ \fb }^2 + \sum_{i=1}^{r}{\beta\alpha_i\frac{\vct{h}^T\ub_i}{\sqrt{n}}} -\beta\alpha_0\frac{\twonorm{\h^\perp}}{\sqrt{n}}+\frac{\twonorm{\Db\tb}^2}{2n}+ \frac{\beta}{2\tau{n}}\twonorm{ \tb }^2 -  \frac{\beta}{\tau{n}}\fb^T\tb ,\nn\\
=&\min_{\substack{\alpha_0\geq 0, \{\alpha_i\}_{i=1}^r, \\ b,\tb, \tau>0}}\text{ }\max_{\beta\geq0} \frac{\beta\tau}{2} +  \frac{\beta}{2\tau{n}}\twonorm{ \fb }^2 + \sum_{i=1}^{r}{\beta\alpha_i\frac{\vct{h}^T\ub_i}{\sqrt{n}}} -\beta\alpha_0\frac{\twonorm{\h^\perp}}{\sqrt{n}}+\frac{1}{2n}\left( \tb^T\left(\Db^2+\left({\beta}/{\tau}\right)\Iden_n\right)\tb - \frac{2\beta}{\tau}\fb^T\tb \right).\nn
\end{align}
where we denote for convenience
\begin{align}
\fb:=\fb\left(\alpha_0, \{\alpha_i\}_{i=1}^r,b\right) = \sqrt{\alpha_0^2 + \sum_{i=1}^r\alpha_i^2}\,\vct{g}+\sum_{i=1}^{r}\alpha_i\sigma_i\mtx{Y}^T\vb_i  +b\vct{1}_n-\mtx{Y}_\ell
\end{align}
{\color{blue}Argue flipping max-min to bring $\min_{\tb}$ inside}We can now optimize over $\tb$ to conclude with the following equivalent formulation of the AO as an optimization problem over only scalar variables:
\begin{align}
&\min_{\substack{\alpha_0\geq 0, \{\alpha_i\}_{i=1}^r, \\ b,\tau>0}}\text{ }\max_{\beta\geq0} \frac{\beta\tau}{2} +  \frac{\beta}{2\tau{n}}\twonorm{ \fb }^2 + \sum_{i=1}^{r}{\beta\alpha_i\frac{\vct{h}^T\ub_i}{\sqrt{n}}} -\beta\alpha_0\frac{\twonorm{\h^\perp}}{\sqrt{n}} - \left(\frac{\beta^2/\tau^2}{\omega^2+\beta/\tau}\right)\left(\frac{1}{2n}\sum_{j\in\Cc_j}\fb_j^2\right) - \left(\frac{\beta^2/\tau^2}{1+\beta/\tau}\right)\left(\frac{1}{2n}\sum_{j\not\in\Cc_j}\fb_j^2\right),\nn\\
=&\min_{\substack{\alpha_0\geq 0, \{\alpha_i\}_{i=1}^r, \\ b,\tau>0}}\text{ }\max_{\beta\geq0} \frac{\beta\tau}{2} + \sum_{i=1}^{r}{\beta\alpha_i\frac{\vct{h}^T\ub_i}{\sqrt{n}}} -\beta\alpha_0\frac{\twonorm{\h^\perp}}{\sqrt{n}} + \left(\frac{1}{\omega^2+\tau/\beta}\right)\left(\frac{1}{2n}\sum_{j\in\Cc_j}\fb_j^2\right) + \left(\frac{1}{1+\tau/\beta}\right)\left(\frac{1}{2n}\sum_{j\not\in\Cc_j}\fb_j^2\right),\label{eq:scal_AO_w2}
\end{align}
where we also recalled \eqref{eq:Db_ell}.

\vp
\noindent\textbf{Convergence of the AO.}~~Let us define $\pib_{-\ell}:=\pib-\pi_\ell\eb_\ell$ and
\begin{subequations}
\begin{align}\label{eq:Amat_w}
\A_\ell&:=\pi_\ell \begin{bmatrix} \Iden_r+\Sigmab\Vb^T\diag{\eb_\ell}\Vb\Sigmab & \Sigmab\Vb^T\eb_\ell \\ \eb_\ell^T\Vb\Sigmab & 1 \end{bmatrix}\quad\quad\text{and}\quad \cb_\ell = \begin{bmatrix} \Sigmab\Vb^T\eb_\ell \\ 1 \end{bmatrix} \\
\A_{-\ell}&:=\begin{bmatrix} (1-\pi_\ell)\Iden_r+\Sigmab\Vb^T\diag{\pib_{-\ell}}\Vb\Sigmab & \Sigmab\Vb^T\pib_{-\ell} \\ \pib_{-\ell}^T\Vb\Sigmab & 1-\pi_\ell \end{bmatrix} \nn
\end{align}
\end{subequations}
Using the WLLN and recalling the definitions of $\Y,\Y_\ell$ it can shown that

\begin{align}
\frac{1}{n}\sum_{j\in\Cc_j}\fb_j^2 &\rP \pi_\ell\left(\alpha_0^2+\twonorm{\alphab}^2\right)+b^2\pi_\ell + \pi_\ell + \alphab^T\Sigmab\Vb^T\diag{\pi_\ell\eb_\ell}\Vb\Sigmab\alphab - 2b\pi_\ell - 2\pi_\ell\eb_\ell^T\Vb\Sigmab\alphab + 2b\pi_\ell\eb_\ell^T\Vb\Sigmab\alphab \nn\\
&\qquad= \pi_\ell\alpha_0^2 + \pi_\ell + \begin{bmatrix}\alphab & b\end{bmatrix}^T\A_\ell \begin{bmatrix}\alphab \\ b\end{bmatrix} - 2\pi_\ell\cb_\ell^T\begin{bmatrix}\alphab & b\end{bmatrix}\nn
\\
\frac{1}{n}\sum_{j\not\in\Cc_j}\fb_j^2 &\rP (1-\pi_\ell)\left(\alpha_0^2+\twonorm{\alphab}^2\right)+b^2(1-\pi_\ell) + \alphab^T\Sigmab\Vb^T\diag{\pib_{-\ell}}\Vb\Sigmab\alphab  + 2b\pib_{-\ell}^T\Vb\Sigmab\alphab,
\nn\\
&\qquad= (1-\pi_\ell)\alpha_0^2  + \begin{bmatrix}\alphab & b\end{bmatrix}^T\A_{-\ell} \begin{bmatrix}\alphab \\ b\end{bmatrix}\nn.
\end{align}
Using this and
$$
\frac{\twonorm{\h^\perp}}{\sqrt{n}}\rP \sqrt{\gamma}\quad\text{and}\quad\frac{\vct{h}^T\ub_i}{\sqrt{n}}\rP 0,
$$
the objective function in \eqref{eq:scal_AO_w} converges pointwise to the following:
\bea\label{eq:Dc_w}
\Dc(\alpha_0,\alphab,b,\tau,\beta):= \frac{\beta\tau}{2} - \beta\alpha_0\sqrt{\gamma} + \frac{\alpha_0^2}{2}\left(
\frac{\pi_\ell}{\omega^2+\tau/\beta}+\frac{1-\pi_\ell}{1+\tau/\beta}\right) + \frac{\pi_\ell}{\omega^2+\tau/\beta} +  \frac{1}{2}\begin{bmatrix}\alphab & b\end{bmatrix}^T\widetilde \A_\ell \begin{bmatrix}\alphab \\ b\end{bmatrix} - \widetilde\cb_\ell^T\begin{bmatrix}\alphab & b\end{bmatrix},
\end{align}
where we have denoted
$$
\widetilde\A_\ell = \widetilde\A_\ell(\tau,\beta) = \frac{\pi_\ell}{\omega^2+\tau/\beta} \A_\ell + \frac{1-\pi_\ell}{1+\tau/\beta} \A_{-\ell}\quad\text{and}\quad\widetilde\cb_\ell = \cb_\ell(\tau,\beta) = \frac{\pi_\ell}{\omega^2+\tau/\beta} \cb_\ell.
$$
The function $\Dc$ is clearly convex in $\alpha_0,\alphab$ and $b$. Also, by the second-derivative test, it can be shown that it is convex in $\tau$ and concave in $\beta$.


\vp
\noindent\textbf{Deterministic analysis}~~It is easy to optimize \eqref{eq:Dc_w} with respect to $\alpha_0,\alphab$ and $b$. Their optimal values are found as follows:
\begin{align}
\alpha_0 &= \left({{\beta}\sqrt{\gamma}}\right)\Big/\left({\frac{\pi_\ell}{\omega^2+\tau/\beta}+\frac{1-\pi_\ell}{1+\tau/\beta}}\right),\\
\begin{bmatrix} \alphab \\ \beta \end{bmatrix} &= \left(\widetilde\A_\ell(\tau,\beta)\right)^{-1}\widetilde\cb_\ell(\tau,\beta),
\end{align}
where $\tau>0,\beta\geq 0$ are solutions to the following min-max optimization
\begin{align}
\min_{\tau>0}~\max_{\beta\geq 0}~\frac{\beta\tau}{2} - \frac{\pi_\ell}{\omega^2+\tau/\beta} - \frac{\beta^2\gamma}{2\left({\frac{\pi_\ell}{\omega^2+\tau/\beta}+\frac{1-\pi_\ell}{1+\tau/\beta}}\right)} - \frac{1}{2}\left(\widetilde\cb_\ell(\tau,\beta)\right)^T\left(\widetilde\A_\ell(\tau,\beta)\right)^{-1}\widetilde\cb_\ell(\tau,\beta).
\end{align}



